LoLCATs: On Low-Rank Linearizing of Large Language Models

Recent works show we can linearize large language models (LLMs) -- swapping the quadratic attentions of popular Transformer-based LLMs with subquadratic analogs, such as linear attention -- avoiding the expensive pretraining costs. However, linearizing LLMs often significantly degrades model quality, still requires training over billions of tokens, and remains limited to smaller 1.3B to 7B LLMs. We thus propose Low-rank Linear Conversion via Attention Transfer (LoLCATs), a simple two-step method that improves LLM linearizing quality with orders of magnitudes less memory and compute. We base these steps on two findings. First, we can replace an LLM's softmax attentions with closely-approximating linear attentions, simply by training the linear attentions to match their softmax counterparts with an output MSE loss ("attention transfer"). Then, this enables adjusting for approximation errors and recovering LLM quality simply with low-rank adaptation (LoRA). LoLCATs significantly improves linearizing quality, training efficiency, and scalability. We significantly reduce the linearizing quality gap and produce state-of-the-art subquadratic LLMs from Llama 3 8B and Mistral 7B v0.1, leading to 20+ points of improvement on 5-shot MMLU. Furthermore, LoLCATs does so with only 0.2% of past methods' model parameters and 0.4% of their training tokens. Finally, we apply LoLCATs to create the first linearized 70B and 405B LLMs (50x larger than prior work). When compared with prior approaches under the same compute budgets, LoLCATs significantly improves linearizing quality, closing the gap between linearized and original Llama 3.1 70B and 405B LLMs by 77.8% and 78.1% on 5-shot MMLU.

==> sections/3_method_old.tex <==

% \input{sections/figures/pull_method}

\section{Method: Linearizing LLMs with \name{}}
\label{sec:method}
We now study how to build a high-quality and highly efficient linearizing method.
%
In Section~\ref{sec:method_framework}, we present our motivating framework,
which aims to (1) learn good softmax attention approximators with linear attentions and (2) enable low-rank adaptation for recovering linearized quality.
% which simply adapts prior swapping-and-finetuning approaches to (1) learn good softmax attention approximators before (2) only using low-rank adaptation. 
%
In Section~\ref{sec:method_study}, we find that while this attention transfer works surprisingly well for low-rank linearizing with existing linear attentions, on certain tasks, it still results in sizable quality gaps compared to prior methods. 
% To support our motivating hypothesis, 
We also find that attention-transfer quality strongly corresponds with the final linearized model's performance. In Section~\ref{sec:method_new_stuff}, we use our learned findings to overcome prior issues, improving attention transfer to subsequently improve low-rank linearizing quality.

% \vspace{-1cm}
\subsection{A Framework for Low-cost Linearizing}
\label{sec:method_framework}

In this section, we present our initial \name{} framework for linearizing LLMs in an effective yet efficient manner. Our main hypothesis is that by first learning linear attentions that approximate softmax, we can then swap these attentions in as drop-in subquadratic replacements. We would then only need a minimal amount of subsequent training---\eg{} that is supported by low-rank updates---to recover LLM quality in a cost-effective manner effectively. We thus proceed in two steps.


% Similar to prior works, we swap each attention in an LLM with a subquadratic analog, before training the model end-to-end with next-token prediction to the modifying layers. 
%
% This involves (1) learning linear attentions that approximate softmax attention, and (2) swapping these learned linear attentions and only finetuning the modified model with LoRA. We train both stages with natural language data.

% Intuitively, if we could replace every LLM softmax attention with a nearly matching linear attention, then we would only need minimal amounts of subsequent training to adjust and recover original LLM quality. Furthermore, by restricting this training to low-rank updates on the attention layers, we hope to avoid drastic or deleterious changes to the pretrained parameters,~\eg{} to preserve pretrained knowledge and avoid overfitting to the linearizing data. 

% We thus proceed in two steps.

% \subsubsection{Replacing Softmax with Parameter-Efficient Attention Transfer}
% \label{sec:method_attn_transfer}

\begin{enumerate}[leftmargin=*]
    \item \textbf{Parameter-Efficient Attention Transfer.} For each softmax attention in an LLM, we aim to learn a closely-approximating linear attention, \ie{} one that computes attention outputs $\hat{\bm{y}} \approx \bm{y}$ for all natural inputs $\bm{x}$. 
    %
    We treat this as a feature map learning problem, learning $\phi$ to approximate softmax. For each head and layer, let $\phi_q, \phi_k$ be query, key feature maps. Per head, we compute:
    \begin{equation}
        \bm{y}_n = \underbrace{
    % \bm{y}_n = 
    \sum_{i=1}^n \frac{ \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})}{\sum_{i=1}^n \exp(\bm{q}_n^\top \bm{k}_i  / \sqrt{d} )} \bm{v}_i
    }_{\text{Softmax Attention}},\;\;\;\;
    \hat{\bm{y}}_n = 
    \underbrace{
    % \hat{\bm{y}}_n = 
    \sum_{i=1}^n \frac{ \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i)}{\sum_{i=1}^n \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i) } \bm{v}_i
    }_{\text{Linear Attention}}
    \end{equation}
    for all $n \in [l]$ with input $\in \mathbb{R}^{l \times d}$,
    and train $\phi_q, \phi_k$ to minimize sample mean squared error (MSE)
    \begin{equation}
    % \begin{align}
        \ell_\text{MSE} = \frac{1}{MH}\sum_{m = 1}^M \sum_{h=1}^H
        \ell_\text{MSE}^{h, m}\;\;,\;\;\;\; 
        \ell_\text{MSE}^{h, m} = \frac{1}{d} \sum_{n=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2
    % \end{align}
        \label{eq:mse_loss}
    \end{equation}
    \ie{} jointly for each head $h$ in layer $m$.
    Similar to past work~\citep{kasai-etal-2021-finetuning,zhang2024the}, rather than manually design $\phi$, we parameterize each $\phi : \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$ as a \textit{learnable} layer:
    % followed by a nonlinear activation,~\ie{} 
    \[
    \phi_q(\bm{q}_n) := f(\bm{q}_n\tilde{\bm{W}}_{(q)} + \tilde{\bm{b}}_{(q)})\;\;,\;\;\;
    \phi_k(\bm{k}_i) := f(\bm{k}_i\tilde{\bm{W}}_{(k)} + \tilde{\bm{b}}_{(k)})
    \]
    Here $\tilde{\bm{W}} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}} \in \mathbb{R}^{d'}$ are trainable weights and optional biases, 
    $f(\cdot)$ is a nonlinear activation, and $d'$ is an arbitrary feature dimension (set to equal head dimension $d$ in practice).
% To train $\phi$, we simply sample layer-wise ($\bm{x},\bm{y}$) as pretrained attention inputs and outputs, computed with our target LLM's inference over natural language samples (Fig.~\ref{}). We train all $\phi$ jointly to minimize Eq.~\ref{eq:attn_matching_setup} with outputs ($\hat{\bm{y}},\bm{y}$) (see App.~\ref{} for training code and implementation details, with more discussion on advantages over related work~\citep{zhang2024the} that supervises with all attention weights ($\hat{\bm{a}},\bm{a}$)).
% % (Fig.~\ref{}; training code and implementation details in App.~\ref{}). Rather than supervise with the attention weights~\citep{zhang2024the}, we also just use outputs to train directly to minimize Eq.~\ref{eq:attn_matching_setup}. This lets us avoid prior   
% Finally, in general we can use any linear attention with learnable $\phi$. To develop \name{} we explore several options that vary in $f(\cdot)$ from prior work. 

% \vspace{0.2cm}

\item \textbf{Low-rank Adjusting.} After training the linearizing layers, we replace the full-parameter training of prior work with low-rank adaptation (LoRA)~\citep{hu2021lora}. 
%
Like prior work, to adjust for the modifying layers and recover language modeling quality, we now train the modified LLM end-to-end over tokens to minimize a sample next-token prediction loss
% over some sample data $\bm{u}$ with a 
% \begin{equation}
\(
\ell_\text{xent} = -\sum \log P_\Theta(\bm{u}_{t+1} \mid \bm{u}_{1:t})
\).
% \label{eq:cross_entropy_loss}
% \end{equation}
%
Here $P_\Theta$ is the modified LLM, $\Theta$ is the set of LLM parameters, and we aim to maximize the probability of true $\bm{u}_{t+1}$ given past tokens $\bm{u}_{1:t}$ (Fig.~\ref{fig:pull_method}~right). 
However, rather than train all LLM parameters, we only train the swapped linear attention $\bm{W}_q, \bm{W}_k, \bm{W}_v, \bm{W}_o$ with LoRA. 
% for parameter-efficiency we only train the query, key, value, and output projections  of the swapped linear attention layers with LoRA. 
Instead of full-rank updates, $\bm{W}' \leftarrow \bm{W} + \Delta \bm{W}$, LoRA decomposes $\Delta \bm{W}$
as the product of two low-rank matrices $\bm{B}\bm{A}$, $\bm{B} \in \mathbb{R}^{d \times r}$, $\bm{A} \in \mathbb{R}^{r \times d}$. 
% We then jointly train all layers 
For parameter efficiency, 
% (\eg{} updating only 0.2\% of a 7B+ LLM's parameters), 
we aim to pick small $r \ll d$. 
\end{enumerate}

\textbf{Training footprint and efficiency}. Both steps remain parameter-efficient.
    For Step 1, optimizing Eq.~\ref{eq:mse_loss} is similar to a layer-by-layer cross-architecture distillation. We compute layer-wise ($\bm{x}, \bm{y}$) as pretrained attention inputs and outputs, using an LLM forward pass over natural language samples (Fig.~\ref{fig:pull_method} middle).
    %
    However, to keep our training footprint low, we freeze the original pretrained attention layer's parameters and 
    % initializing new linear attention layers (or models). We 
    simply \textit{insert} new $\phi_q, \phi_k$ after $\bm{W}_q, \bm{W}_k$ in each softmax attention (Fig.~\ref{fig:pull_method} left). We compute outputs $\bm{y},\hat{\bm{y}}$ with the same attention weights in separate passes (choosing either Eq.~\ref{eq:causal_attention} or Eq.~\ref{eq:linear_attention_2}; Fig.~\ref{fig:pull_method} middle).  
    % By jointly training each head and layer, we make attention transfer 
    %
    For Llama 3 8B or Mistral 7B, training $\phi_q,\phi_k$ with $d' = 64$ then only takes 32 layers $\times$ 32 heads $\times$ 2 feature maps $\times$ (128 $\times$ 64) weights $\approx$ 16.8M trainable weights (0.2\% of LLM sizes). For Step 2, LoRA with $r=8$ on all attention projections suffices for state-of-the-art quality. This updates just $<$0.09\% of 7B parameters.
    % \yell{Also compare to prior linearizing methods in percent of weights changed?}

% For both attention transfer and low-rank linearizing, our key hypothesis is that we can find sufficient linear attention implementations, such that by \emph{training} to minimize Eq.~\ref{eq:attn_matching_setup} over sample data (``attention transfer''), we can learn close enough softmax approximations over natural LLM attention inputs. Then, even if these are not perfect drop-in replacements, we only need minimal amounts of attention weight training---\ie{} that coverable by LoRA with low $r$---to adjust and recover quality. 
% %
% Furthermore, by focusing our training over linearizing data to recover attention sequence modeling patterns, instead of relearning pretrained knowledge, we hypothesize that if \name{} suffices to recover zero-shot LLM abilities, it should also be more token-efficient than full-parameter methods.
% % (our first stage only trains $\bm{q},\bm{k}$ interactions), 


\subsection{Baseline Study: Attention Transfer and Low-rank Linearizing}
\label{sec:method_study}

We now aim to understand if attention transfer and low-rank adjusting are sufficient for linearizing LLMs. 
It is unclear whether these simple steps can lead to high-quality LLMs, given that 
% While intuitive, 
prior works default to more involved approaches~\citep{mercat2024linearizing,yang2024parallelizing,wang2024mamba}. They use linearizing layers featuring GroupNorms~\citep{wu2018group} and decay factors~\citep{sun2023retentive}, or alternate SSM-based architectures~\citep{gu2023mamba,dao2024transformers}. They also all use full-LLM training after swapping in the subquadratic layers. 
%
In contrast, we find that simple linear attentions \textit{can} lead to viable linearizing, with attention transfer + LoRA obtaining competitive quality on 4~/~6 popular LM Eval tasks. 

% Later in Section~\ref{}, we show how by learning better softmax approximations, we can completely close this gap. 
% 
%

% As a baseline study, we thus first explore if we can simply use existing linear attentions under the \name{} framework for high quality yet highly efficient linearizing.
% %
% Somewhat surprisingly, we find that while either attention transfer or LoRA alone fails to lead to convincingly linearized LLMs, simply combining them achieves competitive quality with just 40M tokens (Table~\ref{}).
% %
% However, we do encounter larger quality drops for more challenging tasks. We later study the source of these issues in Section~\ref{}, and present solutions to propose our final method in Section~\ref{}.

\input{sections/figures/method_attn_transfer_curves}
\begin{table}[t]
\vspace{-0.125cm}
\begin{center}
\resizebox{0.96\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
& \multicolumn{4}{c}{Llama 3 8B}                                  & \multicolumn{4}{c}{Mistral 7B}                                  \\ 
% \cmidrule(lr){1-1}
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
  \multicolumn{1}{c}{Attention}                       & \multicolumn{2}{c}{T2R}        & \multicolumn{2}{c}{Hedgehog}   & \multicolumn{2}{c}{T2R}        & \multicolumn{2}{c}{Hedgehog}   \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
\multicolumn{1}{c}{Transfer?} & \cellcolor[HTML]{ECF4FF} PPL@0      &  PPL@2/4     & \cellcolor[HTML]{ECF4FF} PPL@0      &  PPL@2/4       & \cellcolor[HTML]{FFDECA}  PPL@0      &  PPL@2/4      & \cellcolor[HTML]{FFDECA} PPL@0      &  PPL@2/4     \\ 
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
No\; \xmark               & \cellcolor[HTML]{ECF4FF} 1539.39        &  16.05         & \cellcolor[HTML]{ECF4FF} 2448.01        &  9.02          & \cellcolor[HTML]{FFDECA} 2497.13        &  8.85          & \cellcolor[HTML]{FFDECA} 561.47         &  4.87          \\
Yes\; \cmark               & \cellcolor[HTML]{ECF4FF} \textbf{79.33} & \textbf{4.11} & \cellcolor[HTML]{ECF4FF} \textbf{60.86} &  \textbf{3.90} & \cellcolor[HTML]{FFDECA} \textbf{32.78} &  \textbf{3.29} & \cellcolor[HTML]{FFDECA} \textbf{18.94} &  \textbf{3.04} \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-0.25cm}
\caption{\small Alpaca validation set perplexity (PPL) of linearized LLMs, comparing attention transfer, no LoRA adjusting (PPL@0) and PPL after training (PPL@2/4; 2 with attention transfer, 4 without, for equal total steps).
}
\label{table:train_efficiency}
\vspace{-0.35cm}
\end{table}

\paragraph{Experimental Setup.} We test the \name{} framework by linearizing two popular base LLMs, Llama 3 8B~\citep{AI_2024} and Mistral 7B v0.1~\citep{jiang2023mistral}. For linearizing layers, we study two feature maps used in prior work (T2R~\citep{kasai-etal-2021-finetuning} and Hedgehog~\citep{zhang2024the}, Table~\ref{table:linear_attentions_def}). 
% \simran{I still don't really understand why the ROPE thing is super important to the main paper.}
To support the rotary positional embeddings (RoPE)~\citep{su2024roformer} in these LLMs, we apply the feature maps $\phi$ after RoPE,\footnote{
Unlike prior works that apply $\phi$ before RoPE~\citep{mercat2024linearizing, su2024roformer}, our choice preserves the linear attention kernel connection, where we can hope to learn $\phi_q, \phi_k$ for $\exp(\bm{q}_n^\top \bm{k}_i/\sqrt{d}) \approx \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i)$. 
% With the same feature maps, we find this leads to more efficient linearizing in App.~\ref{}.
}
% We show how this allows us to find suitable $\phi$ by only training feature map weights in a parameter- and token-efficient manner.
\ie{} computing query features $\phi_q(\bm{q}) = f(\text{RoPE}(\bm{q})\tilde{\bm{W}}_q + \tilde{\bm{b}}))$.
%
For linearizing data, we wish to see if \name{} with a small amount of data can recover general zero-shot and instruction-following LLM abilities. We use the 50K samples of a cleaned Alpaca dataset\footnote{\url{https://huggingface.co/datasets/yahma/alpaca-cleaned}}, due to its ability to improve general instruction-following in 7B LLMs despite its relatively small size~\citep{alpaca}. Following~\cite{zhang2024the}, we train all feature maps jointly. 
% where layer-wise distillation is similar to finetuning a single model 
We include training code and implementation details in App.~\ref{appendix:implementation_details}).
%

\begin{wraptable}{r}{0.5\textwidth}  % 'r' for right, width 40% of text width
\vspace{-0.25cm}
\centering
\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lcl@{}}
\toprule
Feature Map              & $\phi(\bm{q})$ (same for $\bm{k}$) & Weight Shapes     \\ \midrule
T2R  & $\text{ReLU}(\bm{q}\tilde{\bm{W}} + \tilde{\bm{b}})$ & 
% $\tilde{\bm{W}} \in \mathbb{R}^{128 \times 128}, \tilde{\bm{b}} \in \mathbb{R}^{128}$ \\
$\tilde{\bm{W}}$: (128, 128), $\tilde{\bm{b}}$: (128,) \\
Hedgehog               & $[\text{SM}_d(\bm{q}\tilde{\bm{W})} \oplus \text{SM}_d(-\bm{q}\tilde{\bm{W})} ]$ &
% $\tilde{\bm{W}} \in \mathbb{R}^{128 \times 64}$ 
$\tilde{\bm{W}}: (128, 64)$ 
\\ \bottomrule
\end{tabular}
}
\vspace{-0.125cm}
\caption{\small \textbf{Learnable feature maps}. Transformer to RNN (T2R) from~\cite{kasai-etal-2021-finetuning}, Hedgehog from~\cite{zhang2024the}, both $\oplus$ (concat) and $\text{SM}_d$ (softmax) apply over feature dimension.}
\label{table:linear_attentions_def}
\vspace{-0.25cm}
\end{wraptable}
% }

To study the effects of attention transfer and low-rank linearizing across LLMs and linear attention architectures, we evaluate their validation set perplexity (Table~\ref{table:train_efficiency}, Fig.~\ref{fig:train_efficiency}) and downstream LM Eval zero-shot quality (Table~\ref{table:prelim_mmlu}).
% , (also including sample generations in App.~\ref{}). 
We train both stages with the same data, evaluate with early stopping, and use either two epochs for both attention transfer and LoRA adjusting or four epochs with either alone ($\approx$~40M total training tokens). For LoRA, we use $r = 8$ as a popular default~\citep{hu2021lora}, which results in training 0.2\% of LLM parameter counts. 
% We defer additional training details to App.~\ref{}.

\paragraph{Attention Transfer + LoRA Enables Fast LLM Linearizing.} In Table~\ref{table:train_efficiency} and Fig.~\ref{fig:train_efficiency}, we report the validation PPL of linearized LLMs, ablating attention transfer and LoRA adjusting. We find that while attention transfer alone is often insufficient (\textit{c.f.,} PPL@0, Table~\ref{table:train_efficiency}), a single low-rank update rapidly recovers performance by 15--75 PPL (Fig.~\ref{fig:train_efficiency}), 
where training to approximate softmax leads to up to 11.9 lower PPL than no attention transfer.
% achieves \textcolor{red}{17.3} lower perplexity (PPL) than prior analogs trained with 40M tokens (\textcolor{red}{2.7 versus 20.1 PPL}).
% showing viable 7B LLM linearizing at orders of magnitude less training costs than previously shown.
% With the latter taking 5,000$\times$ the tokens, we find we can viably linearize 7B LLMs at magnitudes smaller training costs than previously shown. 
%
Somewhat surprisingly, this translates to performing competitively with prior linearizing methods that train \textit{all} model parameters~\citep{mercat2024linearizing,wang2024mamba} (within 5 accuracy points on 4~/~6 popular LM Eval tasks; Table~\ref{table:prelim_mmlu}), while \textit{only} training with 0.04$\%$ of their token counts and 0.2\% of their parameter counts. The results suggest we can linearize 7B LLMs at orders-of-magnitude less training costs than previously shown.

\input{sections/figures/method_train_efficiency}

\input{sections/figures/method_problems_llama3}

% the combination of attention transfer and LoRA adjusting consistently achieves best linearized quality. 
% %
% Furthermore, in Fig.~\ref{fig:train_efficiency} we find attention transfer enables rapid recovery in language modeling quality, where a single low-rank update reduces PPL by $\sim$15--75 points.
% %
% Considering zero-shot capability recovery, in Table~\ref{table:prelim_mmlu} we find the better performing Hedgehog LLMs remain competitive on 4~/~6 popular LM Eval tasks (within 5 points of contemporary methods). This is despite only training on 0.04$\%$ of other methods' token counts, and updating $<$0.02\% of their parameter counts. Finally, in Fig.~\ref{fig:mse_vs_ppl} we find that attention matching (via MSE; averaged over all heads and layers) strongly corresponds with better linearized model quality (lower PPL).

\paragraph{\textsc{LoL SAD}: Limitations of Low-Rank Linearizing.} At the same time, we note quality limitations with the present framework. 
%
While sometimes close, low-rank linearized LLMs perform worse than full-parameter alternatives and original Transformers on 5~/~6 LM Eval tasks (up to 42.4 points on 5-shot MMLU; Table~\ref{table:prelim_mmlu}). 
To understand the issue, we study whether the attention transfer stage can produce high-fidelity linear approximations of softmax attention. We note four observations:
\begin{enumerate}[leftmargin=*]
    \item Attention transfer quality (via output MSE) strongly correlates with the downstream low-rank linearization quality (Fig.~\ref{fig:mse_vs_ppl}). This suggests that MSE is a useful way to measure quality during attention transfer.
    \item Larger attention output MSEs coincide with lower softmax attention weight entropies (Fig.~\ref{fig:mse_error_llama3_entropy}). However, prior work shows that lower-entropy distributions are difficult to approximate with linear attentions \citep{zhang2024the}.
    \item Larger MSEs also heavily concentrate in attention input samples from later layers (Fig.~\ref{fig:mse_error_llama3_layer}). Since the MSE metric is scale-sensitive, the later layers could impact our ability to train the earlier layers, using the simple loss summation across layers in \Cref{eq:mse_loss}.
    \item The variation in MSE magnitudes increases with model scale. In Tables~\ref{table:mse_blocks_70b} and \ref{table:mse_blocks_405b}, we measure the magnitude of the MSE loss by layer depth at the 70B and 405B scales. The magnitudes range between 0.02~--~48.66 at the 405B scale versus 0.0008~--~2.91 at the 70B scale. 
\end{enumerate}
% (2) ; and (3) larger MSEs coincide with attention samples from later layers .
%
% isolating these patterns
We thus hypothesize we can improve quality by reducing MSE in two ways. 
%
First, to approximate samples with lower softmax attention weight entropies---\ie{} ``spikier'' distributions more challenging to capture with linear attentions~\citep{zhang2024the}---we may need better attention-matching architectures. 
%
Second, to address the difficulty of learning certain attention layers, we may need more fine-grained layer-wise supervision instead of jointly training all layers, especially for larger models. 


% \subsection{Study of baseline approaches}
% % \label{sec:method_study}
% \textcolor{blue}{
% \begin{itemize}
%     \item What do they do in perplexity and MMLU
%     \item What are the outstanding challenges
% \end{itemize}
% }

% Our observations 



\subsection{\name{}: Improved Low-rank Linearizing}
\label{sec:method_new_stuff}
% \textcolor{blue}{
% \begin{itemize}
%     \item Figure with SWA + linear (MSEs)
%     \item Figure with the attention transfer -- training-wise
%     \item Cost model
% \end{itemize}
% }
We now introduce two simple improvements in architecture (\Cref{sec:method_analogs}) and linearizing procedure (\Cref{sec:method_training}) to improve low-rank linearizing quality. 
% We focus on these linearizing components in this work but also include additional experiments on data selection in App~\ref{}.

\subsubsection{Architecture: Generalizing Learnable Linear Attentions}
% \subsubsection{Architecture: Expanding Learnable $\phi$ Parameterizations}
\label{sec:method_analogs}
% \paragraph{Expanding Learnable $\bm{\phi}$ Parameterizations.} 
As described, we can apply our framework with any linear attentions with learnable $\phi$ (\textit{e.g.}, T2R and Hedgehog, Figure~\ref{fig:train_efficiency}). 
% In our method development, we evaluate two learnable $\phi$ parameterizations. First, we consider the pure linear attention setup discussed above, evaluating how the T2R and Hedgehog activations transfer to our \name{} setting in Section~\ref{}.
%
However, to improve attention-matching quality, we introduce a hybrid $\phi$ parameterization combining linear attention and \textit{sliding window} attention. Motivated by prior works that show quality improvements when combining attention layers with linear attentions~\citep{arora2024simple,Munkhdalai2024-kx}, 
% recurrences~\citep{de2024griffin}, and state-space models~\citep{fu2022hungry,stripedhyena,lieber2024jamba}, 
we combine \textcolor{blue}{short sliding windows} of softmax attention~\citep{beltagy2020longformer,zhu2021long} (size 64 in experiments) followed by linear attention in a single layer. This allows attending to all prior tokens for each layer while keeping the entire LLM subquadratic. For window size $w$ and token indices $[1, \ldots, n-w, \ldots, n]$, we apply the softmax attention over the $w$ most recent tokens, 
and compute attention outputs $\hat{\bm{y}}_n$ as
% \begin{equation}
%     \hat{\bm{y}}_n =  
%     \frac{ \textcolor{blue}{\sum_{i=n-w+1}^n \gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)\bm{v}_i} + \textcolor{cyan}{\phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)\bm{v}_j^\top \big)}}{ \textcolor{blue}{\sum_{i = {n-w+1}}^n\gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)}\; +  \textcolor{cyan}{\phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)^\top \big)}} 
% \label{eq:hybrid_linear_swa}
% \end{equation}
\begin{equation}
    \hat{\bm{y}}_n =  
    \frac{ \textcolor{blue}{\sum_{i=n-w+1}^n \gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)\bm{v}_i} + \phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)\bm{v}_j^\top \big)}{ \textcolor{blue}{\sum_{i = {n-w+1}}^n\gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)}\; +  \phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)^\top \big)} 
\label{eq:hybrid_linear_swa}
\end{equation}
$\gamma$ is a learnable mixing term, and $\bm{c}_n$ is a stabilizing constant as in log-sum-exp calculations ($\bm{c}_n = \max_i\big\{\bm{q}_n^\top \bm{k}_i / \sqrt{d} : i \in [n-w+1, \ldots, n]\big\}$).
Like before, we can pick any learnable $\phi$.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/mse_analogs_llama3_8b_serif.png}
%         % \vspace{-0.5cm}
%         \caption{Llama 3 8B}
%         \label{fig:mse_analogs_llama3}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/mse_analogs_mistral_7b_serif.png}
%         \caption{Mistral 7B (v0.1)}
%         \label{fig:mse_analogs_mistral7b}
%     \end{subfigure}
%     \vspace{-0.25cm}
%     \caption{\textbf{Attention matching MSE}. Across LLMs, linearizing with hybrid linear attention + sliding window better approximates ``ground-truth'' softmax attentions via lower MSE over layers.}
%     \label{fig:mse_analogs}
%     \vspace{-0.25cm}
% \end{figure}

\input{sections/figures/method_attn_mse}

\paragraph{Subquadratic efficiency.} The hybrid layer retains linear time and constant memory generation. For $n$-token prompts, we initially require $\mathcal{O}(w^2 d)$ and $\mathcal{O}((n-w)dd')$ time and space for window and linear attention respectively, attending over a $w$-sized KV-cache and computing KV and K-states (Eq.~\ref{eq:linear_attention_recurrent}). 
For generation, we only need $\mathcal{O}(w^2 d + dd')$ time and space for every token. We evict the KV-cache's first $\bm{k}$, $\bm{v}$, compute $\phi_k(\bm{k})$, and add $\phi_k(\bm{k})\bm{v}^\top$ and  $\phi_k(\bm{k})$ to KV and K-states respectively.

\subsubsection{Training: Layer (or Block)-wise Attention Transfer}
\label{sec:method_training}
We describe the \name{} training approach and provide a simplified model to show its cost-quality tradeoffs.
%
% We modify the training objective in Eq.~\ref{eq:mse_loss} as follows. 
Based on the limitations of low-rank linearizing identified in the prior section, we perform attention transfer at a block-by-block granularity for the large scale models. The MSE loss function is scale-sensitive and our study showed that the later layers consistently result in larger MSEs  (Fig.~\ref{fig:mse_error_llama3_layer}).
Thus, instead of computing the training loss (Eq.~\ref{eq:mse_loss}) over
all $m \in [M]$ for a model with $M$ layers, we compute the loss over $k$-layer blocks, and train each block independently:
% \begin{equation}
%     \ell_\text{MSE}(\bm{y}, \hat{\bm{y}}) =  \sum_{n=1}^{L} \frac{1}{d}\sum_{j=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2 \rightarrow \ell_\text{MSE}(\bm{y}, \hat{\bm{y}}) = \sum_{n=i}^{i+k} \frac{1}{d}  \sum_{j=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2 
%     \label{eq:mse_loss_blocks}
% \end{equation}
\begin{equation}
    % \begin{align}
        \ell_\text{MSE}^{\text{block}} = \frac{1}{kH}\sum_{m = i}^{i + k} \sum_{h=1}^H
        \ell_\text{MSE}^{h, m}\;\;\;\; 
        % \ell_\text{MSE}^{h, m} = \frac{1}{d} \sum_{n=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2,\;\;\;\; 
        (\text{for blocks starting at layers } i = 0, k, 2k, \ldots),
    % \end{align}
        \label{eq:mse_loss_blocks}
    \end{equation}
where the training data for the block starting at layer $i$ is the hidden states outputted by prior block starting at layer $i-k$, for each sequence in the training corpus. After attention transfer, we arrange the blocks back together in their original order. Like before, we then do end-to-end LoRA finetuning to recover quality.
% using an end-to-end LoRA fine-tuning stage. 

\begin{wraptable}{r}{0.24\textwidth}  % 'r' for right, width 40% of text width
\vspace{-0.5cm}
\centering
\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lcl@{}}
\toprule
Method              &  $k \times c$  &  PPL\\ \midrule
Joint          &  126$\times$1  & 4.23 \\
Block-wise      &  9$\times$14  & 3.21
\\ \bottomrule
\end{tabular}
}
\vspace{-0.125cm}
\caption{\small \textbf{Attention transfer} for Llama 3.1 405B using $c$ blocks of $k$ layers.}
\label{table:block_wise}
\vspace{-5mm}
\end{wraptable}

\paragraph{Tradeoffs between quality and efficiency.} We show that the block-wise approach improves linearization quality at large model scales and improves the user's ability to flexibly balance compute and memory efficiency tradeoffs. We compare (1) \textbf{joint ($k=126$)} training, where we load the full model once and compute the loss as the sum of layer-wise MSEs, and (2) \textbf{block-wise ($k=9$)} training, where we break the model into blocks and train each independently.

For quality, we compare the evaluation perplexity of both the attention transfer approaches, after LoRA fine-tuning on the same subset of RedPajama data. The block-wise and joint approaches perform similarly at the 8B and 70B scales, however, as shown in Table~\ref{table:block_wise}, the block-wise approach performs 1.02 points better than joint attention transfer at the 405B scale. These results support our study in Section~\ref{sec:method_study}, which shows the  variation in MSE magnitudes grows large at the 405B scale. 
% To understand why block-wise helps for the largest models, 
% Finer grained block-wise supervision appears to help handle this variation.
% These results emphasize that the large MSEs may warrant finer-grained supervision during attention transfer.



% Especially at the larger LLM scales (e.g., Llama 3.1 405B), we find that jointly performing attention transfer over all $126$ layers fails to produce high quality LLMs. We observe that the uneven magnitudes in the attention outputs, with later layers consistently carrying larger MSEs than earlier ones, presents a challenge (Figure). Across the 70B and 405B parameter models, we show that setting smaller $k$ leads to improved quality (Table).
% The primary costs-tradeoffs between these two approaches are:
Next, for efficiency, we compare the compute and memory use for both methods:
\begin{itemize}[leftmargin=*]
    \item Compute: 
    % Large block sizes, $k$, require more compute to train each block. 
    While the joint training of Llama 3.1 405B in 16-bit precision uses \textit{multiple nodes} (e.g., NVIDIA H100 8$ \times$80GB nodes), an individual block of $k=9$ or fewer layers can be trained on a \textit{single GPU} (e.g., H100 80GB GPU), at sequence length 1024. The block-wise approach is also amenable to using a different training duration (and training data) per block.
    \item Memory: To train block $i$, we need to save the hidden states from the prior block to disk. The total amount of disk space required is 
\(
2 \times T \times d \times \frac{L}{k}
\)
for total training tokens $T$, model dimension $d$, number of layers $L$ and 2-byte (16-bit) precision. 
At the Llama 3.1 405B scale, saving states per-layer ($k=1$) for just $50$M tokens would require over 200TB of disk space, while $k=126$ (joint training) requires no additional disk space for the states.
% Meanwhile, we do not need to save any hidden states for the joint training approach. 
% Sequentially saving the outputs and training the blocks increases total training time.  
% and effort. 
\end{itemize}
% Finally, decentralized training offers the flexibility to 
% The flexibility offered by our training procedure may benefit researchers studying sub-quadratic LLMs on an academic budget.
% the compute required to train each block of $k$ layers and the memory requirement to save hidden outputs of prior blocks as inputs to later ones.  


% \newpage{}


% We describe how we distill Llama 3.1 $70$B and Llama $405$B to linearized \name{}s, in 16-bit precision, on an academic budget. 
% We first evaluate the vanilla \name{} approach used for the $8$Bn parameter models in \Cref{sec:405b_baseline} and then highlight simple extensions enabled by the \name{} framework that provide further  quality and efficiency improvements in \Cref{sec:405b_approach}.
%
% All prior work on linearization operates below $10$Bn parameters in model size \cite{}. We demonstrate that \name{} enables the first hundred-billion parameter sub-quadratic model. Furthermore, our procedure requires just $8$ hours of training.  
%
% \label{sec:405b_baseline}
% We first directly apply the vanilla  \name{} approach, which led to state-of-the-art quality at the $8$Bn parameter scale, to the $70$Bn and $405$Bn models. The results are included in \Cref{table:scale_baseline}. 
%
% \name{} excitingly achieves X\% of Llama 3.1 70B quality with just X\% of trainable parameters and X\% of the number of pretraining tokens. As in the case of the 8Bn parameter models, the initial attention transfer stage helps improve quality by X points on average. 

% However, the vanilla approach falls short at the 405Bn parameter scale, both with and without the initial attention transfer stage. Above this, the $16$-bit $405$B model, requiring a total of $810$ GB for the model parameters alone, does not fit in a single $8 \times 80$GB GPU commodity box, requiring expensive multi-node training that is beyond the scope of most academic budgets. 
% In the next section, we study how to address these limitations and unlock high quality linearized 405Bn parameter models. 
%
% \begin{table}[!h]
% \scriptsize
% \begin{center}
% \resizebox{0.96\linewidth}{!}{
% \begin{tabular}{@{}ccccccccc@{}}
% & \multicolumn{2}{c}{Llama 3.1 70B}                                  & \multicolumn{2}{c}{Llama 3.1 405B}                                  \\ 
% \cmidrule(lr){2-5} 
% % \cmidrule(lr){6-8}
%   \multicolumn{1}{c}{Attention}                       & 
%   \multicolumn{2}{c}{Hedgehog}      & \multicolumn{2}{c}{Hedgehog}   \\ 

% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% \multicolumn{1}{c}{Transfer?} & \cellcolor[HTML]{ECF4FF} Start PPL      &  End PPL       & \cellcolor[HTML]{ECF4FF} Start PPL      &  End PPL  \\ 
% \cmidrule(lr){1-1}
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% No\; \xmark               & \cellcolor[HTML]{ECF4FF}    &        & \cellcolor[HTML]{ECF4FF}     &    \\
% Yes\; \cmark               & 
% \cellcolor[HTML]{ECF4FF} \textbf{} & \textbf{} & \cellcolor[HTML]{ECF4FF} \textbf{} & \textbf{}  \\ 
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \vspace{-2mm}
% \caption{Initial and final perplexities of low-rank linearized LLMs with and without attention transfer at the 70B and 405B parameter scales. 
% }
% \label{table:scale_baseline}
% \vspace{-0.5cm}
% \end{table}
%
% \subsection{Mini \name{} in a trenchcoat}
% \label{sec:405b_approach}
% We show how simple extensions to the \name{} approach unlock quality and efficiency in the large scale regime. For this section, recall that Llama 3.1 405B has a model dimension of $16,384$ and $126$ Transformer layers.
%
% \paragraph{Finer-grained supervision} Recall that in the vanilla \name{} approach is that the total training loss during the attention transfer stage is the sum of the MSE loss between the true and linearized attention maps at each individual layer. We hypothesize that especially for very deep models, like Llama 405B with 126 Transformer layers, the loss scale may greatly vary across the layers, making it difficult to jointly supervise all layers. The natural next step train for attention transfer at a finer-grained, perhaps layer-by-layer, granularity.
%
% \paragraph{Cost Model: Tradeoffs Between Scaled up Quality and Cost.}
%
% \paragraph{Tradeoffs between quality and cost}

==> sections/4_results_old.tex <==
\section{Experiments}
\label{sec:results}
% \vspace{-0.125cm}

Through experiments, we study: (1) if \name{} linearizes LLMs with higher quality than existing subquadratic alternatives and linearizations, and higher generation efficiency than original Transformers (Section~\ref{sec:main_results});  (2) how ablations on attention transfer loss, subquadratic architecture, and parameter and token counts impact LLM downstream quality (Section~\ref{sec:results_ablations}); (3) how \name{}' quality and efficiency holds up to 70B and 405B LLMs, where we linearize and compare model quality across the complete Llama 3.1 family (Section~\ref{sec:chungus_amongus}).

\subsection{Main Results: \name{} Efficiently Recovers Quality in Linearized LLMs}
\label{sec:main_results}

In our main evaluation, we linearize the popular base Llama 3 8B~\citep{AI_2024} and Mistral 7B~\citep{jiang2023mistral} LLMs. We first test if \name{} can efficiently create high-quality subquadratic LLMs from strong base Transformers, comparing to existing linearized LLMs from prior methods. We also test if \name{} can create subquadratic LLMs that outperform modern Transformer alternatives pretrained from scratch. For space, we defer linearizing training details to App.~\ref{appendix:experimental_details}.

\input{sections/tables/main_results_linearize}

\input{sections/tables/main_results_v2_local}

% \paragraph{Natural Language Understanding.} 
In Table~\ref{table:main_results}, we report results on six popular LM Evaluation Harness (LM Eval) tasks~\citep{eval-harness}.
%
Compared to recent linearizing methods, \name{} significantly improves quality and training efficiency across tasks and LLMs. On quality, \name{} closes 
% 73.8\% and 81.1\% 
79.8\% and 86.6\%
of the Transformer-linearizing gap for Mistral 7B and Llama 3 8B respectively, notably improving 5-shot MMLU by 
% 63.8\% and 50\% 
60.9\% and 40.9\% 
over next best fully subquadratic models (17.2 and 9.6 points). On efficiency, we achieve these results while only training $<$0.2\% of model parameters via LoRA versus prior full-parameter training. We also only use 40M tokens versus the prior 20~--~100B (a 500~--~2500$\times$ improvement in ``tokens-to-model'' efficiency).
%
Among all 7B LLMs, \name{}-linearized LLMs further outperform strong subquadratic Transformer alternatives, representing RNNs or linear attentions (RWKV-v6~\citep{peng2024eagle}, Hawk, Griffin~\citep{de2024griffin}, TransNormer~\citep{qin2023scaling}), state-space models (Mamba~\citep{gu2023mamba}), and hybrid architectures with some full attention (StripedHyena~\citep{stripedhyena}, Zamba~\citep{glorioso2024zamba}). 

\subsection{\name{} Component Properties and Ablations}
\label{sec:results_ablations}
We next validate that \name{} linearizing enable subquadratic efficiency, and study how each of \name{}' components contribute to these linearizing quality gains.

\input{sections/figures/benchmark_efficiency}

\paragraph{Subquadratic Generation Throughput and Memory.} We measure the generation throughput and memory of \name{} LLMs, validating that linearizing LLMs can significantly improve their generation efficiency. We use the popular Llama 3 8B HuggingFace checkpoint\footnote{\url{https://huggingface.co/meta-llama/Meta-Llama-3-8B}}, and compare \name{} implemented in HuggingFace Transformers with the supported FlashAttention-2 (FA2) implementation~\citep{dao2023flashattention}. We benchmark on a single 80GB H100 and benchmark two \name{} implementations with the Hedgehog feature map and (linear + sliding window) attention in FP32 and BF16. In Fig.~\ref{fig:generation_throughput} and Fig.~\ref{fig:generation_memory}, we report the effect of scaling batch size on throughput and memory. We measure throughput as $($newly generated tokens $\times$ batch size $/$ total time$)$, using 128 token prompts and 4096 token generations. As batch size scales, \name{}-linearized LLMs achieve significantly higher throughput than FA2. We note this is primarily due to lower memory, where FA2 runs out of memory at batch size 64. Meanwhile, \name{} supports up to 3000 tokens / second with batch size 2048 (Fig.~\ref{fig:generation_throughput}), only maintaining a fixed ``KV state'' as opposed to the growing KV cache in all attention implementations (Fig.~\ref{fig:generation_memory}).

\paragraph{Ablations.}
We study how adding the attention transfer and linear + sliding window attention in \name{} contribute to downstream linearized LLM performance, linearizing  Llama 3 8B over 1024-token long samples (Table~\ref{table:main_results_ablations}). We start with standard linear attentions (Hedgehog,~\cite{zhang2024the}; T2R,~\cite{kasai-etal-2021-finetuning}), using the prior linearizing procedure of just swapping attentions and finetuning the model to predict next tokens~\citep{mercat2024linearizing}. We then add either (i) attention transfer, (ii) linear + sliding window attentions, or (iii) both, and report the average LM Eval score over the six popular zero-shot tasks in Table~\ref{table:main_results} and 5-shot MMLU accuracy. Across feature maps, we validate the \name{} combination leads to best performance.


\input{sections/tables/main_results_ablation_v2}

\subsection{Scaling Up Linearizing to 70B and 405B LLMs}
\label{sec:chungus_amongus}
We finally use \name{} to scale up linearizing to Llama 3.1 70B and 405B models. 
%
In Table~\ref{table:chungus_results}, we find that \name{} provides the first practical solution for linearizing larger LLMs, achieving significant quality improvements over prior linearizing approaches of swapping in attentions and finetuning~\citep{mercat2024linearizing}. Controlling for the same linear + sliding window layer, for Llama 3.1 70B we achieve a 
% 41.1 
39.0
point improvement in 5-shot MMLU accuracy. For Llama 3.1 405B, \name{} similarly achieves a 38.3 point improvement. These results highlight \name{}' ability to linearize large-scale models with greater efficiency and improved performance, showing for the first time that we can scale up linearizing to 70B+ LLMs.

\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{0.99\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                       & PiQA           & ARC Easy       & ARC Challenge  & HellaSwag      & WinoGrande     & MMLU (5-shot)  \\ 
                       & acc            & acc            & (acc norm)     & (acc norm)     & acc            & acc            \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Llama 3.1 8B          & 79.87          & 81.52          & 53.58          & 79.01          & 73.48          & 66.11          \\
Linearized, no attn. transfer & 78.67	& 78.11	& 49.83	& 77.83 & 	68.51 & 	51.44          \\



\name{} (Ours)                & \textbf{80.96} & \textbf{82.37} & \textbf{54.44} & \textbf{79.07} & \textbf{69.69} & \textbf{54.88} \\ \midrule

\rowcolor[HTML]{EFEFEF} 
Llama 3.1 70B          & 83.10          & 87.30          & 60.60          & 85.00          & 79.60          & 78.80          \\
% Linearized, no attn. transfer & 75.70          & 70.10          & 39.10          & 77.40          & 58.60          & 26.60          \\

Linearized, no attn. transfer & 81.99 &	80.89 &	54.44 &	82.29 &	71.19 &	28.74 \\
\name{} (Ours)                & \textbf{82.10} & \textbf{84.98} & \textbf{60.50} & \textbf{84.62} & \textbf{73.72} & \textbf{67.70} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Llama 3.1 405B         & 85.58          & 87.58          & 66.21          & 87.13          & 79.40          & 82.98          \\
Linearized, no attn. transfer & 84.44          & 86.62          & 64.33          & 86.19          & 79.87          & 33.86          \\
\name{} (Ours)                & \textbf{85.58} & \textbf{88.80} & \textbf{67.75} & \textbf{87.41} & \textbf{80.35} & \textbf{72.20} \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{Linearizing Llama 3.1 70B and 405B}. Among the first linearized 70B and 405B LLMs (via low-rank linearizing), \name{} significantly improves zero- and few-shot quality.
}
\label{table:chungus_results}
% \vspace{-0.5cm}
\end{table}


==> sections/figures/attention_weights.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats-Softmax-q=122_h=0-m=distill_llama3_8b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_llama_softmax}
    \end{subfigure}
    % \hfill
    \vspace{-0.5cm}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats-Softmax-q=122_h=0-m=distill_mistral_7b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_mistral_softmax}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats-LoLCATs-q=122_h=0-m=distill_llama3_8b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_llama_lolcats}
    \end{subfigure}
    % \hfill
    \vspace{-0.5cm}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats-LoLCATs-q=122_h=0-m=distill_mistral_7b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_mistral_lolcats}
    \end{subfigure}
    % \vspace{-0.5cm}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats-LoLCATs_;_;(init.)-q=122_h=0-m=distill_llama3_8b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        \caption{Llama 3 8B attention weights}
        \label{fig:attn_maps_llama_lolcats_init}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats-LoLCATs_;_;(init.)-q=122_h=0-m=distill_mistral_7b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        \caption{Mistral 7B (v0.1) attention weights}
        \label{fig:attn_maps_mistral_lolcats_init}
    \end{subfigure}
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats_vla-Hedgehog-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Llama 3 8B attention weights}
    %     \label{fig:attn_maps_llama_hedghog}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats_vla-Hedgehog-q=122_h=0-m=distill_mistral_7b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Mistral 7B (v0.1) attention weights}
    %     \label{fig:attn_maps_mistral_hedgehog}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats_vla-Hedgehog_;_;(init.)-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Llama 3 8B attention weights}
    %     \label{fig:attn_maps_llama_hedghog_init}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps_lolcats_vla-Hedgehog_;_;(init.)-q=122_h=0-m=distill_mistral_7b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Mistral 7B (v0.1) attention weights}
    %     \label{fig:attn_maps_mistral_hedgehog_init}
    % \end{subfigure}
    % \vspace{-0.5cm}
    \caption{\textbf{Attention Transfer}. For both Llama 3 8B and Mistral 7B v0.1 LLMs, \name{} attention transfer trains subquadratic attentions that match original attention weights, despite only supervising based on attention layer outputs. They also learn to recover weights outside of the softmax windows, \textit{c.f.} trained versus initialized (init.) attentions between queries at positions 130 - 150 and keys at positions 0 -  32.}
    \label{fig:results_attn_weight_ex}
\end{figure}

==> sections/figures/benchmark_efficiency.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/benchmark_thruput_bs.png}
%         % \vspace{-0.5cm}
%         \caption{Batch size vs.~Throughput}
%         \label{fig:generation_throughput}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/benchmark_memory_bs.png}
%         \caption{Batch size vs.~Memory}
%         \label{fig:generation_memory}
%     \end{subfigure}
%     \vspace{-0.25cm}
%     \caption{\textbf{\name{} Generation Efficiency}, Llama 3 8B.}
%     \label{fig:bm_efficiency}
%     \vspace{-0.25cm}
% \end{figure}
\begin{wrapfigure}{r}{0.55\textwidth}
% \hspace{-1cm}
% \vspace{-0.9cm}
\vspace{-0.75cm}
    \centering
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/benchmark_thruput_bs.png}
        % \vspace{-0.5cm}
        % \caption{Batch size vs.~Thruput}
        \label{fig:generation_throughput}
    \end{subfigure}
    \vspace{-0.12cm}
    % \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/benchmark_memory_bs.png}
        % \vspace{-0.5cm}
        % \caption{Batch size vs.~Mem.}
        \label{fig:generation_memory}
    \end{subfigure}
    % \vspace{-0.12cm}
    % \vspace{-0.5cm}
    \vspace{-1cm}
    \caption{\small \textbf{ Generation Efficiency}, Llama 3 8B.}
    \label{fig:bm_efficiency}
    \vspace{-0.75cm}
    % \vspace{-0.5cm}
\end{wrapfigure}


==> sections/figures/method_attn_weight_comparison.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.235\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps-Softmax-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
        \caption{Ground-truth}
        \label{fig:attn_match_softmax}
    \end{subfigure}
    % \hfill
    % \vspace{-0.5cm}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps-Hedgehog (init.)-q=122_h=0-m=distill_llama3_8b_lk_t2r-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
        \caption{Untrained}
        \label{fig:attn_match_no_train}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps-Hedgehog-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent_mse1000_lr1e-2.pdf}
        \caption{Cross-entropy Loss}
        \label{fig:attn_match_xent_loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/attn_maps/attn_maps-Hedgehog-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
        \caption{MSE Loss (Ours)}
        \label{fig:attn_match_mse_loss}
    \end{subfigure}
    \caption{\textbf{Attention weight comparison}. Across layers of Llama 3 8B, we visualize sample attention weights computed for queries 120 -- 152  and keys 0 -- 32, 120 -- 152. We compare original softmax attentions (\ref{fig:attn_match_softmax}), Hedgehog attentions without attention transfer (\ref{fig:attn_match_no_train}), Hedgehog trained with the prior cross-entropy loss on attention weights~\cite{zhang2024the} (\ref{fig:attn_match_xent_loss}), and Hedgehog trained with our proposed MSE loss on attention outputs (\ref{fig:attn_match_mse_loss}). Despite only training to minimize MSE of attention outputs, we still recover similar attention weights.}
    % \vspace{-0.5cm}
    \label{fig:method_attn_weight_comparison}
\end{figure}

==> sections/figures/pull_results_v2.tex <==
\begin{figure*}[t]
  \centering
   \vspace{-0.25cm}
  % \includegraphics[width=\textwidth]{figures/pull_fig_combine_v1.pdf}
  {figures/lolcats_pull_v3.pdf}
  \vspace{-0.5cm}
  % \vspace{-0.5cm}
  \caption{\small By training subquadratic attentions to match an LLM's softmax attentions (``attention transfer''), (\textbf{top-left}), \textbf{\name{}} allows using low-rank adaptation to convert exist LLMs into subquadratic variants (\textbf{bottom-left}). 
  %  
  With only 0.003\% of the tokens required to pretrain prior 7B subquadratic LLMs, this creates state-of-the-art-quality ``linearized'' LLMs 
  % with state-of-the-art quality and training efficiency (closing average overall LM Eval score gap by 24.1-97.0\%, with only 0.003-0.04\% of the training tokens)
  that close LM Evaluation Harness~\cite{eval-harness} gaps to Transformers by 24.1-97.0\% (\textbf{middle}), while retaining subquadratic capabilities such as constant memory generation (\textbf{right}) \MZ{placeholder}.
  % /the training tokens of prior subquadratic LLMs
  }
  
  % Via what we call ``attention transfer'', \name{} trains subquadratic attentions to match softmax attentions for rapid linearization (left), with state-of-the-art linearized LLM zero-to-few-shot quality and training efficiency (middle), while turning existing Transformer-based LLMs into fully recurrent models (right).}
\vspace{-0.5cm}
\label{fig:pull_method}
\end{figure*}

==> sections/figures/results_attn_weight_ex.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats-Softmax-q=122_h=0-m=distill_llama3_8b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_llama_softmax}
    \end{subfigure}
    % \hfill
    \vspace{-0.5cm}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats-Softmax-q=122_h=0-m=distill_mistral_7b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_mistral_softmax}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats-LoLCATs-q=122_h=0-m=distill_llama3_8b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_llama_lolcats}
    \end{subfigure}
    % \hfill
    \vspace{-0.5cm}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats-LoLCATs-q=122_h=0-m=distill_mistral_7b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        % \caption{Llama 3 8B, T2R}
        \label{fig:attn_maps_mistral_lolcats}
    \end{subfigure}
    % \vspace{-0.5cm}
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats-LoLCATs_;_;(init.)-q=122_h=0-m=distill_llama3_8b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        \caption{Llama 3 8B attention weights}
        \label{fig:attn_maps_llama_lolcats_init}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats-LoLCATs_;_;(init.)-q=122_h=0-m=distill_mistral_7b_lk_smd_wtk64_fd64_w01-d=distill_alpaca_clean_xent0_mse1000_lr1e-2 (1).pdf}
        \caption{Mistral 7B (v0.1) attention weights}
        \label{fig:attn_maps_mistral_lolcats_init}
    \end{subfigure}
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats_vla-Hedgehog-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Llama 3 8B attention weights}
    %     \label{fig:attn_maps_llama_hedghog}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats_vla-Hedgehog-q=122_h=0-m=distill_mistral_7b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Mistral 7B (v0.1) attention weights}
    %     \label{fig:attn_maps_mistral_hedgehog}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats_vla-Hedgehog_;_;(init.)-q=122_h=0-m=distill_llama3_8b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Llama 3 8B attention weights}
    %     \label{fig:attn_maps_llama_hedghog_init}
    % \end{subfigure}
    % % \hfill
    % \begin{subfigure}[b]{0.49\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/lolcats/attn_maps/attn_maps_lolcats_vla-Hedgehog_;_;(init.)-q=122_h=0-m=distill_mistral_7b_lk_smd_fd64-d=distill_alpaca_clean_xent0_mse1000_lr1e-2.pdf}
    %     \caption{Mistral 7B (v0.1) attention weights}
    %     \label{fig:attn_maps_mistral_hedgehog_init}
    % \end{subfigure}
    % \vspace{-0.5cm}
    \caption{\textbf{Attention Transfer}. For both Llama 3 8B and Mistral 7B v0.1 LLMs, \name{} attention transfer trains subquadratic attentions that match original attention weights, despite only supervising based on attention layer outputs. They also learn to recover weights outside of the softmax windows, \textit{c.f.} trained versus initialized (init.) attentions between queries at positions 130 - 150 and keys at positions 0 -  32.}
    \label{fig:results_attn_weight_ex}
\end{figure}

==> sections/iclr_0_abstract.tex <==
% \vspace{=0.25cm}
\begin{abstract}

\noindent Recent works show we can linearize large language models (LLMs)---swapping the quadratic attentions of popular Transformer-based LLMs with subquadratic analogs, such as linear attention---avoiding the expensive pretraining costs.  
However, linearizing LLMs
often significantly degrades model quality, still requires training over billions of tokens, and remains limited to smaller 1.3B to 7B LLMs.
% We show that the subquadratic analogs used in prior work struggle to approximate the original softmax attention layer. 
We thus propose Low-rank Linear Conversion via Attention Transfer (\name{}), a simple two-step method that improves LLM linearizing quality with orders of magnitudes less memory and compute. 
% \name{} is based on two findings: 
We base these steps on two findings.
First, we can replace an LLM's softmax attentions with closely-approximating linear attentions, simply by 
\textit{training} the linear attentions to match their softmax counterparts with an output MSE loss (``\textit{attention transfer}'').
Then, this enables adjusting for approximation errors and recovering LLM quality simply with \textit{low-rank} adaptation (LoRA).
\name{} significantly improves linearizing quality, training efficiency, and scalability. We significantly reduce the linearizing quality gap and produce state-of-the-art subquadratic LLMs from Llama 3 8B and Mistral 7B v0.1, leading to 20+ points of improvement on 5-shot MMLU. Furthermore, \name{} does so with only 0.2\% of past methods' model parameters and 0.04-0.2\% of their training tokens.  
Finally, we apply \name{} to create the first linearized 70B and 405B LLMs (50$\times$ that of prior work).
When compared with prior approaches under the same compute budgets, \name{} significantly improves linearizing quality, closing the gap between linearized and original Llama 3.1 70B and 405B LLMs by 77.8\% and 78.1\% on 5-shot MMLU.
\end{abstract}

==> sections/iclr_1_intro.tex <==
% \input{sections/figures/pull_results}
% \input{sections/figures/pull_results_v2}

\section{Introduction}
\label{sec:intro}

% Opening; why interesting
``Linearizing'' large language models (LLMs)---or converting existing Transformer-based LLMs into attention-free or subquadratic alternatives---has shown promise for scaling up efficient architectures. While many such architectures offer complexity-level efficiency gains, like \textit{linear-time} and \textit{constant-memory} generation, they are often limited to smaller models pretrained on academic budgets~\citep{gu2023mamba,peng2023rwkv,yang2023gated,arora2024simple,beck2024xlstm}.  
% In complement, 
In a complementary direction,
linearizing aims to start with openly available LLMs---\eg{} those with 7B+ parameters pretrained on trillions of tokens~\citep{AI_2024,jiang2023mistral}---and (i) swap their softmax attentions with subquadratic analogs, before (ii) further finetuning to recover quality. This holds exciting promise for quickly scaling up subquadratic capabilities.
% in modern LLMs.

% Problem; why hard
However, to better realize this promise and allow anyone to convert LLMs into subquadratic models, we desire methods that are
(1) \textbf{quality-preserving}, \eg{} to recover the zero-shot abilities of modern LLMs; (2) \textbf{parameter and token efficient}, to linearize LLMs on widely accessible compute; and (3) \textbf{highly scalable}, to support linearizing 70B+ LLMs available today~\citep{touvron2023llama,touvron2023llama2}. 
% recent methods struggle to maintain high (1) \textbf{quality-preservation}, (2) \textbf{training efficiency}, and (3) \textbf{large model scalability}. 

Existing methods present opportunities to improve all three criteria.
On quality, despite using motivated subquadratic analogs such
as RetNet-inspired 
linear attentions~\citep{sun2023retentive,mercat2024linearizing} 
% \textit{linear attentions}~\citep{katharopoulos2020transformers,mercat2024linearizing} 
or state-space model (SSM)-based 
Mamba layers~\citep{gu2023mamba,bick2024transformers,wang2024mamba},
prior works significantly reduce performance on popular LM Evaluation Harness tasks (LM Eval)~\citep{eval-harness} (up to 23.4-28.2 pts on 5-shot MMLU~\citep{hendrycks2020measuring}).
%
On parameter and token efficiency, to adjust for architectural differences, prior methods update \textit{all} model parameters in at least one stage of training~\citep{mercat2024linearizing,wang2024mamba,bick2024transformers}, and use 20~-~100B tokens to linearize 7B LLMs.
%
On scalability, these training costs make linearizing larger models on academic compute more difficult; 
% we uncover additional quality and feasibility challenges.
% these costs further limit linearizing's viability as a way to quickly scale up subquadratic architectures on academic compute. 
existing works only linearize up to 8B LLMs. This makes it unclear how to support linearizing 70B to 405B LLMs~\citep{dubey2024llama}.


\input{sections/figures/pull_method}

In this work, we thus propose \textbf{\name{}} 
(\textbf{\textsc{Lo}}w-rank \textbf{\textsc{L}}inear \textbf{\textsc{C}}onversion with \textbf{\textsc{A}}ttention \textbf{\textsc{T}}ran\textbf{\textsc{s}}fer), a simple approach to improve the quality, efficiency, and scalability of linearizing LLMs. 
As guiding motivation, we ask if we can linearize LLMs by simply reducing architectural differences,~\ie{}
\begin{enumerate}[leftmargin=*]
    \item Starting with simple softmax attention analogs such as linear attention (Eq.~\ref{eq:linear_attention_2}), and \textit{training} their parameterizations explicitly to approximate softmax attention (``\textbf{attention transfer}'').
    \item Subsequently only training with low-cost finetuning to adjust for any approximation errors,~\eg{} with low-rank adaptation (LoRA)~\citep{hu2021lora} (``\textbf{low-rank linearizing}'').
\end{enumerate}

In evaluating this hypothesis, we make several contributions. 
%
First, to better understand linearizing feasibility, we empirically study attention transfer and low-rank linearizing with existing linear attentions. While intuitive---by swapping in perfect subquadratic softmax attention approximators, we could get subquadratic LLMs with no additional training---prior works suggest linear attentions struggle to match softmax expressivity~\citep{keles2023computational,qin-etal-2022-devil} 
% are expensive to train as softmax approximators~\citep{zhang2024the}, 
% They also 
or need full-model updates to recover linearizing quality~\citep{kasai-etal-2021-finetuning,mercat2024linearizing}. 
%  This calls into question if LoRA can suffice to recover quality post-swapping.
%
In contrast, we find that while \textit{either} attention transfer or LoRA alone is insufficient, we can rapidly recover quality by simply doing \textit{both} (Figure~\ref{fig:train_efficiency}, Table~\ref{table:train_efficiency}). 
%
At the same time, we do uncover quality issues related to attention-matching architecture and training. With prior linear attentions, the best low-rank linearized LLMs still significantly degrade in quality  
% get significant quality gaps 
vs.~original Transformers (up to 42.4 pts on 5-shot MMLU). 
%
With prior approaches that train all attentions jointly~\citep{zhang2024the}, we also find that later layers can result in 200$\times$ the MSE of earlier ones (Figure~\ref{fig:mse_analogs}). We later find this issue aggravated by larger LLMs; jointly training all Llama 3.1 405B's 126 attention layers fails to viably linearize. 

Next, to resolve these issues and improve upon our original criteria, we detail \name{}' method components. 
For \textbf{quality}, we generalize prior notions of learnable linear attentions to sliding window + linear attention variants. These remain subquadratic to compute yet consistently yield better attention transfer via lower mean-squared error (MSE) on attention outputs. For \textbf{parameter and token efficiency}, we maintain our simple 2-step framework of (1) training subquadratic attentions to match softmax attentions, 
% via only their feature maps, 
before (2) adjusting for any errors via only LoRA. For \textbf{scalability}, we use finer-grained ``block-by-block''
% \footnote{Or for Llama models, cria-by-cria, where a cria is a baby llama $\smwhitestar \smallwhitestar \medwhitestar$} 
training. We split LLMs into blocks of $k$ layers before jointly training attentions only within each block to improve layer-wise attention matching. We pick $k$ to balance the speed of training blocks in parallel with the memory of saving hidden state outputs of prior blocks (as inputs for later ones). We provide a simple cost model to navigate these tradeoffs.
% in Section~\ref{sec:chungus_amongus}.

Finally, in experiments, we validate that \name{} improves on
each of our desired criteria.
\begin{itemize}[leftmargin=*]
    \item On \textbf{quality}, when linearizing popular LLMs such as Mistral-7B and Llama 3 8B, \name{} substantially improves past linearizing methods (by 
    % 0.2$-$8.0 
    1.1$-$8.6 
    points (pts) on zero-shot LM Eval tasks; 
    % +17.8 pts 
    +17.2 pts 
    on 5-shot MMLU)). With Llama 3 8B, \name{} for the first time closes the zero-shot LM Eval gap between linearized and Transformer models 
    % (73.1 vs 73.7 pts),
    (73.1 vs 74.2 pts),
    while supporting 3$\times$ the throughput and 64$\times$ the batch sizes vs.~popular FlashAttention-2~\citep{dao2023flashattention} models (generating 4096 tokens on an 80GB H100). As an alternative to pretraining, \name{} outperforms strong pretrained 7B subquadratic LLMs 
    % (RWKV-v6~\citep{peng2024eagle}, Mamba~\citep{gu2023mamba}, Griffin~\citep{de2024griffin}) 
    and hybrids 
    % (StripedHyena~\citep{poli2023hyena}, Zamba~\citep{glorioso2024zamba}) 
    % trained from scratch by 
    % 1.8 to 4.7 pts
    by 1.2--9.9 pts
    (LM Eval avg.).
    % on popular LM Eval tasks.
    
    \item On \textbf{parameter and token-efficiency}, by only training linear attention feature maps in Stage 1, while only using LoRA on linear attention projections in Stage 2, \name{} enables these gains while updating only $<$0.2\% of past linearizing methods' model parameters, making a single 40GB GPU sufficient for 7B LLM linearizing. This also only takes 40M tokens,~\ie{} 0.003\% and 0.04\% of prior pretraining and linearizing methods' token counts.

    \item On \textbf{scalability}, with \name{} we scale up linearizing to support Llama 3.1 70B and 405B LLMs~\citep{dubey2024llama}. \name{} presents the first viable approach to linearizing larger LLMs. We create the first linearized 70B LLM, taking only 18 hours on one 8$\times$80GB H100 node, and the first linearized 405B LLM with  
    a combination of 5 hours on 14 80GB H100 GPUs (attention transfer) +
    16 hours on three 8$\times$80GB H100 nodes (LoRA finetuning) for Llama 3.1 405B. 
    For both models, this amount to under half the total GPU hours than prior methods reported to linearize 8B models (5 days on 8$\times$80GB A100s)~\citep{wang2024mamba}. Furthermore, under these computational constraints, \name{} significantly improves quality versus prior linearizing approaches without attention transfer. With Llama 3.1 70B and 405B, we close 
    77.8\% and 78.1\% of the 5-shot MMLU gap between Transformers and linearized variants respectively.
\end{itemize}

% \noindent Our code is available at: \url{https://github.com/HazyResearch/lolcats}.
\input{sections/figures/pull_results_v3}




==> sections/iclr_2_preliminaries.tex <==
% \section{Preliminaries and Related Work}
% \section{Preliminaries: Building Blocks for Linearizing LLMs}
\vspace{-0.25cm}
\section{Preliminaries}
\label{sec:preliminaries}
\vspace{-0.25cm}
To motivate \name{}, we first go over Transformers, attention, and linear attention. We then briefly discuss related works on linearizing Transformers and Transformer-based LLMs.

\paragraph{Transformers and Attention.}
Popular LLMs such as Llama 3 8B~\citep{llama3modelcard} and Mistral 7B~\citep{jiang2023mistral} are decoder-only Transformers, with repeated blocks of multi-head \textit{softmax attention} followed by MLPs~\citep{vaswani2017attention}.
% 
For one head, attention computes outputs $\bm{y} \in \mathbb{R}^{l \times d}$ from inputs $\bm{x} \in \mathbb{R}^{l \times d}$ (where 
% $h$ is number of heads, 
$l$ is sequence length, 
$d$ is head dimension) with query, key, and value weights $\bm{W}_q, \bm{W}_k, \bm{W}_v \in \mathbb{R}^{d \times d}$. In causal language modeling, we compute $\bm{q} = \bm{x}\bm{W}_q$, $ \bm{k} = \bm{x}\bm{W}_k$, $ \bm{v} = \bm{x}\bm{W}_v$, before getting attention weights $\bm{a}$ and outputs $\bm{y}$ via
% \begin{equation}
%     \mathnormal{
%     \underbrace{
%     a_{n, i} = \frac{\exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})}{\sum_{i=1}^n \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})},
%     \;
%     \bm{y}_n = 
%     \sum_{i=1}^n a_{n, i} \bm{v}_i
%     }_{\text{Softmax Attention}}
%     , \;\;
%     \underbrace{
%     \hat{a}_{n, i} =
%     % \sum_{i=1}^n
%     \frac{ \phi(\bm{q}_n)^\top \phi(\bm{k}_i)}{\sum_{i=1}^n \phi(\bm{q}_n)^\top \phi(\bm{k}_i)},
%     \;
%     \hat{\bm{y}}_n = \sum_{i=1}^n \hat{a}_{i, n} \bm{v}_i
%     }_{\text{Linear Attention}}}
%     % \left)
% \label{eq:attn_matching_setup}
% \end{equation}
\begin{equation}
    a_{n, i} = \frac{\exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})}{\sum_{i=1}^n \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})},
    \;\;\;
    \bm{y}_n = 
    \sum_{i=1}^n a_{n, i} \bm{v}_i,
    \;\;\;
    \text{for $n$ in $[1, \ldots, l]$}
    % \bm{q}_n = \bm{x}_n\bm{W}_q, \bm{k}_i = \bm{x}_i\bm{W}_k, \bm{v}_i = \bm{x}_i\bm{W}_v
\label{eq:causal_attention}
\end{equation}
Multi-head attention maintains inputs, outputs, and weights for each head, \textit{e.g.,} $\bm{x} \in \mathbb{R}^{h \times l \times d}$ or $ \bm{W}_q \in \mathbb{R}^{h \times d \times d}$ ($h$ being number of heads), and computes Eq.~\ref{eq:causal_attention} for each head. In both cases, we compute final outputs by 
concatenating $\bm{y}_n$ across heads, before using output weights $\bm{W}_o \in \mathbb{R}^{hd \times hd}$ to compute $\bm{y}_n\bm{W}_o \in \mathbb{R}^{l \times hd}$.
%
While expressive, causal softmax attention requires all $\{ \bm{k}_i, \bm{v}_i\}_{i \leq n}$ to compute $\bm{y}_n$. 
% For large $n$ or generating many samples in parallel (large batch), 
For long context or large batch settings,
% (\emph{e.g.} in long context or large-batch settings), 
this growing \textit{KV cache} can incur prohibitive memory costs even with state-of-the-art implementations such as FlashAttention~\citep{dao2023flashattention}.
% We thus want to replace attention.

\paragraph{Linear Attention.} To get around this,~\citet{katharopoulos2020transformers} show a similar attention operation, but with \textit{linear} time and \textit{constant} memory over generation length (linear time and space when processing inputs).
% with only a constant-sized ``KV state''. This unlocks constant-memory generation that scales independently of sequence length. 
To see how, note that 
softmax attention's exponential is a kernel function $\mathcal{K}(\bm{q}_n, \bm{k}_i)$, which in general can be expressed as the dot product of feature maps $\phi: \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$. Swapping $\exp(\bm{q}_n^\top \bm{k}_i/\sqrt{d})$ with $\phi(\bm{q}_n)^\top \phi(\bm{k}_i)$ in Eq.~\ref{eq:causal_attention} gives us \emph{linear attention} weights 
% $\hat{a}$
and outputs:
% % $\hat{\bm{y}}$:
% % \begin{equation}
% %     \begin{aligned}
% %         \hat{\bm{y}}_n 
% %         &= 
% %         \sum_{i=1}^n\frac{ \phi(\bm{q}_n)^\top \phi(\bm{k}_i)}{\sum_{i=1}^n \phi(\bm{q}_n)^\top \phi(\bm{k}_i)} 
% %         =
% %         \frac{ \phi(\bm{q}_n)^\top \Big(\sum_{i=1}^n  \phi(\bm{k}_i)\bm{v}_i^\top \Big)}{\phi(\bm{q}_n)^\top \sum_{i=1}^n
% %  \phi(\bm{k}_i)} 
% %     \end{aligned}
% % \end{equation}
% \begin{equation}
%     \hat{a}_{n, i} =
%     % \sum_{i=1}^n
%     \frac{ \phi(\bm{q}_n)^\top \phi(\bm{k}_i)}{\sum_{i=1}^n \phi(\bm{q}_n)^\top \phi(\bm{k}_i)},
%     \;\;\;
%     \hat{\bm{y}}_n = \sum_{i=1}^n \hat{a}_{i, n} \bm{v}_i
% \label{eq:linear_attention}
% \end{equation}
% % While similar in architecture without the softmax, with Eq.~\ref{eq:linear_attention} we can now compute outputs with linear time
% Rearranging terms via matrix product associativity, we get
% via associativity we can now re-express Eq.~\ref{eq:linear_attention} as
\begin{equation}
    \hat{\bm{y}}_n 
    =
    \sum_{i=1}^n \frac{ \phi(\bm{q}_n)^\top \phi(\bm{k}_i)\bm{v}_i}{\sum_{i=1}^n \phi(\bm{q}_n)^\top \phi(\bm{k}_i) } 
    =    
    \frac{ \phi(\bm{q}_n)^\top \Big(\sum_{i=1}^n  \phi(\bm{k}_i)\bm{v}_i^\top \Big)}{\phi(\bm{q}_n)^\top \sum_{i=1}^n
 \phi(\bm{k}_i)}
 % =
 % \frac{\phi(\bm{q}_n)^\top \bm{s}_n}{\phi(\bm{q}_n)^\top \bm{z}_n}
 % \;\;\;\;
\label{eq:linear_attention_2}
\end{equation}
This lets us compute both the numerator $\bm{s}_n = \sum_{i=1}^n \phi(\bm{k}_i)\bm{v}_i^\top$ and denominator $\bm{z}_n = \sum_{i=1}^n \phi(\bm{k}_i)$ as recurrent ``KV states''. With $\bm{s}_0 = \bm{0},\bm{z}_0 = \bm{0}$, we recurrently compute linear attention outputs as
% $\bm{s}_n \in \mathbb{R}^{d \times d'}$ and denominator ``K state'' $\bm{z}_n \in \mathbb{R}^{d}$:
\begin{equation}
\hat{\bm{y}}_n 
= \frac{\phi(\bm{q}_n)^\top \bm{s}_n}{\phi(\bm{q}_n)^\top \bm{z}_n}
\;\;
\text{for}
\;\;
\bm{s}_n = \bm{s}_{n-1} + \phi(\bm{k}_n)\bm{v}_n^\top
% \bm{s}_{n-1} = \sum_{i=1}^{n-1} \phi(\bm{k}_i)\bm{v}_i^\top,
\;\;
\text{and}
\;\;
% \text{and}
% \;\;\;
\bm{z}_n = \bm{z}_{n-1} + \phi(\bm{k}_n)
\;\;\;
% \text{and}
% \;\;\;
% \bm{s}_0 = \bm{0},\;\;\; \bm{z}_0 = \bm{0}
\label{eq:linear_attention_recurrent}
\end{equation}
% and initial values $\bm{s}_0 = \bm{0}, \bm{z}_0 = \bm{0}:
% \begin{aligned}
% \bm{s}_n &= \bm{s}_{n-1} + \phi(\bm{k}_n)\bm{v}_n^\top,\;\;\;
%     \bm{s}_{n-1} = \sum_{i=1}^{n-1} \phi(\bm{k}_i)\bm{v}_i^\top \\
% \bm{z}_n &= \bm{z}_{n-1} + \phi(\bm{k}_n),\;\;\;\;\;\;\;\;
% \bm{z}_{n-1} = \sum_{i=1}^{n-1} \phi(\bm{k}_i)
% \end{aligned}
% \label{eq:linear_attention_recurrent}
% \end{equation}
% for ``KV state'' $\bm{s}_n \in \mathbb{R}^{d \times d'}$ and ``K state'' $\bm{z}_n \in \mathbb{R}^{d}$:
% \begin{equation}
% \begin{aligned}
% \bm{s}_n &= \bm{s}_{n-1} + \phi(\bm{k}_n)\bm{v}_n^\top,\;\;\;
%     \bm{s}_{n-1} = \sum_{i=1}^{n-1} \phi(\bm{k}_i)\bm{v}_i^\top \\
% \bm{z}_n &= \bm{z}_{n-1} + \phi(\bm{k}_n),\;\;\;\;\;\;\;\;
% \bm{z}_{n-1} = \sum_{i=1}^{n-1} \phi(\bm{k}_i)
% \end{aligned}
% \label{eq:linear_attention_recurrent}
% \end{equation}
Eq.~\ref{eq:linear_attention_2} lets us compute attention over an input sequence of length $n$ in $\mathcal{O}(ndd')$ time and space, while Eq.~\ref{eq:linear_attention_recurrent} lets us compute $n$ new tokens in $\mathcal{O}(ndd')$ time and $\mathcal{O}(dd')$ memory.
% for every new token.
Especially during generation, when softmax attention has to compute new tokens sequentially anyway, Eq.~\ref{eq:linear_attention_recurrent} enables time and memory savings if $d' <$ (prompt length + prior generated tokens).

% \simran{Here I wonder if there is anything useful to say around the properties of a good feature map, per the hedgehog work -- since attention matching is a big focus.}
% To combine efficiency with quality, various works propose different $\phi$. These enforce positive affine attention weights~\citep{katharopoulos2020transformers,qin-etal-2022-devil} or approximate $\exp(\cdot)$ via randomized~\citep{choromanski2020rethinking,peng2021random,zheng2022linear}, polynomial~\citep{alman2023fast, keles2023computational}, or learnable features~\citep{kasai-etal-2021-finetuning,mao-2022-fine,zhang2024the}. 
% % Beyond designing $\phi$, other works add decay factors~\citep{schlag2021linear,sun2023retentive} and gating~\citep{yang2023gated}. 

\paragraph{Linearizing Transformers.} 
To combine efficiency with quality, various works propose different $\phi$, (\eg{} $\phi(x) = 1 + \text{ELU}(x)$ as in ~\cite{katharopoulos2020transformers}). However, they typically train linear attention Transformers from scratch. 
% scaling up these layers to 7B+ LLMs remains costly. 
%
% Recent works thus aim to replace softmax attentions of existing LLMs with linear attention. 
%
We build upon recent works that \textit{swap} the softmax attentions of \textit{existing} Transformers with linear attention before finetuning the modified models with next-token prediction to recover language modeling quality. 
%
These include methods proposed for LLMs~\citep{mercat2024linearizing}, and those for smaller Transformers---\textit{e.g.,} 110M BERTs~\citep{devlin2018bert})---reasonably adaptable to modern LLMs~\citep{kasai-etal-2021-finetuning,mao-2022-fine,zhang2024the}.

% In both settings, prior works simply (1) replace the softmax attentions of an existing Transformer with linear attentions---keeping all pretrained weights while introducing feature maps $\phi$ and the alternative computation (Eq.~\ref{eq:linear_attention_2})---before (2) training the modified model end-to-end on a collection of pretraining tokens with a next-token prediction loss. 
% %
% By starting with the pretrained weights of available Transformers, linearizing offers a way to more accessibly scale up subquadratic architectures versus pretraining from scratch. However, while swapping attentions necessarily introduces linear time and constant memory generation, existing methods struggle to recover original LLM quality---\eg{} as measured by general pretrained zero or few-shot language modeling capabilities---while still training billions of parameters on billions of tokens~\citep{mercat2024linearizing}.
% %

% % Next, we describe the \name{} implementation of the specific linearizing LLM architecture and both these linearizing steps.

==> sections/iclr_3_method.tex <==

% \input{sections/figures/pull_method}

\section{Method: Linearizing LLMs with \name{}}
\label{sec:method}
We now study how to build a high-quality and highly efficient linearizing method.
%
In Section~\ref{sec:method_framework}, we present our motivating framework,
which aims to (1) learn good softmax attention approximators with linear attentions and (2) enable low-rank adaptation for recovering linearized quality.
% which simply adapts prior swapping-and-finetuning approaches to (1) learn good softmax attention approximators before (2) only using low-rank adaptation. 
%
In Section~\ref{sec:method_study}, we find that while this attention transfer works surprisingly well for low-rank linearizing with existing linear attentions, on certain tasks, it still results in sizable quality gaps compared to prior methods. 
% To support our motivating hypothesis, 
We also find that attention-transfer quality strongly corresponds with the final linearized model's performance. In Section~\ref{sec:method_new_stuff}, we use our learned findings to overcome prior issues, improving attention transfer to subsequently improve low-rank linearizing quality.

% \vspace{-1cm}
\subsection{\name{} Part 1: A Framework for Low-cost Linearizing}
\label{sec:method_framework}

In this section, we present our initial \name{} framework for linearizing LLMs in an effective yet efficient manner. Our main hypothesis is that by first learning linear attentions that approximate softmax, we can then swap these attentions in as drop-in subquadratic replacements. We would then only need a minimal amount of subsequent training---\eg{} that is supported by low-rank updates---to recover LLM quality in a cost-effective manner effectively. We thus proceed in two steps.

\begin{enumerate}[leftmargin=*]
    \item \textbf{Parameter-Efficient Attention Transfer.} For each softmax attention in an LLM, we aim to learn a closely-approximating linear attention, \ie{} one that computes attention outputs $\hat{\bm{y}} \approx \bm{y}$ for all natural inputs $\bm{x}$. 
    %
    We call this ``attention transfer'', as we aim to \textit{transfer} the attention modeling of existing softmax attentions into target linear attentions. Due to architectural similarity,
    %
    we can treat this as a feature map learning problem, learning $\phi$ to approximate softmax. For each head and layer, let $\phi_q$ and $ \phi_k$ be query and key feature maps. Per head, we compute:
    \begin{equation}
        \bm{y}_n = \underbrace{
    % \bm{y}_n = 
    \sum_{i=1}^n \frac{ \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})}{\sum_{i=1}^n \exp(\bm{q}_n^\top \bm{k}_i  / \sqrt{d} )} \bm{v}_i
    }_{\text{Softmax Attention}},\;\;\;\;
    \hat{\bm{y}}_n = 
    \underbrace{
    % \hat{\bm{y}}_n = 
    \sum_{i=1}^n \frac{ \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i)}{\sum_{i=1}^n \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i) } \bm{v}_i
    }_{\text{Linear Attention}}
    \end{equation}
    for all $n \in [l]$ with input $\in \mathbb{R}^{l \times d}$,
    and train $\phi_q, \phi_k$ to minimize sample mean squared error (MSE)
    \begin{equation}
    % \begin{align}
        \ell_\text{MSE} = \frac{1}{MH}\sum_{m = 1}^M \sum_{h=1}^H
        \ell_\text{MSE}^{h, m}\;\;,\;\;\;\; 
        \ell_\text{MSE}^{h, m} = \frac{1}{d} \sum_{n=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2
    % \end{align}
        \label{eq:mse_loss}
    \end{equation}
    \ie{} jointly for each head $h$ in layer $m$.
    Similar to past work~\citep{kasai-etal-2021-finetuning,zhang2024the}, rather than manually design $\phi$, we parameterize each $\phi : \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$ as a \textit{learnable} layer:
    % followed by a nonlinear activation,~\ie{} 
    \[
    \phi_q(\bm{q}_n) := f(\bm{q}_n\tilde{\bm{W}}_{(q)} + \tilde{\bm{b}}_{(q)}),\;\;\;
    \phi_k(\bm{k}_i) := f(\bm{k}_i\tilde{\bm{W}}_{(k)} + \tilde{\bm{b}}_{(k)})
    \]
    Here $\tilde{\bm{W}} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}} \in \mathbb{R}^{d'}$ are trainable weights and optional biases, 
    $f(\cdot)$ is a nonlinear activation, and $d'$ is an arbitrary feature dimension (set to equal head dimension $d$ in practice).
% To train $\phi$, we simply sample layer-wise ($\bm{x},\bm{y}$) as pretrained attention inputs and outputs, computed with our target LLM's inference over natural language samples (Fig.~\ref{}). We train all $\phi$ jointly to minimize Eq.~\ref{eq:attn_matching_setup} with outputs ($\hat{\bm{y}},\bm{y}$) (see App.~\ref{} for training code and implementation details, with more discussion on advantages over related work~\citep{zhang2024the} that supervises with all attention weights ($\hat{\bm{a}},\bm{a}$)).
% % (Fig.~\ref{}; training code and implementation details in App.~\ref{}). Rather than supervise with the attention weights~\citep{zhang2024the}, we also just use outputs to train directly to minimize Eq.~\ref{eq:attn_matching_setup}. This lets us avoid prior   
% Finally, in general we can use any linear attention with learnable $\phi$. To develop \name{} we explore several options that vary in $f(\cdot)$ from prior work. 

% \vspace{0.2cm}

\item \textbf{Low-rank Adjusting.} After training the linearizing layers, we replace the full-parameter training of prior work with low-rank adaptation (LoRA)~\citep{hu2021lora}. 
%
Like prior work, to adjust for the modifying layers and recover language modeling quality, we now train the modified LLM end-to-end over tokens to minimize a sample next-token prediction loss
% over some sample data $\bm{u}$ with a 
% \begin{equation}
\(
\ell_\text{xent} = -\sum \log P_\Theta(\bm{u}_{t+1} \mid \bm{u}_{1:t})
\).
% \label{eq:cross_entropy_loss}
% \end{equation}
%
Here $P_\Theta$ is the modified LLM, $\Theta$ is the set of LLM parameters, and we aim to maximize the probability of true $\bm{u}_{t+1}$ given past tokens $\bm{u}_{1:t}$ (Fig.~\ref{fig:pull_method}~right). 
However, rather than train all LLM parameters, we only train the swapped linear attention $\bm{W}_q, \bm{W}_k, \bm{W}_v, \bm{W}_o$ with LoRA, 
% for parameter-efficiency we only train the query, key, value, and output projections  of the swapped linear attention layers with LoRA. 
updating $\bm{W}' \leftarrow \bm{W} + \Delta \bm{W}$ with $\Delta \bm{W}$
as the product of two low-rank matrices $\bm{B}\bm{A}$, $\bm{B} \in \mathbb{R}^{d \times r}$, $\bm{A} \in \mathbb{R}^{r \times d}$. 
% We then jointly train all layers 
This enables parameter efficiency for 
% (\eg{} updating only 0.2\% of a 7B+ LLM's parameters), 
$r \ll d$. 
\end{enumerate}

\textbf{Training footprint and efficiency}. Both steps remain parameter-efficient.
    For Step 1, optimizing Eq.~\ref{eq:mse_loss} is similar to a layer-by-layer cross-architecture distillation. We compute layer-wise ($\bm{x}, \bm{y}$) as pretrained attention inputs and outputs, using an LLM forward pass over natural language samples (Fig.~\ref{fig:pull_method} middle).
    %
    However, to keep our training footprint low, we freeze the original pretrained attention layer's parameters and 
    % initializing new linear attention layers (or models). We 
    simply \textit{insert} new $\phi_q, \phi_k$ after $\bm{W}_q, \bm{W}_k$ in each softmax attention (Fig.~\ref{fig:pull_method} left). We compute outputs $\bm{y},\hat{\bm{y}}$ with the same attention weights in separate passes (choosing either Eq.~\ref{eq:causal_attention} or Eq.~\ref{eq:linear_attention_2}; ``teacher-forcing'' by only sending softmax outputs $\bm{y}$ to future layers and preventing error propagation, Fig.~\ref{fig:pull_method} middle). 
    %
    % By jointly training each head and layer, we make attention transfer 
    %
    For Llama 3 8B or Mistral 7B, training $\phi_q,\phi_k$ with $d' = 64$ then only takes 32 layers $\times$ 32 heads $\times$ 2 feature maps $\times$ (128 $\times$ 64) weights $\approx$ 16.8M trainable weights (0.2\% of LLM sizes). 
    %
    Furthermore, Eq.~\ref{eq:mse_loss} keeps attention transfer memory-efficient. While \cite{zhang2024the} also train layer-wise $\phi$ to approximate softmax attention, they supervise by matching on the $n^2$ \textit{attention weights}  computed for $n$-token inputs (App.~\ref{appendix:related_work}, Eq.~\ref{eq:hedgehog_loss}). This scales poorly for large $n$. Instead, by only needing attention outputs, we can reduce memory from $\mathcal{O}(n^2)$ to $\mathcal{O}(n)$, computing softmax attention $\bm{y}$ with FlashAttention~\citep{dao2022flashattention, dao2023flashattention} 
    % for $\bm{y}$ 
    and 
    linear attention $\hat{\bm{y}}$ with Eq.~\ref{eq:linear_attention_2} (or~\ref{eq:hybrid_linear_swa}) both in $\mathcal{O}(n)$ memory by not materializing attention weights. Despite these savings, we show similar attention weight recovery in App.~\ref{app:artifacts_attention_weights}.
    %
    In Step 2, LoRA with $r=8$ on all attention projections suffices for state-of-the-art quality. This updates just $<$0.09\% of 7B parameters.
    % \yell{Also compare to prior linearizing methods in percent of weights changed?}

% For both attention transfer and low-rank linearizing, our key hypothesis is that we can find sufficient linear attention implementations, such that by \emph{training} to minimize Eq.~\ref{eq:attn_matching_setup} over sample data (``attention transfer''), we can learn close enough softmax approximations over natural LLM attention inputs. Then, even if these are not perfect drop-in replacements, we only need minimal amounts of attention weight training---\ie{} that coverable by LoRA with low $r$---to adjust and recover quality. 
% %
% Furthermore, by focusing our training over linearizing data to recover attention sequence modeling patterns, instead of relearning pretrained knowledge, we hypothesize that if \name{} suffices to recover zero-shot LLM abilities, it should also be more token-efficient than full-parameter methods.
% % (our first stage only trains $\bm{q},\bm{k}$ interactions), 


\subsection{Baseline Study: Attention Transfer and Low-rank Linearizing}
\label{sec:method_study}

As a first step, we aim to understand if attention transfer and low-rank adjusting as proposed are sufficient for linearizing LLMs. 
While simple,
it is unclear whether these steps can lead to high-quality linearizing, as all 
% While intuitive, 
prior works default to more involved approaches~\citep{mercat2024linearizing,bick2024transformers,wang2024mamba}. They use linearizing layers featuring GroupNorms~\citep{wu2018group} and decay factors~\citep{sun2023retentive}, or alternate SSM-based architectures~\citep{gu2023mamba,dao2024transformers}. They also all use full-LLM training after swapping in the subquadratic layers. 
%
In contrast, as a first contribution we find that simple linear attentions \textit{can} lead to viable linearizing, with attention transfer + LoRA obtaining competitive quality on 4~/~6 popular LM Eval tasks. 

\begin{wraptable}{r}{0.5\textwidth}  % 'r' for right, width 40% of text width
\vspace{-0.35cm}
\centering
\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{2pt}
\begin{tabular}{@{}lcl@{}}
\toprule
Feature Map              & $\phi(\bm{q})$ (same for $\bm{k}$) & Weight Shapes     \\ \midrule
T2R  & $\text{ReLU}(\bm{q}\tilde{\bm{W}} + \tilde{\bm{b}})$ & 
% $\tilde{\bm{W}} \in \mathbb{R}^{128 \times 128}, \tilde{\bm{b}} \in \mathbb{R}^{128}$ \\
$\tilde{\bm{W}}$: (128, 128), $\tilde{\bm{b}}$: (128,) \\
Hedgehog               & $[\text{SM}_d(\bm{q}\tilde{\bm{W})} \oplus \text{SM}_d(-\bm{q}\tilde{\bm{W})} ]$ &
% $\tilde{\bm{W}} \in \mathbb{R}^{128 \times 64}$ 
$\tilde{\bm{W}}: (128, 64)$ 
\\ \bottomrule
\end{tabular}
}
\vspace{-0.25cm}
\caption{\small \textbf{Learnable feature maps}. Transformer to RNN (T2R) from~\cite{kasai-etal-2021-finetuning}, Hedgehog from~\cite{zhang2024the}, both $\oplus$ (concat) and $\text{SM}_d$ (softmax) apply over feature dimension.}
\label{table:linear_attentions_def}
\vspace{-0.35cm}
\end{wraptable}

\paragraph{Experimental Setup.} We test the \name{} framework by linearizing two popular base LLMs, Llama 3 8B~\citep{AI_2024} and Mistral 7B v0.1~\citep{jiang2023mistral}. For linearizing layers, we study two feature maps used in prior work 
(Table~\ref{table:linear_attentions_def}). 
To support the rotary positional embeddings (RoPE)~\citep{su2024roformer} in these LLMs, we apply the feature maps $\phi$ after RoPE,\footnote{
Unlike prior works that apply $\phi$ before RoPE~\citep{mercat2024linearizing, su2024roformer}, our choice preserves the linear attention kernel connection, where we can hope to learn $\phi_q, \phi_k$ for $\exp(\bm{q}_n^\top \bm{k}_i/\sqrt{d}) \approx \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i)$. 
}
\ie{} computing query features $\phi_q(\bm{q}) = f(\text{RoPE}(\bm{q})\tilde{\bm{W}}_q + \tilde{\bm{b}}))$.
%
For linearizing data, we wish to see if \name{} with a small amount of data can recover general zero-shot and instruction-following LLM abilities. We use the 50K samples of a cleaned Alpaca dataset\footnote{\url{https://huggingface.co/datasets/yahma/alpaca-cleaned}}, due to its ability to improve general instruction-following in 7B LLMs despite its relatively small size~\citep{alpaca}. 
% Following~\cite{zhang2024the}, 
We train all feature maps jointly. 
% where layer-wise distillation is similar to finetuning a single model 
Training code and implementation details are in App.~\ref{appendix:implementation_details}.
%

To study the effects of attention transfer and low-rank linearizing across LLMs and linear attention architectures, we evaluate their validation set perplexity (Table~\ref{table:train_efficiency}, Fig.~\ref{fig:train_efficiency}) and downstream LM Eval zero-shot quality (Table~\ref{table:prelim_mmlu}).
% , (also including sample generations in App.~\ref{}). 
We use the same data for both stages, early stopping, and either 2 epochs for attention transfer and LoRA adjusting or 4 epochs for either alone ($\approx$~40M total training tokens). We use LoRA $r=8$ by popular default~\citep{hu2021lora}, training 0.2\% of LLM parameter counts. 
% We defer additional training details to App.~\ref{}.

\begin{table}[h]
\vspace{-0.25cm}
\begin{center}
\resizebox{0.96\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
& \multicolumn{4}{c}{Llama 3 8B}                                  & \multicolumn{4}{c}{Mistral 7B}                                  \\ 
% \cmidrule(lr){1-1}
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
  \multicolumn{1}{c}{Attention}                       & \multicolumn{2}{c}{T2R}        & \multicolumn{2}{c}{Hedgehog}   & \multicolumn{2}{c}{T2R}        & \multicolumn{2}{c}{Hedgehog}   \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
\multicolumn{1}{c}{Transfer?} & \cellcolor[HTML]{ECF4FF} PPL@0      &  PPL@2/4     & \cellcolor[HTML]{ECF4FF} PPL@0      &  PPL@2/4       & \cellcolor[HTML]{FFDECA}  PPL@0      &  PPL@2/4      & \cellcolor[HTML]{FFDECA} PPL@0      &  PPL@2/4     \\ 
\cmidrule(lr){1-1}
\cmidrule(lr){2-3}\cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
No\; \xmark               & \cellcolor[HTML]{ECF4FF} 1539.39        &  16.05         & \cellcolor[HTML]{ECF4FF} 2448.01        &  9.02          & \cellcolor[HTML]{FFDECA} 2497.13        &  8.85          & \cellcolor[HTML]{FFDECA} 561.47         &  4.87          \\
Yes\; \cmark               & \cellcolor[HTML]{ECF4FF} \textbf{79.33} & \textbf{4.11} & \cellcolor[HTML]{ECF4FF} \textbf{60.86} &  \textbf{3.90} & \cellcolor[HTML]{FFDECA} \textbf{32.78} &  \textbf{3.29} & \cellcolor[HTML]{FFDECA} \textbf{18.94} &  \textbf{3.04} \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-0.25cm}
\caption{\small Alpaca validation set perplexity (PPL) of linearized LLMs, comparing attention transfer, no LoRA adjusting (PPL@0) and PPL after training (PPL@2/4; 2 with attention transfer, 4 without, for equal total steps).
}
\label{table:train_efficiency}
\vspace{-0.25cm}
\end{table}
\input{sections/figures/method_attn_transfer_curves}
% }

\paragraph{Attention Transfer + LoRA Enables Fast LLM Linearizing.} In Table~\ref{table:train_efficiency} and Fig.~\ref{fig:train_efficiency}, we report the validation PPL of linearized LLMs, ablating attention transfer and LoRA adjusting. We find that while attention transfer alone is often insufficient (\textit{c.f.,} PPL@0, Table~\ref{table:train_efficiency}), a single low-rank update rapidly recovers performance by 15--75 PPL (Fig.~\ref{fig:train_efficiency}), 
where training to approximate softmax leads to up to 11.9 lower PPL than no attention transfer.
% achieves \textcolor{red}{17.3} lower perplexity (PPL) than prior analogs trained with 40M tokens (\textcolor{red}{2.7 versus 20.1 PPL}).
% showing viable 7B LLM linearizing at orders of magnitude less training costs than previously shown.
% With the latter taking 5,000$\times$ the tokens, we find we can viably linearize 7B LLMs at magnitudes smaller training costs than previously shown. 
%
Somewhat surprisingly, this translates to performing competitively with prior linearizing methods that train \textit{all} model parameters~\citep{mercat2024linearizing,wang2024mamba} (within 5 accuracy points on 4~/~6 popular LM Eval tasks; Table~\ref{table:prelim_mmlu}), while \textit{only} training with 0.04$\%$ of their token counts and 0.2\% of their parameter counts. The results suggest we can linearize 7B LLMs at orders-of-magnitude less training costs than previously shown.

\input{sections/figures/method_train_efficiency}

\input{sections/figures/method_problems_llama3}

% the combination of attention transfer and LoRA adjusting consistently achieves best linearized quality. 
% %
% Furthermore, in Fig.~\ref{fig:train_efficiency} we find attention transfer enables rapid recovery in language modeling quality, where a single low-rank update reduces PPL by $\sim$15--75 points.
% %
% Considering zero-shot capability recovery, in Table~\ref{table:prelim_mmlu} we find the better performing Hedgehog LLMs remain competitive on 4~/~6 popular LM Eval tasks (within 5 points of contemporary methods). This is despite only training on 0.04$\%$ of other methods' token counts, and updating $<$0.02\% of their parameter counts. Finally, in Fig.~\ref{fig:mse_vs_ppl} we find that attention matching (via MSE; averaged over all heads and layers) strongly corresponds with better linearized model quality (lower PPL).

\paragraph{\textsc{LoL SAD}: Limitations of Low-Rank Linearizing.} At the same time, we note quality limitations with the present framework. 
%
While sometimes close, low-rank linearized LLMs perform worse than full-parameter alternatives and original Transformers on 5~/~6 LM Eval tasks (up to 42.4 points on 5-shot MMLU; Table~\ref{table:prelim_mmlu}). 
To understand the issue, we study if the attention transfer stage can produce close linear attention approximations of LLM softmax attentions. We note 
% four 
three
observations:
\begin{enumerate}[leftmargin=*]
    \item Attention transfer quality (via output MSE) strongly ties to final linearized LLM quality (via PPL) (Fig.~\ref{fig:mse_vs_ppl}), suggesting we can improve quality by reducing MSE with softmax attentions.
    \item However, larger MSEs coincide with lower softmax attention weight entropies (Fig.~\ref{fig:mse_error_llama3_entropy}). 
    ~\cite{zhang2024the} find  linear attentions struggle to approximate such ``spikier'' distributions, suggesting we may need better attention-matching layers
    % ---or some softmax attention---
    to reduce MSE and improve final linearized quality.
    \item When training layers jointly like in prior work~\citep{zhang2024the}, larger MSEs also heavily concentrate in later layers (Fig.~\ref{fig:mse_error_llama3_layer}). To bring the MSE in these layers down, we may thus need more fine-grained layer-wise supervision, rather than the objective over all layers in Eq.~\ref{eq:mse_loss}.
\end{enumerate}

\subsection{\name{} Part 2: Components to Improve Low-rank Linearizing}
\label{sec:method_new_stuff}
% \textcolor{blue}{
% \begin{itemize}
%     \item Figure with SWA + linear (MSEs)
%     \item Figure with the attention transfer -- training-wise
%     \item Cost model
% \end{itemize}
% }
Following our motivating hypotheses, framework, and observations, we now introduce two simple improvements to improve linearized LLM quality by reducing MSE: (1) better attention-matching architectures (\Cref{sec:method_analogs}), and (2) finer-grained layer-wise attention transfer (\Cref{sec:method_training}).

% We now introduce two simple improvements in architecture (\Cref{sec:method_analogs}) and linearizing procedure (\Cref{sec:method_training}) to improve low-rank linearizing quality. 
% We focus on these linearizing components in this work but also include additional experiments on data selection in App~\ref{}.

\input{sections/figures/method_attn_mse}

% \vspace{-0.5cm}
\subsubsection{Architecture: Generalizing Learnable Linear Attentions}
% \vspace{-0.125cm}
% \subsubsection{Architecture: Expanding Learnable $\phi$ Parameterizations}
\label{sec:method_analogs}
% \paragraph{Expanding Learnable $\bm{\phi}$ Parameterizations.} 
As described, we can apply our framework with any linear attentions with learnable $\phi$ (\textit{e.g.}, T2R and Hedgehog, Figure~\ref{fig:train_efficiency}). 
% In our method development, we evaluate two learnable $\phi$ parameterizations. First, we consider the pure linear attention setup discussed above, evaluating how the T2R and Hedgehog activations transfer to our \name{} setting in Section~\ref{}.
%
However, to improve attention-matching quality, we introduce a hybrid $\phi$ parameterization combining linear attention and \textit{sliding window} attention. Motivated by prior works that show quality improvements when combining attention layers with linear attentions~\citep{arora2024simple,Munkhdalai2024-kx}, 
% recurrences~\citep{de2024griffin}, and state-space models~\citep{fu2022hungry,stripedhyena,lieber2024jamba}, 
we combine \textcolor{blue}{short sliding windows} of softmax attention~\citep{beltagy2020longformer,zhu2021long} (size 64 in experiments) followed by linear attention in a single layer. This allows attending to all prior tokens for each layer while keeping the entire LLM subquadratic. For window size $w$ and token indices $[1, \ldots, n-w, \ldots, n]$, we apply the softmax attention over the $w$ most recent tokens, 
and compute attention outputs $\hat{\bm{y}}_n$ as
% \begin{equation}
%     \hat{\bm{y}}_n =  
%     \frac{ \textcolor{blue}{\sum_{i=n-w+1}^n \gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)\bm{v}_i} + \textcolor{cyan}{\phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)\bm{v}_j^\top \big)}}{ \textcolor{blue}{\sum_{i = {n-w+1}}^n\gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)}\; +  \textcolor{cyan}{\phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)^\top \big)}} 
% \label{eq:hybrid_linear_swa}
% \end{equation}
\begin{equation}
    \hat{\bm{y}}_n =  
    \frac{ \textcolor{blue}{\sum_{i=n-w+1}^n \gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)\bm{v}_i} + \phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)\bm{v}_j^\top \big)}{ \textcolor{blue}{\sum_{i = {n-w+1}}^n\gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)}\; +  \phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)^\top \big)} 
\label{eq:hybrid_linear_swa}
\end{equation}
$\gamma$ is a learnable mixing term, and $\bm{c}_n$ is a stabilizing constant as in log-sum-exp calculations ($\bm{c}_n = \max_i\big\{\bm{q}_n^\top \bm{k}_i / \sqrt{d} : i \in [n-w+1, \ldots, n]\big\}$).
Like before, we can pick any learnable $\phi$.

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/mse_analogs_llama3_8b_serif.png}
%         % \vspace{-0.5cm}
%         \caption{Llama 3 8B}
%         \label{fig:mse_analogs_llama3}
%     \end{subfigure}
%     % \hfill
%     \begin{subfigure}[b]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/mse_analogs_mistral_7b_serif.png}
%         \caption{Mistral 7B (v0.1)}
%         \label{fig:mse_analogs_mistral7b}
%     \end{subfigure}
%     \vspace{-0.25cm}
%     \caption{\textbf{Attention matching MSE}. Across LLMs, linearizing with hybrid linear attention + sliding window better approximates ``ground-truth'' softmax attentions via lower MSE over layers.}
%     \label{fig:mse_analogs}
%     \vspace{-0.25cm}
% \end{figure}

\paragraph{Subquadratic efficiency.} The hybrid layer retains linear time and constant memory generation. For $n$-token prompts, we initially require $\mathcal{O}(w^2 d)$ and $\mathcal{O}((n-w)dd')$ time and space for window and linear attention respectively, attending over a $w$-sized KV-cache and computing KV and K-states (Eq.~\ref{eq:linear_attention_recurrent}). 
For generation, we only need $\mathcal{O}(w^2 d + dd')$ time and space for every token. We evict the KV-cache's first $\bm{k}$, $\bm{v}$, compute $\phi_k(\bm{k})$, and add $\phi_k(\bm{k})\bm{v}^\top$ and  $\phi_k(\bm{k})$ to KV and K-states respectively.

\paragraph{Hardware-aware implementation.} To make Eq.~\ref{eq:hybrid_linear_swa} competitive with modern softmax attentions like FlashAttention-2~\citep{dao2023flashattention}, we provide a ``hardware-aware'' Eq.~\ref{eq:hybrid_linear_swa} with the Hedgehog feature map. For space, we defer implementation details to App.~\ref{appendix:experimental_details},~\ref{app:tk_implementation}. We evaluate this version by default. 

% \vspace{-0.5cm}
\subsubsection{Training: Layer (or Block)-wise Attention Transfer}
\label{sec:method_training}
% We describe the \name{} training approach and provide a simplified model to show its cost-quality tradeoffs.
We describe our training approach and provide a simplified model to show its cost-quality tradeoffs.
%
% We modify the training objective in Eq.~\ref{eq:mse_loss} as follows. 
Based on the layer-wise MSE differences in Sec.~\ref{sec:method_study} from training all layers jointly (Eq.~\ref{eq:mse_loss}),
% (Eq.~\ref{eq:mse_loss}) over all $m \in [M]$ for an $M$ layer model, 
we instead generalize to training over finer-grained $b$-layer blocks, and train each block independently:
% Based on the limitations of low-rank linearizing identified in the prior section, we perform attention transfer at a block-by-block granularity for the large scale models. The MSE loss function is scale-sensitive and our study showed that the later layers consistently result in larger MSEs  (Fig.~\ref{fig:mse_error_llama3_layer}).
% Thus, instead of computing the training loss (Eq.~\ref{eq:mse_loss}) over
% all $m \in [M]$ for a model with $M$ layers, we compute the loss over $k$-layer blocks, and train each block independently:
% \begin{equation}
%     \ell_\text{MSE}(\bm{y}, \hat{\bm{y}}) =  \sum_{n=1}^{L} \frac{1}{d}\sum_{j=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2 \rightarrow \ell_\text{MSE}(\bm{y}, \hat{\bm{y}}) = \sum_{n=i}^{i+k} \frac{1}{d}  \sum_{j=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2 
%     \label{eq:mse_loss_blocks}
% \end{equation}
\begin{equation}
    % \begin{align}
        \ell_\text{MSE}^{\text{block}} = \frac{1}{bH}\sum_{m = i}^{i + b} \sum_{h=1}^H
        \ell_\text{MSE}^{h, m}\;\;\;\; 
        % \ell_\text{MSE}^{h, m} = \frac{1}{d} \sum_{n=1}^d (\bm{y}_n - \hat{\bm{y}}_n)^2,\;\;\;\; 
        (\text{for blocks starting at layers } i = 0, b, 2b, \ldots)
    % \end{align}
        \label{eq:mse_loss_blocks}
    \end{equation}
We choose $b$ to balance quality and cost in both memory and training time, which we find particularly helpful for linearizing larger LLMs. Several block-wise training approaches exist,
including joint training with separate optimizer groups per block, sequentially training separate blocks, or precomputing hidden states and training blocks in parallel across GPUs. For space, we report results on LLM quality trade-offs in App.~\ref{app:blockwise_study}, where we find smaller $b$ improves \name{} Llama 3.1 405B PPL by 1.02 points (Table~\ref{table:block_wise_ppl}). Below we discuss primary cost trade-offs:
\begin{itemize}[leftmargin=*]
    \item \textbf{Compute}: 
    % Large block sizes, $k$, require more compute to train each block. 
    While the joint training of Llama 3.1 405B in 16-bit precision uses \textit{multiple nodes} (e.g., NVIDIA H100 8$ \times$80GB nodes), an individual block of $b=9$ or fewer layers can be trained on a \textit{single GPU} (e.g., H100 80GB GPU) at sequence length 1024. 
    % The block-wise approach is also amenable to using a different training duration (and training data) per block.
    \item \textbf{Time}: However, doing so on a single GPU multiples total training time by $M / b$. With multiple GPUs, we can distribute training different blocks on difference devices in parallel. To train blocks at layers $b, 2b, ...$, we need the outputs from each prior block. 
    % to disk. 
    As we teacher-force with the ``true'' softmax attention outputs, we can simply precompute these with the original Transformer.
    \item \textbf{Memory}: Lastly, we need to save each precomputed block's outputs 
    % hidden states 
    to disk.
    The total disk space required is 
\(
2 \times T \times d \times \frac{L}{k}
\)
for total training tokens $T$, model dimension $d$, number of layers $L$ and 2-byte (16-bit) precision. 
For Llama 3.1 405B, saving states per-layer ($b=1$) for just 50M tokens requires over 200TB of disk space. Larger $b$ divides this storage, potentially at the cost of quality.
% ~\eg{} $b=9$ cuts by 14$\times$.

% while $k=126$ (joint training) requires no additional disk space for the states.
% Meanwhile, we do not need to save any hidden states for the joint training approach. 
% Sequentially saving the outputs and training the blocks increases total training time.  
% and effort. 
\end{itemize}
For each target LLM, we thus aim to make low-rank linearizing feasible by first doing block-wise attention transfer, adjusting parameters based on linearizing quality and what is feasible in compute, time, and memory. We summarize \name{} with Alg.~\ref{alg:lolcats_stage_1},~\ref{alg:lolcats_stage_2}, providing pseudocode in App.~\ref{appendix:code}.
% and training details in App.~\ref{app:experimenta_details_linearizing_7b},~\ref{app:experimenta_details_linearizing_70b},~\ref{app:experimenta_details_linearizing_405b}.

% where the training data for the block starting at layer $i$ is the hidden states outputted by prior block starting at layer $i-b$, for each sequence in the training corpus. After attention transfer, we arrange the blocks back together in their original order. Like before, we then do end-to-end LoRA finetuning to recover quality.
% % using an end-to-end LoRA fine-tuning stage. 

% \begin{wraptable}{r}{0.24\textwidth}  % 'r' for right, width 40% of text width
% \vspace{-0.5cm}
% \centering
% \resizebox{1\linewidth}{!}{
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{@{}lcl@{}}
% \toprule
% Method              &  $k \times c$  &  PPL\\ \midrule
% Joint          &  126$\times$1  & 4.23 \\
% Block-wise      &  9$\times$14  & 3.21
% \\ \bottomrule
% \end{tabular}
% }
% \vspace{-0.125cm}
% \caption{\small \textbf{Attention transfer} for Llama 3.1 405B using $c$ blocks of $k$ layers.}
% \label{table:block_wise_ppl}
% \vspace{-5mm}
% \end{wraptable}

% \paragraph{Tradeoffs between quality and efficiency.} We show that the block-wise approach improves linearization quality at large model scales and improves the user's ability to flexibly balance compute and memory efficiency tradeoffs. We compare (1) \textbf{joint ($k=126$)} training, where we load the full model once and compute the loss as the sum of layer-wise MSEs, and (2) \textbf{block-wise ($k=9$)} training, where we break the model into blocks and train each independently.

% For quality, we compare the evaluation perplexity of both the attention transfer approaches, after LoRA fine-tuning on the same subset of RedPajama data. The block-wise and joint approaches perform similarly at the 8B and 70B scales, however, as shown in Table~\ref{table:block_wise_ppl}, the block-wise approach performs 1.02 points better than joint attention transfer at the 405B scale. These results support our study in Section~\ref{sec:method_study}, which shows the  variation in MSE magnitudes grows large at the 405B scale. 
% % To understand why block-wise helps for the largest models, 
% % Finer grained block-wise supervision appears to help handle this variation.
% % These results emphasize that the large MSEs may warrant finer-grained supervision during attention transfer.

% \begin{algorithm}[H]
% \scriptsize 
% \caption{\name{} Step 1: Attn. Transfer}
% \label{alg:lolcats_stage_1_and_2}
% \begin{algorithmic}[1]
% \Require{Transformer with $M$ attention layers}
% \Require{Linear attn.~feature map params.~$\{\phi_q^m, \phi_k^m, \gamma^m : m \in [M]\}$, window size $w$, layer block-size $b$, learning rate $\alpha$}
% % \Require{Training token input $x$}
% % \Ensure{\name{} attention output $\bm{o} \in \mathbb{R}^{N \times d}$}
%     % \Statex Let $\mathbf{local}_{KV}$ be the cumulative recurrent state (``KV-state'') initialized to $0$ in waprgroup 2's registers.
%     \State Freeze all Transformer parameters
%     \State \textbf{Initialize} block-wise losses $\{\ell_i \gets 0 : i \in [M /\!\!/ b] \}$ 
%     % \Comment Step 1: Attention Transfer
%     \For{input token {$\bm{u}$}}
%         \State Compute initial attn. input $\bm{x}_1 \gets \texttt{embed}(\bm{u})$
%         \For{attn. layer {$m \in [M]$}}  \Comment Compute attentions
%     % \State \textbf{Initialize} feature maps $\phi_q$ and $\phi_k$ for each attention head {$h \in [H]$}
%     % \State Assign $\phi_q, \phi_k$ to optimizer $m /\!\!/ k $ 
%             \State $\bm{q}_m,\bm{k}_m,\bm{v}_m = \texttt{qkv\_proj}_m(\bm{x}_m)$
%             \State $\bm{y}_m = \texttt{softmax\_attn}(\bm{q}_m,\bm{k}_m,\bm{v}_m)$ (Eq.~\ref{eq:causal_attention})
%             \State $\hat{\bm{y}}_m = \texttt{linear\_attn}(\bm{q}_m,\bm{k}_m,\bm{v}_m, w, \phi_q^m, \phi_k^m, \gamma^m)$ (Eq.~\ref{eq:hybrid_linear_swa})
%             \State $\ell_{m/\!\!/b} \gets \ell_{m/\!\!/b} + \ell_{\text{MSE}}(\hat{\bm{y}}_m, \bm{y}_m)$  (Eq.~\ref{eq:mse_loss_blocks})
%             \State $\bm{x}_{m+1} = \texttt{mlp}_m(\texttt{o\_proj}_m(\bm{y}))$ \Comment Next layer input
%         \EndFor
%         \For{attn. layer {$m \in [M]$}} \Comment Update feature maps
%             \For{weights {$\theta \in \{\phi_q^m, \phi_k^m, \gamma^m\}$}}
%                 \State Update $\theta \gets \theta - \alpha \frac{\partial}{ \partial \theta}\ell_{m/\!\!/b}$ 
%             \EndFor
%             % \State $\phi'_{(q,m)} \gets \phi_q^m - \alpha \frac{\partial \ell_{m/\!\!/b}}{ \partial \phi_q^m}$  
%             % \State $\phi'_{(k,m)} \gets \phi_k^m - \alpha \frac{\partial \ell_{m/\!\!/b}}{ \partial \phi_k^m}$
%             % \State $\gamma'_{m} \gets \gamma_{m} - \alpha \frac{\partial \ell_{m/\!\!/b}}{ \partial \gamma^m}$
%         \EndFor
%     \EndFor
% \end{algorithmic}
% \end{algorithm}

\begin{minipage}{0.49\textwidth}
\vspace{-0.5cm}
\begin{algorithm}[H]
\scriptsize 
\caption{\name{} Step 1: Attn. Transfer}
\label{alg:lolcats_stage_1}
\begin{algorithmic}[1]
\Require{Pretrained Transformer with $M$ attn.~layers; input tokens $\bm{u}$}
% \Require{Input tokens $\bm{u}$}
\Require{Linear attn.~feature map params.~$\{\phi_q^m, \phi_k^m, \gamma^m : m \in [M]\}$, window size $w$; layer block-size $b$, learning rate $\alpha$}
    \State Freeze all Transformer parameters
    \State \textbf{Initialize} block-wise losses $\{\ell_i \gets 0 : i \in [M /\!\!/ b] \}$ 
    % \Comment Step 1: Attention Transfer
    % \For{input token {$\bm{u}$}}
    \State Compute initial attn. input $\bm{x}^1 \gets \texttt{embed}(\bm{u})$
    \For{attn. layer {$m \in [M]$}}  \Comment \textbf{Compute attentions}
        % \State $\bm{q},\bm{k},\bm{v} = \texttt{qkv\_proj}_m(\bm{x}^m)$
        \State $\bm{q},\bm{k},\bm{v} = \bm{x}^m\bm{W}_q^m, \bm{x}^m\bm{W}_k^m, 
        \bm{x}^m\bm{W}_v^m$
        \State $\bm{y}^m = \texttt{softmax\_attn}(\bm{q},\bm{k},\bm{v})$ (Eq.~\ref{eq:causal_attention}) \Comment (No grad)
        \State $\hat{\bm{y}}^m = \texttt{linear\_attn}(\bm{q},\bm{k},\bm{v}, w, \phi_q^m, \phi_k^m, \gamma^m)$ \hfill (Eq.~\ref{eq:hybrid_linear_swa})
        \State $\ell_{m/\!\!/b} \gets \ell_{m/\!\!/b} + \ell_{\text{MSE}}(\hat{\bm{y}}^m, \bm{y}^m)$ \hfill (Eq.~\ref{eq:mse_loss_blocks})
        % \State $\bm{x}^{m+1} = \texttt{mlp}_m(\texttt{o\_proj}_m(\bm{y}))$ \Comment \textcolor{blue}{(Next layer input)}
        \State $\bm{x}^{m+1} = \texttt{mlp}^m(\bm{y}^m\bm{W}_o^m)$ \Comment (Teacher-force next layer)
    \EndFor
    \For{attn. layer {$m \in [M]$}} \Comment \textbf{Update feature maps}
        \For{weights {$\theta \in \{\phi_q^m, \phi_k^m, \gamma^m\}$}}
            \State Update $\theta \gets \theta - \alpha \frac{\partial}{ \partial \theta}\ell_{m/\!\!/b}$ 
        \EndFor
    \EndFor
    % \EndFor
\end{algorithmic}
\end{algorithm}
\vspace{-0.5cm}
\end{minipage}
\hfill
\begin{minipage}{0.49\textwidth}
\vspace{-0.5cm}
\begin{algorithm}[H]
\scriptsize 
\caption{\name{} Step 2: LoRA Adjust}
\label{alg:lolcats_stage_2}
\begin{algorithmic}[1]
\Require{\textit{Linearized} Transformer with $M$ attn. layers; input tokens $\bm{u}$}
% \Require{Input tokens $\bm{u}$}
\Require{\textit{Trained} feature map params.~$\{\phi_q^m, \phi_k^m, \gamma^m : m \in [M]\}$, window size $w$; learning rate $\alpha$}
    % \State Freeze all Transformer parameters, including linear attentions
    \For{attn. layer {$m \in [M]$}} \Comment (Add LoRA weights)
        \Statex\;\;\;\; \textbf{Init.}~LoRA $\bm{A}^m, \bm{B}^m$ for each $\bm{W}_q^m,\bm{W}_k^m,\bm{W}_v^m,\bm{W}_o^m$
    \EndFor
    % \State \textbf{Initialize} sample loss $\ell \gets 0$ 
    % \Comment Step 1: Attention Transfer
    % \For{input token {$\bm{u}$}}
    \State Compute initial attn. input $\bm{x}^1 \gets \texttt{embed}(\bm{u})$
    \For{attn. layer {$m \in [M]$}}  \Comment \textbf{Compute attentions}
        \State $\bm{q} = \bm{x}^m (\bm{W}_q^m + \bm{B}_q^m\bm{A}_q^m)$ \Comment (LoRA forward pass)
        \State $\bm{k} = \bm{x}^m (\bm{W}_k^m + \bm{B}_k^m\bm{A_k}^m)$
        \State $\bm{v} = \bm{x}^m (\bm{W}_v^m + \bm{B}_v^m\bm{A}_v^m)$
        
        \State $\hat{\bm{y}}^m = \texttt{linear\_attn}(\bm{q},\bm{k},\bm{v}, w, \phi_q^m, \phi_k^m, \gamma^m)$ \hfill (Eq.~\ref{eq:hybrid_linear_swa})
        \State $\bm{x}^{m+1} = \texttt{mlp}^m(\bm{y}^m (\bm{W}_o^m + \bm{B}_o^m\bm{A}_o^m))$ 
        % \Comment \textcolor{blue}{(Next layer input)}
    \EndFor
    \State Compute next-token pred $\hat{\bm{u}} = \texttt{lm\_head}(\bm{x}^M)$ \Comment \textbf{Train LoRA}
    \State Compute sample loss $\ell = \ell_{\text{CrossEnt}}(\hat{\bm{u}}_{0:n-1}, \bm{u}_{1:n})$ 
    % \State $\ell \gets \ell + \ell_{\text{CrossEnt}}(\hat{\bm{u}}_{0:n-1}, \bm{u}_{1:n})$ \Comment \textcolor{blue}{\textbf{Update LoRAs}}
    
    % \For{attn. layer {$m \in [M]$}} \Comment \textcolor{blue}{\textbf{Update LoRAs}}
        % \For{weights {$\bm{A},\bm{B}$}}
        %     \State Update $\theta \gets \theta - \alpha \frac{\partial}{ \partial \theta}\ell$ 
        % \EndFor
        \State Update $\theta \gets \theta - \alpha \frac{\partial \ell}{ \partial \theta}$ for all $\theta$ in all $\bm{A},\bm{B}$ 
    % \EndFor
    % \EndFor
\end{algorithmic}
\end{algorithm}
\vspace{-0.5cm}
\end{minipage}




% % Especially at the larger LLM scales (e.g., Llama 3.1 405B), we find that jointly performing attention transfer over all $126$ layers fails to produce high quality LLMs. We observe that the uneven magnitudes in the attention outputs, with later layers consistently carrying larger MSEs than earlier ones, presents a challenge (Figure). Across the 70B and 405B parameter models, we show that setting smaller $k$ leads to improved quality (Table).
% % The primary costs-tradeoffs between these two approaches are:
% Next, for efficiency, we compare the compute and memory use for both methods:
% \begin{itemize}[leftmargin=*]
%     \item Compute: 
%     % Large block sizes, $k$, require more compute to train each block. 
%     While the joint training of Llama 3.1 405B in 16-bit precision uses \textit{multiple nodes} (e.g., NVIDIA H100 8$ \times$80GB nodes), an individual block of $k=9$ or fewer layers can be trained on a \textit{single GPU} (e.g., H100 80GB GPU), at sequence length 1024. The block-wise approach is also amenable to using a different training duration (and training data) per block.
%     \item Memory: To train block $i$, we need to save the hidden states from the prior block to disk. The total amount of disk space required is 
% \(
% 2 \times T \times d \times \frac{L}{k}
% \)
% for total training tokens $T$, model dimension $d$, number of layers $L$ and 2-byte (16-bit) precision. 
% At the Llama 3.1 405B scale, saving states per-layer ($k=1$) for just $50$M tokens would require over 200TB of disk space, while $k=126$ (joint training) requires no additional disk space for the states.
% % Meanwhile, we do not need to save any hidden states for the joint training approach. 
% % Sequentially saving the outputs and training the blocks increases total training time.  
% % and effort. 
% \end{itemize}
% % Finally, decentralized training offers the flexibility to 
% % The flexibility offered by our training procedure may benefit researchers studying sub-quadratic LLMs on an academic budget.
% % the compute required to train each block of $k$ layers and the memory requirement to save hidden outputs of prior blocks as inputs to later ones.  


% % \newpage{}


% % We describe how we distill Llama 3.1 $70$B and Llama $405$B to linearized \name{}s, in 16-bit precision, on an academic budget. 
% % We first evaluate the vanilla \name{} approach used for the $8$Bn parameter models in \Cref{sec:405b_baseline} and then highlight simple extensions enabled by the \name{} framework that provide further  quality and efficiency improvements in \Cref{sec:405b_approach}.
% %
% % All prior work on linearization operates below $10$Bn parameters in model size \cite{}. We demonstrate that \name{} enables the first hundred-billion parameter sub-quadratic model. Furthermore, our procedure requires just $8$ hours of training.  
% %
% % \label{sec:405b_baseline}
% % We first directly apply the vanilla  \name{} approach, which led to state-of-the-art quality at the $8$Bn parameter scale, to the $70$Bn and $405$Bn models. The results are included in \Cref{table:scale_baseline}. 
% %
% % \name{} excitingly achieves X\% of Llama 3.1 70B quality with just X\% of trainable parameters and X\% of the number of pretraining tokens. As in the case of the 8Bn parameter models, the initial attention transfer stage helps improve quality by X points on average. 

% % However, the vanilla approach falls short at the 405Bn parameter scale, both with and without the initial attention transfer stage. Above this, the $16$-bit $405$B model, requiring a total of $810$ GB for the model parameters alone, does not fit in a single $8 \times 80$GB GPU commodity box, requiring expensive multi-node training that is beyond the scope of most academic budgets. 
% % In the next section, we study how to address these limitations and unlock high quality linearized 405Bn parameter models. 
% %
% % \begin{table}[!h]
% % \scriptsize
% % \begin{center}
% % \resizebox{0.96\linewidth}{!}{
% % \begin{tabular}{@{}ccccccccc@{}}
% % & \multicolumn{2}{c}{Llama 3.1 70B}                                  & \multicolumn{2}{c}{Llama 3.1 405B}                                  \\ 
% % \cmidrule(lr){2-5} 
% % % \cmidrule(lr){6-8}
% %   \multicolumn{1}{c}{Attention}                       & 
% %   \multicolumn{2}{c}{Hedgehog}      & \multicolumn{2}{c}{Hedgehog}   \\ 

% % \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% % \multicolumn{1}{c}{Transfer?} & \cellcolor[HTML]{ECF4FF} Start PPL      &  End PPL       & \cellcolor[HTML]{ECF4FF} Start PPL      &  End PPL  \\ 
% % \cmidrule(lr){1-1}
% % \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% % No\; \xmark               & \cellcolor[HTML]{ECF4FF}    &        & \cellcolor[HTML]{ECF4FF}     &    \\
% % Yes\; \cmark               & 
% % \cellcolor[HTML]{ECF4FF} \textbf{} & \textbf{} & \cellcolor[HTML]{ECF4FF} \textbf{} & \textbf{}  \\ 
% % \bottomrule
% % \end{tabular}
% % }
% % \end{center}
% % \vspace{-2mm}
% % \caption{Initial and final perplexities of low-rank linearized LLMs with and without attention transfer at the 70B and 405B parameter scales. 
% % }
% % \label{table:scale_baseline}
% % \vspace{-0.5cm}
% % \end{table}
% %
% % \subsection{Mini \name{} in a trenchcoat}
% % \label{sec:405b_approach}
% % We show how simple extensions to the \name{} approach unlock quality and efficiency in the large scale regime. For this section, recall that Llama 3.1 405B has a model dimension of $16,384$ and $126$ Transformer layers.
% %
% % \paragraph{Finer-grained supervision} Recall that in the vanilla \name{} approach is that the total training loss during the attention transfer stage is the sum of the MSE loss between the true and linearized attention maps at each individual layer. We hypothesize that especially for very deep models, like Llama 405B with 126 Transformer layers, the loss scale may greatly vary across the layers, making it difficult to jointly supervise all layers. The natural next step train for attention transfer at a finer-grained, perhaps layer-by-layer, granularity.
% %
% % \paragraph{Cost Model: Tradeoffs Between Scaled up Quality and Cost.}
% %
% % \paragraph{Tradeoffs between quality and cost}

==> sections/iclr_4_results.tex <==
\section{Experiments}
\label{sec:results}
\vspace{-0.25cm}

Through experiments, we study: (1) if \name{} linearizes LLMs with higher quality than existing subquadratic alternatives and linearizations, and higher generation efficiency than original Transformers (Sec.~\ref{sec:main_results});  (2) how ablations on attention transfer loss, subquadratic architecture, and parameter and token counts impact LLM quality (Sec.~\ref{sec:results_ablations}); and (3) how \name{}' quality and efficiency holds up to 70B and 405B LLMs by linearizing the complete Llama 3.1 family
% where we linearize and compare model quality across the complete Llama 3.1 family 
(Sec.~\ref{sec:chungus_amongus}).

\subsection{Main Results: \name{} Efficiently Recovers Quality in Linearized LLMs}
\label{sec:main_results}
\vspace{-0.125cm}

In our main evaluation, we linearize the popular base Llama 3 8B~\citep{AI_2024} and Mistral 7B~\citep{jiang2023mistral} LLMs. We first test if \name{} can efficiently create high-quality subquadratic LLMs from strong base Transformers, comparing to existing linearized LLMs from prior methods. We also test if \name{} can create subquadratic LLMs that outperform modern Transformer alternatives pretrained from scratch. For space, we defer linearizing training details to Appendix~\ref{appendix:experimental_details}.

\input{sections/tables/main_results_linearize}

\input{sections/tables/main_results_v2_local}

% \paragraph{Natural Language Understanding.} 
In Table~\ref{table:main_results}, we report results on six popular LM Evaluation Harness (LM Eval) tasks~\citep{eval-harness}.
%
Compared to recent linearizing methods, \name{} significantly improves quality and training efficiency across tasks and LLMs. On quality, \name{} closes 
% 73.8\% and 81.1\% 
79.8\% and 86.6\%
of the Transformer-linearizing gap for Mistral 7B and Llama 3 8B respectively, notably improving 5-shot MMLU by 
% 63.8\% and 50\% 
60.9\% and 40.9\% 
over next best fully subquadratic models (17.2 and 9.6 points). On efficiency, we achieve these results while only training $<$0.2\% of model parameters via LoRA versus prior full-parameter training. We also only use 40M tokens versus the prior 20~--~100B (a 500~--~2500$\times$ improvement in ``tokens-to-model'' efficiency).
%
Among all 7B LLMs, \name{}-linearized LLMs further outperform strong subquadratic Transformer alternatives, representing RNNs or linear attentions (RWKV-v6~\citep{peng2024eagle}, Hawk, Griffin~\citep{de2024griffin}, TransNormer~\citep{qin2023scaling}), state-space models (Mamba~\citep{gu2023mamba}), and hybrid architectures with some full attention (StripedHyena~\citep{stripedhyena}, Zamba~\citep{glorioso2024zamba}). 

\vspace{-0.125cm}
\subsection{\name{} Component Properties and Ablations}
\vspace{-0.125cm}
\label{sec:results_ablations}
We next validate that \name{} enables subquadratic efficiency, and study how each of \name{}' components contribute to these quality gains. We include additional ablations in Appendix~\ref{appendix:additional_experiments}.

\input{sections/figures/benchmark_efficiency}

\paragraph{Subquadratic Generation Throughput and Memory.} We measure generation throughput and memory of \name{} LLMs, validating that linearizing LLMs can significantly improve their generation efficiency. We use the popular Llama 3 8B HuggingFace model\footnote{\url{https://huggingface.co/meta-llama/Meta-Llama-3-8B}}, and compare \name{} implemented in HuggingFace Transformers with the supported FlashAttention-2 (FA2)~\citep{dao2023flashattention}. We benchmark \name{} with Hedgehog feature map and linear + sliding window attention in FP32 and BF16 on one 80GB H100.
% In Fig.~\ref{fig:generation_throughput},~\ref{fig:generation_memory},
Fig.~\ref{fig:bm_efficiency} reports scaling batch size on throughput (left) and memory (right). We measure throughput as $($generated tokens $\times$ batch size $/$ total time$)$, with 128-token prompts and 4096-token generations. With larger batch size, \name{}-linearized LLMs achieve higher throughput than FA2. This corresponds with lower memory, where FA2 exceeds memory at batch size 64. Meanwhile, \name{} supports 3000 tokens / second at batch size 2048 
% (Fig.~\ref{fig:generation_throughput}),
(Fig.~\ref{fig:bm_efficiency} left),
 with fixed ``KV state'' vs.~softmax attention's growing KV cache  
% (Fig.~\ref{fig:generation_memory})
(Fig.~\ref{fig:bm_efficiency} right). 

\paragraph{Ablations.}
We study how attention transfer and linear + sliding window attention in \name{} contribute to downstream linearized Llama 3 8B performance  
% over 1024-token long samples 
(Table~\ref{table:main_results_ablations}). We start with prior linear attentions (Hedgehog,~\cite{zhang2024the}; T2R,~\cite{kasai-etal-2021-finetuning}), using the prior linearizing approach that swaps attentions and finetunes the model to predict next tokens~\citep{mercat2024linearizing}. We then add (i) attention transfer, (ii) sliding window attentions, or (iii) both. On average LM Eval score and 5-shot MMLU accuracy, \name{}' default performs best across feature maps.


\input{sections/tables/main_results_ablation_v2}
\vspace{-0.125cm}
\subsection{Scaling Up Linearizing to 70B and 405B LLMs}
\vspace{-0.125cm}
\label{sec:chungus_amongus}
We finally use \name{} to scale up linearizing to Llama 3.1 70B and 405B models. 
%
In Table~\ref{table:chungus_results}, \name{} provides the first practical solution for linearizing larger LLMs, achieving significant quality improvements over prior linearizing approaches of swapping in attentions and finetuning~\citep{mercat2024linearizing}. With the same linear + sliding window layer, \name{} gets +39.0 points in 5-shot MMLU accuracy on Llama 3.1 70B, and +38.3 on Llama 3.1 405B.
% leads to 
% 41.1 
% +39.0
% points in 5-shot MMLU accuracy. For Llama 3.1 405B, \name{} similarly gets +38.3 points. 
These results highlight \name{}' ability to linearize large-scale models with greater efficiency and improved performance, showing for the first time that we can scale up linearizing to 70B+ LLMs.

\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{0.99\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}lcccccc@{}}
\toprule
                       & PiQA           & ARC Easy       & ARC Challenge  & HellaSwag      & WinoGrande     & MMLU (5-shot)  \\ 
                       & acc            & acc            & (acc norm)     & (acc norm)     & acc            & acc            \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Llama 3.1 8B          & 79.87          & 81.52          & 53.58          & 79.01          & 73.48          & 66.11          \\
Linearized, no attn. transfer & 78.67	& 78.11	& 49.83	& 77.83 & 	68.51 & 	51.44          \\



\name{} (Ours)                & \textbf{80.96} & \textbf{82.37} & \textbf{54.44} & \textbf{79.07} & \textbf{69.69} & \textbf{54.88} \\ \midrule

\rowcolor[HTML]{EFEFEF} 
Llama 3.1 70B          & 83.10          & 87.30          & 60.60          & 85.00          & 79.60          & 78.80          \\
% Linearized, no attn. transfer & 75.70          & 70.10          & 39.10          & 77.40          & 58.60          & 26.60          \\

Linearized, no attn. transfer & 81.99 &	80.89 &	54.44 &	82.29 &	71.19 &	28.74 \\
\name{} (Ours)                & \textbf{82.10} & \textbf{84.98} & \textbf{60.50} & \textbf{84.62} & \textbf{73.72} & \textbf{67.70} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
Llama 3.1 405B         & 85.58          & 87.58          & 66.21          & 87.13          & 79.40          & 82.98          \\
Linearized, no attn. transfer & 84.44          & 86.62          & 64.33          & 86.19          & 79.87          & 33.86          \\
\name{} (Ours)                & \textbf{85.58} & \textbf{88.80} & \textbf{67.75} & \textbf{87.41} & \textbf{80.35} & \textbf{72.20} \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-0.25cm}
\caption{\textbf{Linearizing Llama 3.1 8B, 70B, and 405B}. Among the first linearized 70B and 405B LLMs (via low-rank linearizing), \name{} significantly improves zero- and few-shot quality.
}
\label{table:chungus_results}
\vspace{-0.5cm}
\end{table}


==> sections/iclr_5_conclusion.tex <==
\vspace{-0.25cm}
\section{Conclusion}
\label{sec:conclusion}
\vspace{-0.25cm}
We propose \name{}, an efficient LLM linearizing method that (1) trains linear attentions
% attention analogs---such as linear attentions and linear attention + sliding window hybrids---
to match an LLM's self-attentions, before (2) swapping the attentions and only finetuning the replacing attentions with LoRA. 
%
% We exploit the fidelity between these attention analogs and softmax attention, 
This reduces linearizing to learning good softmax attention approximations, and we study how to do so.
% study how to better approximate softmax attention.
% in a subquadratic analog. 
%
% Furthermore, we demonstrate that via an MSE-based attention output-matching loss, we \emph{are able} to train such attention analogs to approximate the ``ground-truth'' softmax attentions in practice. 
%
On popular LM Eval tasks,
% and 5-shot MMLU, 
% we find \name{} 
\name{} enables LLMs with high quality and inference efficiency, outperforming prior Transformers alternatives while only updating 0.2\% of model parameters and requiring 0.003\% of LLM pretraining tokens. Our findings substantially improve linearizing quality and accessibility, enabling the first linearized 70B and 405B LLMs. 

==> sections/old/1_intro_0924.tex <==
% \input{sections/figures/pull_results}
% \input{sections/figures/pull_results_v2}
\clearpage
\section{Introduction (Another Pass)}
\label{sec:intro}

% Opening
Recently, ``linearizing'' Transformers---or converting existing Transformers into attention-free subquadratic alternatives---has shown exciting promise for scaling up new architecture candidates. 
A number of works propose alternative architectures to the Transformer, often pretraining small models from scratch on modest academic budgets~\citep{gu2023mamba,peng2023rwkv,yang2023gated,arora2024simple,beck2024xlstm}.  
In contrast, modern large language models are trained with 7B+ parameters and trillions of tokens~\citep{AI_2024,jiang2023mistral}. 
To improve the accessibility of subquadratic LLMs, linearization methods seek to use a pretrained Transformer LLM as a starting point and simply replace the quadratic softmax attention with the alternative---\eg{} \textit{linear attentions}~\citep{kasai-etal-2021-finetuning,mao-2022-fine,zhang2024the} or state-space model (SSM)~\citep{yang2024parallelizing,wang2024mamba}---resulting in a model with  \textit{linear} time and \textit{constant} memory generation.


% Challenges
We desire methods that are (1) \textbf{quality-preserving} to maintain the abilities of modern LLMs, and (2) \textbf{parameter-} and (3) \textbf{token-efficient} to to linearize LLMs on widely accessible compute budgets. 
% reduce the training speed.
% What's wrong with prior
However, current linearization methods struggle along the three criteria. 
Relative to the Transformer baseline, these methods reduce quality by 1.7--8.0 points on popular zero-shot LM Evaluation Harness (LM Eval)~\citep{eval-harness} tasks, while dropping up to 28.0 points on 5-shot MMLU \simran{a X\% drop}. 
% This quality drop amounts to the difference between a \simran{X} and \simran{X} billion parameter model.  
In efficiency, all the existing procedures use full-model training in the adjustment step and use 100B tokens to linearize 7B LLMs. These costs limit the accessibility of linearization at the 7B parameter scale, let alone 100B+ parameters, ~\eg{} Llama 3.1 405B~\citep{dubey2024llama}.

% for popular 7B+ LLMs such as Llama 3 8B~\citep{llama3modelcard} or Mistral 7B~\citep{jiang2023mistral}. They also make linearizing difficult to scale to larger LLMs,~\eg{} Llama 3.1 405B~\citep{dubey2024llama}, where full-model training remains prohibitively expensive under ``academic'' compute~\citep{wang2024mamba}.

We thus propose \textbf{\textsc{Lo}}w-rank \textbf{\textsc{L}}inear \textbf{\textsc{C}}onversion with \textbf{\textsc{A}}ttention \textbf{\textsc{T}}ran\textbf{\textsc{s}}fer (\name{}). With \name{}, we not only linearize models that outperform the prior methods by \simran{X} at 7B parameters, but also release the \textit{first subquadratic 100B parameter LLM} ($50\times$ larger models than prior work), which we linearize from Llama 3 $405$B with just $40$M tokens ($4$\% the tokens the prior work).
% requires at the 7B scale alone

We identify and address two key challenges to enable this progress. Following the standard two-stage approach in the prior work, we (1) initialize our LLM with the pretrained Transformer weights and replace attentions with subquadratic analogs, before (2) training the LLM end-to-end with next-token-prediction to adjust for the swapped layers ~\citep{mercat2024linearizing,yang2024parallelizing,wang2024mamba}. Our insights are:
\begin{enumerate}[leftmargin=*]
    \item[(1)] \textbf{Low-Rank. All prior LLM linearizing works update all the Transformer's parameters after attention swapping.} Correspondingly, these prior works report that the linear attentions are unstable to train~\citep{ mercat2024linearizing,qin2023scaling} and SSMs take even larger architectural departures from attention, requiring further re-training. In \name{}, we show a suprirising result that we can \textit{freeze all the Transformer parameters} (MLPs and attention weights). We (1) introduce learned \textit{feature maps}, applied to the queries and keys, that are trained to mimic the original attention weights (\simran{X} additional parameters) and (2), to adjust for the swapped layers, we use low-rank adaptations (LoRA). 
    \item[(2)] \textbf{Attention transfer. Subquadratic architectures struggle to approximate softmax attention.} Prior works suggest that linear attentions struggle to match the expressivity of softmax~\citep{keles2023computational,qin-etal-2022-devil}. \name{} addresses this challenge by first combining linear attention with a subquadratic sliding window variant to support the long range and dense local token interactions of attention, respectively. Second, we introduce an explicit ``attention transfer'' training stage, where we train the swapped attentions to match the Transformer attention weights using a mean-squared error loss over the attention outputs of each layer (Figure~\ref{fig:results_attn_weight_ex}), before stitching the layers together with the end-to-end LoRA stage.
\end{enumerate}
We show that these simple insights produce high-quality subquadratic LLMs with state-of-the-art parameter- and token-efficiency both at 7B and 70B parameters. 

Motivated by the large efficiency and quality improvements, we explore the next challenge --- linearizing Llama 405B on an academic budget -- an uncharted regime in prior work. We uncover surprising quality and efficiency tradeoffs. In quality, we find that applying \name{} approach  with ``attention transfer'' excitingly performs \simran{X} better than a model trained without attention transfer, however remains \simran{X} worse than Llama 405B. Studying the remaining gap, we observe that the magnitudes of the attention weights increase with the layer depth (Figure), making it difficult to supervise with the joint MSE over $126$ layers. We thus propose finer-grained \textit{Cria-by-Cria attention transfer}: we split the Llama into Crias (blocks of $K$ layers) and perform attention transfer at this granularity, before stitching the Cria together. \footnote{Recall that a baby Llama is called a Cria.} We validate that this recoverse quality. However in efficiency, this requires \textit{saving} the hidden states of prior Cria as training inputs for subsequent Cria. At the Llama 405B scale, just $40$M tokens of data takes $165$ terrabytes of disk space if the number of layers per Cria $K=1$. Meanwhile, as $K$ increases, the GPUs required per Cria increases (\textit{e.g.}, $K=9$ is the limit to train on a single NVIDIA H100 80GB GPU at sequence length $1024$). We provide a simple cost model in \Cref{sec:method} to help navigate these tradeoffs.


\input{sections/figures/pull_results_v2}

Our experiments validate that \name{} results in high-quality and efficient linearization:
\begin{itemize}[leftmargin=*]
    \item \textbf{Quality.} (1) Compared to past linearizing methods, \name{} linearized Mistral-7B and Llama 3 8B improves by 0.2$-$8.0 points (pts) on zero-shot LM Eval tasks and +17.8 pts on 5-shot MMLU. (2) Compared to strong 7B subquadratic LLMs \textit{pretrained from scratch} (RWKV-v6~\citep{peng2024eagle}, Mamba~\citep{gu2023mamba}, Griffin~\citep{de2024griffin}) and hybrids (StripedHyena~\citep{poli2023hyena}, Zamba~\citep{glorioso2024zamba}), \name{} gives 1.8 to 4.7 pts improvement on average over LM Eval tasks. Finally, (3) \name{} Llama 3 8B for the first time closes the zero-shot LM Eval gap between linearized and Transformer models (73.1 vs 73.7 pts), while supporting 3$\times$ higher throughput and 64$\times$ larger batch sizes vs popular FlashAttention-2~\citep{dao2023flashattention} implementations when generating 4096 token samples on an 80GB H100. In ablations, we show the insights in \name{} bring these improvements.
    
    \item \textbf{Parameter and token efficiency.} By only training linear attentions in Stage 1, while only using LoRA in Stage 2, \name{} enables these gains despite only updating $<$0.2\% of the model parameters. \name{} produces these results with only 40 million tokens, \textit{i.e.,} 0.003\% of the token budget of prior pretraining, and 0.04\% of those in prior linearizing methods. 
\end{itemize}


\name{} presents the first viable approach to linearizing the complete Llama 3.1 model family of 8B, 70B, and 405B parameter LLMs~\citep{dubey2024llama}. 
For 70B, we improve 5-shot MMLU accuracy by 43.5 points over prior work ~\citep{mercat2024linearizing} and at 405B, uniquely enable viable linearization, where the baseline fails to train (2.41 versus \textcolor{red}{X.XX} PPL. 
In efficiency, training takes only 8 hours on 1 40GB A100 for 8B (versus 5 days on 8$\times$80GB H100s with prior work~\citep{wang2024mamba}), 8 H100s for 70B and 16 hours across 24 80GB H100s for 405B \textcolor{red}{(need a relative)}.  
We hope \name{} improves the accessibility of subquadratic LLMs.





==> sections/old/3_method_0927.tex <==
% \section{\name{}: {Low-rank Linear Conversion via Attention Transfer}}
\section{Method: Linearizing LLMs with \name{}}
\label{sec:method}
We now present \name{}, a simple and efficient method to linearize LLMs. 
%
In Section~\ref{sec:method_arch}, we first describe our initial architecture setup for replacing a Transformer LLM's softmax attentions with linear attention analogs.
% , and our candidates for these analogs (learnable linear attentions; \ref{}). 
% By replacing the attentions at each layer, we aim to remove the source of the Transformer's generation inefficiency, while introducing an expressive enough linear attention to act as a literal drop-in replacement. 
%
In Section~\ref{sec:method_train}, we next describe our two-step training procedure to (1) train these linear attentions to match softmax attentions (\ref{}), before (2) joining the layers together via low-rank adaptation (\ref{}). 
%
As motivation for each of our design choices, we hypothesize that by replacing softmax attentions with closely approximating linear variants in Step 1, we can effectively linearize LLMs with minimal subsequent parameter updates or training tokens in Step 2.

% In Section~\ref{sec:method_asdf}, we study how these components together enable LLM linearizing with higher quality, parameter-efficiency, and token-efficiency. 

% perform a preliminary study to see  

% such that we remove the source of a Transformer's generation inefficiency, while ideally 



% Like past work~\citep{mercat2024linearizing}, we (1) swap an LLM's softmax attentions with subquadratic analogs, before (2) training the LLM end-to-end with next-token prediction to adjust for swapping.
% %
% However, to improve linearizing quality, parameter efficiency, and token efficiency, we (1) replace softmax attentions with subquadratic analogs \emph{trained} to approximate softmax attention (``attention transfer''), before (2) only adjusting via low-rank adaptation (LoRA). Below we expand on these steps and their contributions to our linearizing criteria in Section~\ref{sec:method_1_attn_transfer} and Section~\ref{sec:method_2_lora_linearize}.

% with the following sections:
% %
% \begin{itemize}[leftmargin=*]
%     \item In Section~\ref{sec:modeling_setup}, we describe our modeling setup for parameter-efficient attention transfer and LoRA. 
    
%     \item In Section~\ref{}, we validate that via attention transfer, we \emph{can} train existing linear attentions to sufficiently approximate softmax attention. Furthermore, doing this training enables significantly improves linearizing quality and parameter- and token-efficiency among existing linear attentions.
    
%     \item In Section~\ref{}, we show that we can further improve attention transfer's quality and training feasibility. 
% \end{itemize}
% % to replace softmax attention with ``close'' subquadratic attention analogs
    
%     that we \emph{can} learn 
%     Here we hypothesize that by replacing softmax attentions with ``close'' subquadratic attention analogs, we then only need a minimal amount of additional training 


% \subsection{Modeling Setup: Low-rank Linearizing with Linear Attention}
% \label{sec:modeling_setup}
% \label{sec:method_1_attn_transfer}

% \subsection{\name{} Architecture: Linearizing Llamas as 32 Hedgehogs in a Trenchcoat}
\subsection{\name{} Architecture}
\label{sec:method_arch}
To convert Transformer-based LLMs into subquadratic variants, like prior work we start by simply replacing softmax attentions with linear attention counterparts. Here we go over our exact architectural setup, which supports linearizing LLMs with various linear attentions using \textit{learnable} feature maps proposed in prior work~\citep{kasai-etal-2021-finetuning,zhang2024the}. 

\input{sections/figures/pull_method}


% This necessarily removes the source of Transformers' quadratic generation inefficiencies. However, to improve quality and training efficiency, we study how to replace softmax attentions with linear attentions with \textit{learnable} feature maps. 


% By first replacing each softmax attention with a linear attention counterpart, we remove the source of Transformers' generation inefficiency. At the same time, we introduce an expressive enough linear attentions to approximate softmax attention and facilitate parameter and token-efficient linearizing.

% We go over how we replace the attentions at each layer. we aim to remove the source of the Transformer's generation inefficiency, while introducing an expressive enough linear attention to act as a literal drop-in replacement. 

\subsubsection{Replacing Softmax with Learnable Linear Attentions}  
% irst considering the single head linear attention case. 
% Due to architectural similarities, for every layer we simply replace the original softmax attention with a linear attention
For every Transformer block, we replace the original softmax attention with a linear attention layer. With notation from Section~\ref{sec:preliminaries}, we initialize the linear attention layers by simply using the same projection weights $\bm{W}_q, \bm{W}_k, \bm{W}_v, \bm{W}_o$ due to architectural similarities. This retains inputs $\bm{q}_n, \bm{k}_i, \bm{v}_i$. We only introduce new query and key feature maps $\phi_q$ and $\phi_k$ for each head, thus changing the head-specific attention outputs from:

\begin{equation}
    % \hat{\bm{y}}_n 
    % =
    % \right(
    \mathnormal{
    \underbrace{
    \bm{y}_n = 
    \sum_{i=1}^n \frac{ \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})}{\sum_{i=1}^n \exp(\bm{q}_n^\top \bm{k}_i  / \sqrt{d} )} \bm{v}_i
    }_{\text{Softmax Attention}}
    \;\;\rightarrow \;\;
    \underbrace{
    \hat{\bm{y}}_n = 
    \sum_{i=1}^n \frac{ \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i)}{\sum_{i=1}^n \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i) } \bm{v}_i
    }_{\text{Linear Attention}}}
    % \left)
\label{eq:attn_matching_setup}
\end{equation}

\begin{equation}
    % \hat{\bm{y}}_n 
    % =
    % \right(
    \underbrace{
    \bm{y}_n = 
    \sum_{i=1}^n \frac{ \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d})}{\sum_{i=1}^n \exp(\bm{q}_n^\top \bm{k}_i  / \sqrt{d} )} \bm{v}_i
    }_{\text{Softmax Attention}}
    \;\;\rightarrow \;\;
    \underbrace{
    \hat{\bm{y}}_n = 
    \sum_{i=1}^n \frac{ \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i)}{\sum_{i=1}^n \phi_q(\bm{q}_n)^\top \phi_k(\bm{k}_i) } \bm{v}_i
    }_{\text{Linear Attention}}
    % \left)
\label{eq:attn_matching_setup}
\end{equation}
% for all positions $n$ in a sequence. 
Like prior work~\citep{kasai-etal-2021-finetuning,zhang2024the}, we parameterize the feature maps $\phi : \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$ (where $d$ is head dimension, $d'$ is arbitrary ``feature'' dimension) as trainable neural net layers 
% , we parameterize feature maps as trainable layers~\citep{kasai-etal-2021-finetuning,mao-2022-fine,zhang2024the} where
% like prior linearizing work~\citep{kasai-etal-2021-finetuning,mao-2022-fine,zhang2024the} we parameterize the feature maps as trainable layers 
% for queries and keys in $\mathbb{R}^{l \times d}$ (where $l$ is sample length).  
% with trainable weights and biases $\tilde{\bm{W}} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}} \in \mathbb{R}^{d'}$
\begin{equation}
    \phi_q(\bm{q}) := f(\bm{q}\tilde{\bm{W}}_q + \tilde{\bm{b}}_q),
    \;\;\;
    \phi_k(\bm{k}) := f(\bm{k}\tilde{\bm{W}}_k + \tilde{\bm{b}}_k)
\label{eq:feature_maps}
\end{equation}
% \textit{i.e.,} $\phi_\text{mlp}(\bm{q}) := f(\bm{q}\tilde{\bm{W}} + \tilde{\bm{b}})$,
where $\tilde{\bm{W}} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}} \in \mathbb{R}^{d'}$ are trainable weights and optional biases, 
% Here $\tilde{\bm{W}}_{(\cdot)} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}}_{(\cdot)} \in \mathbb{R}^{d'}$ are trainable weights and optional biases,
and $f(\bm{x})$ is a nonlinear activation. In this work we study two activations used in prior linearizing works: element-wise $\text{ReLU}(\bm{x})$ as used in Transformer-to-RNN (T2R)~\citep{kasai-etal-2021-finetuning} and SUPRA~\citep{mercat2024linearizing}, and dimension-wise $[\text{softmax}(\bm{x}) \oplus \text{softmax}(-\bm{x})]$ as used in Hedgehog~\citep{zhang2024the}. 

\paragraph{Positional encoding details.}To support modern LLMs like Llama 3 8B~\citep{llama3modelcard} and Mistral 7B~\citep{jiang2023mistral} that use rotary embeddings to encode position~\citep{su2024roformer}, we apply the feature maps $\phi$ \textit{after} positional encoding. Letting $\text{RoPE}(\cdot)$ denote applying rotary embeddings, before apply feature maps as in Eq.~\ref{eq:feature_maps} we compute initial query, key, and value inputs 
\begin{equation}
    \bm{q} = \text{RoPE}(\bm{x}\bm{W}_q),
    \;\;\;
    \bm{k} = \text{RoPE}(\bm{x}\bm{W}_k),
    \;\;\;
    \bm{v} = \bm{x}\bm{W}_v
\end{equation}
Unlike prior works that apply $\phi$ \textit{before} positional encoding~\citep{mercat2024linearizing, su2024roformer}, our choice preserves the linear attention kernel where $k(\bm{x}, \bm{x}') = \exp(\bm{x}^\top \bm{x}') \approx \phi_q(\bm{x})^\top \phi_k(\bm{x}')$, $(\bm{x},\bm{x}') = (\bm{q},\bm{k})$. Later we show how this allows us to find suitable $\phi$ by only training feature map weights in a parameter- and token-efficient manner. 

\subsubsection{Expanding Learnable $\phi$ Parameterizations}
\label{sec:method_analogs}
% \paragraph{Expanding Learnable $\bm{\phi}$ Parameterizations.} 
As described, we can apply the \name{} setup to linearize with any pure linear attentions with learnable $\phi$ (\textit{e.g.}, T2R and Hedgehog, Figure~\ref{fig:train_efficiency}). 
% In our method development, we evaluate two learnable $\phi$ parameterizations. First, we consider the pure linear attention setup discussed above, evaluating how the T2R and Hedgehog activations transfer to our \name{} setting in Section~\ref{}.
%
However, to improve attention-matching quality, we introduce a hybrid $\phi$ parameterization combining linear attention and \textit{sliding window attention}. Motivated by prior works that show quality improvements when combining attention layers with linear attentions~\citep{arora2024simple,Munkhdalai2024-kx}, 
% recurrences~\citep{de2024griffin}, and state-space models~\citep{fu2022hungry,stripedhyena,lieber2024jamba}, 
we combine \textcolor{blue}{short sliding windows of softmax attention}~\citep{beltagy2020longformer,zhu2021long} (size 64 in experiments) \textcolor{cyan}{followed by linear attention} in a single layer. This allows attending to all prior tokens for each layer, while keeping the entire LLM fully subquadratic. For window size $w$ and token indices $[1, \ldots, n-w, \ldots, n]$, we apply the softmax attention over the $w$ most recent tokens, 
and compute attention outputs $\hat{\bm{y}}_n$ as
\begin{equation}
    \hat{\bm{y}}_n =  
    \frac{ \textcolor{blue}{\sum_{i=n-w+1}^n \gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)\bm{v}_i} + \textcolor{cyan}{\phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)\bm{v}_j^\top \big)}}{ \textcolor{blue}{\sum_{i = {n-w+1}}^n\gamma \exp(\bm{q}_n^\top \bm{k}_i / \sqrt{d} - \bm{c}_n)}\; +  \textcolor{cyan}{\phi_q(\bm{q}_n)^\top \big( \sum_{j=1}^{n-w}\phi_k(\bm{k}_j)^\top \big)}} 
\label{eq:hybrid_linear_swa}
\end{equation}
$\gamma$ is a learnable mixing term, and $\bm{c}_n$ is a stabilizing constant as in log-sum-exp calculations ($\bm{c}_n = \max_i\big\{\bm{q}_n^\top \bm{k}_i / \sqrt{d} : i \in [n-w+1, \ldots, n]\big\}$).
Like before, we can pick any learnable $\phi$.

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mse_analogs_llama3_8b_serif.png}
        % \vspace{-0.5cm}
        \caption{Llama 3 8B}
        \label{fig:mse_analogs_llama3}
    \end{subfigure}
    % \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/mse_analogs_mistral_7b_serif.png}
        \caption{Mistral 7B (v0.1)}
        \label{fig:mse_analogs_mistral7b}
    \end{subfigure}
    \vspace{-0.25cm}
    \caption{\textbf{Attention matching MSE}. Across LLMs, linearizing with hybrid linear attention + sliding window better approximates ``ground-truth'' softmax attentions via lower MSE over layers.}
    \label{fig:mse_analogs}
    \vspace{-0.25cm}
\end{figure}

\paragraph{Subquadratic efficiency.} The hybrid layer retains linear time and constant memory generation. For $n$-token prompts, we initially require $\mathcal{O}(w^2 d)$ and $\mathcal{O}((n-w)dd')$ time and space for window and linear attention respectively, attending over a $w$-sized KV-cache and computing KV and K-states (Eq.~\ref{eq:linear_attention_recurrent}). 
For generation, we only need $\mathcal{O}(w^2 d + dd')$ time and space for every token. We evict the KV-cache's first $\bm{k}$, $\bm{v}$, compute $\phi_k(\bm{k})$, and add $\phi_k(\bm{k})\bm{v}^\top$ and  $\phi_k(\bm{k})$ to KV and K-states respectively.

\paragraph{Hardware-aware implementation.} 
\input{sections/figures/method_sliding_window}
We further support two sliding window setups for fast inference: a standard sliding window where $w$ is the same for all tokens, and a ``terraced'' window where $w$ changes based on token index (Figure~\ref{fig:hybrid_attn}). While we found both comparable in quality, the latter exploits the new ThunderKittens (TK) DSL~\citep{todo}'s primitives for implementing fast CUDA kernels. Here we prefer contiguous blocks of size 64, which can quickly 
% compute the softmax terms 
be computed
in parallel on modern GPUs. We include implementation details in Appendix~\ref{app:tk_implementation}. 

\subsection{\name{} Training \MZ{some pun on crias in trenchcoats}}
We next train these linearizing layers to recover LLM quality in two simple steps. First, we train feature maps so the layers approximate softmax attentions (\ref{sec:method_step_1}). Next, we only apply low-rank adaptation (LoRA) on their projections to subsequently adjust for any approximation errors (\ref{sec:method_step_2}).

% our two-step procedure for linearizing LLMs to recover quality while remaining parameter and token-effic


\subsubsection{Step 1: Learning Softmax Replacements with Attention Transfer}
\label{sec:method_step_1}

% \paragraph{Approximating Softmax with Efficient Attention Transfer.}
% \subsubsection{Learning to Approximate Softmax with Efficient Attention Transfer}


To find desirable $\phi$, we explicitly train these feature maps such that the replacing linear attentions approximate softmax attention.
Following Hedgehog \citep{zhang2024the}, we treat this as distillation across architectures.
%
However, while Hedgehog learns this approximation via an expensive cross-entropy loss over all $n^2$ attention weights for $n$-token samples, we find a simple mean-squared error (MSE) loss over attention outputs---computable in $O(n)$ memory---suffices.
% %
% Instead, we find a simple mean-squared error (MSE) loss over attention outputs---computable in $O(n)$ memory---suffices. 
%

For each layer we first simply compute $\bm{q}, \bm{k}, \bm{v}$ from real data as distillation inputs.
%
We then train $\phi_q$ and $\phi_k$ jointly such that with ``predicted'' linear attention outputs $\{\hat{\bm{y}}_n\}_{n=1}^l$ via Eq.~\ref{eq:linear_attention_2} and ``ground-truth'' softmax attention outputs $\{\bm{y}_n\}_{n=1}^l$ via Eq.~\ref{eq:causal_attention}, we minimize a sample MSE loss:
\begin{equation}
    \ell_n(\bm{y}_n, \hat{\bm{y}}_n) = \frac{1}{d}\sum_{i=1}^d (y_{n,i} - \hat{y}_{n,i})^2
\label{eq:lolcats_mse_loss}
\end{equation}
% \paragraph{Multiple heads and layers.} 
For an LLM's multi-head attention and multiple layers, we simply use unique $\phi_q$ and $\phi_k$ for each head and layer.
% We jointly train $\phi$ to minimize MSE between each head's outputs. 
To train these layers, we freeze all parameters outside of $\phi_q,\phi_k$, and compute layer-wise inputs $\bm{q}, \bm{k}, \bm{v}$ and outputs $\bm{y}$ with the original softmax attentions. This allows parallel training across layers, where we can train any contiguous set of layers' $\phi_q, \phi_k$ jointly to minimize output MSEs. ``Teacher-forcing'' with the softmax-derived inputs also prevents errors in earlier layers from impacting later layers. We include full implementation details in Appendix~\ref{} and our code release\footnote{\url{https://github.com/lolcats_iclr2025}}.
% \footnote{\url{https://github.com/HazyResearch/lolcats}}.

% \paragraph{Attention matching quality.} In Figure~\ref{fig:method_attn_weight_comparison}, we visualize Llama 3 8B sample attention weights computed with various (trained) linear attentions.  Despite only training to minimize the MSE between attention outputs, our proposed attention transfer loss recovers similar attention weights to the prior Hedgehog loss. Both losses recover softmax attentions versus untrained Hedgehog feature maps. \textcolor{blue}{(MZ: violin plot)}

% \input{sections/figures/results_attn_weight_comparison}
\input{sections/figures/method_attn_weight_comparison}

\input{sections/figures/method_train_efficiency}

\paragraph{Memory Savings.}
With just the attention outputs, \name{} reduces attention transfer memory from Hedgehog's $O(n^2)$ in sequence length to $O(n)$. 
For subquadratic analogs we use Eq.~\ref{eq:linear_attention_2} or Eq.~\ref{eq:hybrid_linear_swa} to compute outputs in linear time and space. For softmax attentions, we use FlashAttention to also compute outputs in linear space, never materializing all softmax attention weights with tiling and recomputation~\citep{dao2022flashattention,dao2023flashattention,shah2024flashattention}. 

\subsubsection{Step 2: Low-rank Linearizing with LoRA}
% \label{sec:method_2_lora_linearize}
\label{sec:method_step_2}

% \paragraph{Step 2. Low-rank Linearizing.} 
After training and swapping in the linearizing layers, we proceed by simply replacing the full-parameter training of prior work with low-rank adaptation (LoRA)~\citep{hu2021lora}. Like prior work, we train the modified LLM end-to-end with a next-token prediction loss over some sample data. However, rather than train all LLM parameters, we only train the swapped linear attention projections with LoRA. 
% for parameter-efficiency we only train the query, key, value, and output projections  of the swapped linear attention layers with LoRA. 
Instead of full-rank updates $\bm{W}' \leftarrow \bm{W} + \Delta \bm{W}$, LoRA decomposes $\Delta \bm{W}$
into the product of two low-rank matrices $\bm{B}\bm{A}$, $\bm{B} \in \mathbb{R}^{d \times r}$, $\bm{A} \in \mathbb{R}^{r \times d}$. For parameter-efficiency, we aim to pick small $r \ll d$ that still enables sufficient updates for adjusting to the swapped attentions.

\subsection{Empirical Analysis: Validating \name{} Components}

\MZ{discuss}
Before evaluating \name{} in our main results, we evaluate whether each of our components leads to its stated claim of improving attention matching quality, while remaining parameter and token efficient.   

\paragraph{Attention matching quality.} In Figure~\ref{fig:method_attn_weight_comparison}, we visualize Llama 3 8B sample attention weights computed with various (trained) linear attentions.  Despite only training to minimize the MSE between attention outputs, our proposed attention transfer loss recovers similar attention weights to the prior Hedgehog loss. Both losses recover softmax attentions versus untrained Hedgehog feature maps. \textcolor{blue}{(MZ: violin plot)}

\paragraph{Parameter efficiency.} 
Despite using separate $\phi$ for each head and layer, doing this attention transfer remains more parameter-efficient than the full-training in prior linearizing work~\citep{mercat2024linearizing,yang2024parallelizing,wang2024mamba}.
For Llama 3 8B or Mistral 7B,
we train $\phi$ with feature dimension $d' = 64$ and no bias. This amounts to 
32 layers $\times$ 32 heads $\times$ 2 feature maps $\times$ $(128 \times 64)$ weights $\approx$ 16.8M trainable parameters (about 0.2$\%$ of original LLM sizes).

Furthermore, in Stage 2 by sweeping $r \in \{4, 8, 16, 32, 128\}$, we find that $r = $ 8 $\ll$ head dimension 128 suffices. 

\paragraph{Token efficiency.}
While \name{} as described reduces linearizing parameter count and improves quality, 
% (allowing us to linearize 7B LLMs in native \texttt{bfloat16} on one 40GB GPU), 
we find the attention transfer also unlocks higher training efficiency, \textit{i.e.}, higher quality linearizing with fewer training tokens.
We compare the validation split perplexity of low-rank linearized Llama 3 8B and Mistral 7B with and without attention transfer, using both T2R and Hedgehog, and the Alpaca dataset. For fair comparison, we now equalize training budgets: 2 epochs for attention transfer and 2 epochs for post-swap training, or 4 epochs for post-swap training alone.
%
Even when accounting for attention training time, linearizing with attention transfer consistently achieves lower perplexity faster (Figure~\ref{fig:train_efficiency}). 
%

% As a hypothesis for why this may be possible, via only low-rank updates on the attention layers, we (1) preserve the pretrained ``knowledge and concepts'' in parameter-heavy layers such as the MLPs, and (2) focus training with the linearizing data on recovering the sequence-mixing patterns of the original attentions. We can thus recover generalized LLM capabilities with limited samples.
% We find evidence of this in our main results (\textit{e.g.,} recovering zero-shot LM Eval and 5-shot MMLU quality despite training on 50K Alpaca instruction-following samples).



\paragraph{Data.} \MZ{Discussion on robustness of linearizing data; can use RedPajama or Alpaca}








% \paragraph{Better Attention Matching Corresponds with Linearizing Quality}

% % Through experiments, we find $r = 8$ (versus $d = 128$ for Llama and Mistral LLMs) sufficient, enabling much more accessible linearizing by updating $<$0.09\% of original LLM parameter counts.


% % \subsection{Motivating Analysis: Is Low-rank Linearizing Even Possible?}

% \subsubsection{Attention Transfer Enables Parameter and Token-Efficient Linearizing}

% As an initial test, we aim to understand if attention transfer can enable low-rank linearizing. While prior methods also often selectively train just their attention analogs during an initial stage of attention distillation or transfer~\citep{zhang2024the,yang2024parallelizing,wang2024mamba}, they still train all model parameters in subsequent stages of adjusting to the replacing layers. For 7B LLMs, prior works also advertise training on 100B tokens. Towards efficiently scaling up linearizing to modern LLMs with 7B+ parameters, it thus remains unclear if we can significantly improve parameter and token-efficiency without a substantial drop in quality. 

% % While we would like to remove this parameter-inefficient training, \textit{e.g.,} to to efficiently scale up linearizing to modern LLMs with 7B+ parameters, it thus remains unclear if we can do so without a substantial drop in quality. 

% \textbf{Experimental Setup.} As an initial study of \name{}' proposed components, we evaluate whether attention transfer and low-rank linearizing can produce viable linearized LLMs in a token and parameter-efficient manner. For linearizing layers, we consider both the Transformer-to-RNN (T2R)~\citep{kasai-etal-2021-finetuning} and Hedgehog~\citep{zhang2024the} linear attentions featured in prior work. To study if a small amount of linearizing data can suffice, we use the $\sim$50K samples of a cleaned Alpaca dataset\footnote{\url{https://huggingface.co/datasets/yahma/alpaca-cleaned}}, citing Alpaca's ability to showcase instruction-following over diverse topics in 7B LLMs despite its relatively small size~\citep{alpaca}.  To study performance across multiple models, we linearize the base versions of two popular 7B LLMs: Llama 3 8B~\citep{llama3modelcard} and Mistral 7B v0.1~\citep{jiang2023mistral}. 

% % We pack samples into 1024-token sequences  

% To study attention transfer's impact, we linearize both with and without attention transfer.
% With transfer, in Step 1 we train all feature map weights via Eq.~\ref{eq:attn_matching_setup} for two epochs with learning rate 1e-2, and in Step 2 apply LoRA on
% the attention projection layers for two epochs with learning rate 1e-4. Without transfer, we swap attentions and apply Step 2 for four epochs.
% %
% For all steps, we use the same Alpaca training samples packed into 1024-token sequences with batch size 8, and train with early stopping, and AdamW optimizer~\citep{loshchilov2017decoupled}.
% % 8192-token sequences with batch size 1.
% % either batch size 8 with 1024-long packed sequences, or batch size 1 with 8192-long packed sequences. 

% % We include additional details in Appendix~\ref{} and our code release\footnote{\url{https://github.com/HazyResearch/lolcats}}.
% \textbf{Finding 1: Attention Transfer Improves Low-Rank Linearizing Quality}

% \textbf{Finding 2: Attention Transfer }

% We use Alpaca due to
% its ability to showcase general instruction-following in 7B
% LLMs despite its relatively small size



% adapt their replacing attention analogs 


% selectively train just the attention analogs 

% that adapt the replacing attention analogs 



% freeze attention-heavy blocks such as MLPs, they still involve some form of full-parameter training after post-swapping, and report  

% In this section, we aim to understand if \name{} as proposed 

% Can we remove MLP training entirely? Furthermore, 



% We next describe these components and our steps to find these subquadratic attention analogs below.
% %

% \textbf{Modeling Setup}

% \textbf{Determining if we can learn attention approximations}

% Rather than train the LLM with these linear attentions from scratch, we aim to first ``initialize'' then 

% feature maps from scratch, we aim to first ``initialize them'' 

% \textbf{Attention Transfer unlocks low-rank linearization}


% % while some subsequent adjusting may be necessary, we hope to avoid both (i) needing to re-incorporate ``pretrained knowledge'' in the linearizing data, and (ii) introducing drastic or deleterious changes,~\textit{i.e.,} by overfitting to the linearizing data.

% % to the pretrained weights,

% % \textit{e.g.}, to preserve pretrained knowledge and avoid overfitting to the linearizing data.

% \name{}' key components thus involve (1) replacing LLM attentions with subquadratic attention analogs ``close'' to softmax attention, and (2) only doing subsequent adjusting via LoRA.
% %
% We next describe these components and our contributions to make them work in \name{} below.

% Below, we first describe our modeling setup. 

% We next describe motivating experiments that allow us to identify exact subquadratic attentions. 

% \subsection{Modeling Setup: Low-rank Linearizing with Linear Attention}
% \label{sec:low_rank_linear_attn}

% To improve quality, 

% Given an existing Transformer-based LLM, we aim to replace each softmax attention layer with subquadratic alternative, noting that if we could re


% such that the resulting LLM is subquadratic in time and space over input and generation sequence length. We then wish to tune the resulting model, such that we can also reduces drops in modeling quality compared to the original LLM. 

% Learning close analogs via attention transfer. 


% while minimizing any loss in the original LLM's modeling quality. 

% \paragraph{Replacing softmax attentions with close attention analogs}


% Towards finding a suitable replacement, we consider the general form of \textit{learnable} linear attentions, where instead of manually specifying the feature map $\phi$, we in


% While some quality drop may be inevitable from this attention-replacing, we aim to reduce this loss in quality as much as possible. 



% while ideally maintaining the quality of the unmodified model. 


% for each head and layer we aim to 


% \subsubsection{Motivating experiments: Learning softmax attentions}

% We use the Alpaca dataset






% \subsubsection{Modeling Setup}

% \paragraph{Replacing Attentions with Linear Attention}

% \paragraph{Low-rank Linearizing}

% \paragraph{Is linear attention all we need?}

% As a first step, we ask whether we can simply replace the prior linearizing steps with low-rank linearizing. 

% Attention Transfer: 
% * In this case need to be able to show tha


% consider replacing the softmax attentions in LLMs with linear attentions as considered in prior work,  

% \paragraph{Linear Attention}


% \paragraph{Parameter-efficient attention transfer}

% % and how \name{} makes them work below. 

% \newpage





% % However, to improve linearizing model quality, parameter-efficiency, and token-training efficiency, we aim to intorudce




% % we introduce both (1) a linearizing architecture, and (2) a parameter- and token-efficient training method


% % % introduce:


% % We aim to identify both a (1) linearizing architecture, and (2) training method, 

% % % training efficiency, linearized model quality, and context-length support, we introduce:

% \begin{enumerate}
%     \item \textbf{Parameter-efficient attention transfer and model training}, where by first training subquadratic attentions to match softmax attentions, before using low-rank adaptation for post-swap training, we linearize with only $<$0.4$\%$ of a 7B+ LLM's parameters and 0.02$\%$ of prior methods' training tokens.
%     \item \textbf{Expanded subquadratic attention analogs}, where rather than restrict this attention transfer to a single linear attention formulation, we support both T2R and Hedgehog ``pure'' linear attentions, as well as newly introduced learnable \emph{linear attention} + \emph{sliding window attention} hybrid analogs for improved quality while retaining linear time and constant memory generation.

%     \item \textbf{Layer-wise attention output matching}, where we use an MSE-based attention training loss on the attention \textit{outputs} computable in $\mathcal{O}(n)$ instead of $\mathcal{O}(n^2)$ time and space complexity. This allows us to linearize over longer contexts, \textit{e.g.,} by using FlashAttention~\citep{dao2022flashattention,dao2023flashattention,shah2024flashattention} to compute softmax attention outputs and never having to materialize the $n^2$ attention weights.
% \end{enumerate}
% We describe each component below in further detail.
% % validating their contributions with motivating experiments. 
% Later in Section~\ref{sec:results}, we show how these components allow us to efficiently linearize LLMs into state-of-the-art subquadratic LLMs, compared to both non-Transformers architectures trained from scratch and prior linearizations.



% % \name{} simply:
% % \begin{enumerate}
% %     \item Trains attention analogs to match softmax attentions via an \emph{output-based MSE loss} before swapping.
% %     \item Only trains the swapped attention layers with \emph{low-rank adaptation} (LoRA).
% % \end{enumerate}
% % We next describe these steps in further detail.
% % %     \item First 
% % %     \item Then 
% % % \end{itemize}
% % % (i) low-rank adaptation (LoRA) instead of full model training, (ii) new learnable attention analogs that improve quality while retaining linear time and constant memory generation, and (iii) an MSE-based attention distillation loss which enables attention transfer in $\mathcal{O}(n)$ instead of $\mathcal{O}(n^2)$ time and space complexity.
% % \begin{itemize}
% %     \item Low-rank adaptation (LoRA) instead of full model training.
% %     \item New learnable (linear attention + sliding window) analogs trained to approximate softmax attentions, which improve quality yet retain linear time and constant memory generation.
% %     \item An MSE-based attention training loss computable in $\mathcal{O}(n)$ instead of $\mathcal{O}(n^2)$ time and space complexity.
% % \end{itemize}
% % \subsection{Method: Linearizing with \name{}}
% % \label{sec:method_lolcats}

% \subsection{Improving Training Efficiency with Attention Transfer and LoRA}
% % \subsubsection{Improving Training Efficiency with Attention Transfer and LoRA}
% \label{sec:method_lora}
% To better reduce the costs of obtaining subquadratic LLMs, our main insight is that we can both:
% % \begin{enumerate}g
% %     \item[(a)] Remove the need to update all 7B+ parameters of an LLM
% %     \item[(b)] Reduce the number of training tokens needed to recover performance
% % \end{enumerate}
% (a) remove the need to update all 7B+ parameters of an LLM and (b) reduce the number of training tokens needed to recover performance, 
% by (1) explicitly training subquadratic attention analogs to match the outputs of an LLM's softmax attentions before attention swapping, and (2) subsequently only training the introduced attention's projection layers with low-rank adaptation (LoRA) and a standard next-token prediction loss.

% % Specifically, for each head and layer, 



% % This follows from the intuition that 
% Intuitively, if we could replace an LLM's softmax attentions with nearly-matching linear attentions for every head and layer,
% % then we would only require a minimal amount of subsequent model parameter updating---if any at all---to adjust and recover original LLM quality.
% then we would only need minimal amounts of subsequent training---if any at all---to adjust and recover original LLM quality. We next describe how \name{} does this below.
% %

% Later
% Furthermore, by restricting this training to low-rank updates on the attention layers, we aim to avoid drastic or deleterious changes to the pretrained parameters, \textit{e.g.}, to preserve pretrained knowledge and avoid overfitting to the linearizing data. 

% to parameter-heavy layers such as the MLPs. 
% This may help 
% % retain ``pretrained knowledge'', 
% reduce overfitting to linearizing data for general LLM capability recovery with less samples.
% with less samples.
% We leave further empirical analysis of this idea to Appendix~\ref{}, but find evidence in our main results (\textit{e.g.,} recovering zero-shot LM Eval quality despite training on 50k Alpaca instruction-following samples).
%


% \begin{enumerate}
%     \item \textbf{Parameter-efficient attention transfer:} For each softmax attention in every layer, we aim to learn a corresponding linear attention, which minimizes the mean-squared error (MSE) over attention head outputs. We simply treat this as a feature map learning problem. 
%     %
%     We first consider a single head and layer, with MLP-based feature maps $\phi_\text{mlp} : \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$ (where $d$ is head dimension, $d'$ is an arbitrary output or ``feature'' dimension), we initialize separate MLPs to process queries and keys $\bm{q}, \bm{k} \in \mathbb{R}^{l \times d}$
%     % for each head and layer we train query and key-specific MLPs
%     \begin{equation}
%         \phi_q(\bm{q}) := f(\bm{q}\tilde{\bm{W}}_q + \tilde{\bm{b}}_q),
%         \;\;\;
%         \phi_k(\bm{k}) := f(\bm{k}\tilde{\bm{W}}_k + \tilde{\bm{b}}_k)
%     \end{equation}
%     % \textit{i.e.,} $\phi_\text{mlp}(\bm{q}) := f(\bm{q}\tilde{\bm{W}} + \tilde{\bm{b}})$,
%     Here $\tilde{\bm{W}} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}} \in \mathbb{R}^{d'}$ are MLP weights and biases, and $f(x)$ is any element-wise ``activation'' used in prior linear attentions ($\text{ReLU}(x)$ for T2R~\citep{kasai-etal-2021-finetuning}, $[\text{softmax}(x) \oplus \text{softmax}(-x)]$ for Hedgehog~\citep{zhang2024the}).
% %
%     To train these MLPs, given attention head input $\bm{x} \in \mathbb{R}^{l \times d}$ (where $l$ is sequence length) and original softmax attention weights $\bm{W}_q, \bm{W}_k, \bm{W}_v \in \mathbb{R}^{d \times d}$, 
%     we compute the original queries, keys, and values
%     % softmax attention queries, keys, and values 
%     % $\{\bm{q}_i\}_{i=1}^{l}, \{\bm{k}_i\}_{i=1}^{l}, \{\bm{v}_i\}_{i=1}^{l}$
%     % $\bm{q}, \bm{k}, \bm{v}$ 
%     % (all $\in \mathbb{R}^{l \times d}$)
%     % where 
%     \begin{equation}
%         \bm{q} = \text{RoPE}(\bm{x}\bm{W}_q),
%         \;\;\;
%         \bm{k} = \text{RoPE}(\bm{x}\bm{W}_k),
%         \;\;\;
%         \bm{v} = \bm{x}\bm{W}_v
%     \end{equation}
%     where $\text{RoPE}$ denotes applying rotary embeddings~\citep{su2024roformer} to encode position in Llama and Mistral LLMs\footnote{This differs from prior linearizing methods like SUPRA~\citep{mercat2024linearizing}, which apply rotary embeddings \emph{after} the feature map. Unlike the prior, our choice preserves the linear attention kernel connection between $\phi(\cdot)^\top \phi(\cdot)$ and $\exp(\cdot, \cdot)$; Llama and Mistral apply rotary embeddings before the exponential, \textit{i.e.,} 
%     % \(
%     % \bm{q}_i^\top \bm{k}_j = ( \bm{x}_i\bm{W}_q \bm{R}^d_\Theta)^\top (\bm{x}_j\bm{W}_k \bm{R}^d_\Theta)
%     % \)
%     % where $\bm{R}^d_\Theta$ represents the rotary position matrix~\citep{su2024roformer},
%     \(
%     \exp(\bm{q}_i^\top \bm{k}_j) = \exp(\text{RoPE}( \bm{x}_i\bm{W}_q)^\top \text{RoPE}(\bm{x}_j\bm{W}_k))
%     \)
%     % where $\bm{R}^d_\Theta$ represents the rotary position matrix
%     \citep{su2024roformer},
%     }.

%     For all token positions $n \in [l]$, we compute ``ground-truth'' softmax attention outputs $\{\bm{y}_n\}_{n=1}^l$ with Eq.~\ref{eq:causal_attention} and ``predicted'' linear attention outputs $\{\hat{\bm{y}}_n\}_{n=1}^l$ with Eq.~\ref{eq:linear_attention_2},
%     and jointly train $\phi_q, \phi_k$ to minimize the MSE
%     % \begin{equation}
%     %     % \phi_q^*, \phi_k^* = \underset{\phi_q, \phi_k}{\argmin}\;\Big(\; \frac{1}{n}\sum_{i=1}^n (\bm{y}_i - \hat{\bm{y}_i})^2\; \Big)
%     %     \mathcal{L} = \frac{1}{n}\sum_{i=1}^n (\bm{y}_i - \hat{\bm{y}_i})^2
%     % \label{eq:lolcats_mse_loss}
%     % \end{equation}
%     \(
%         \ell_n(\bm{y}_n, \hat{\bm{y}}_n) = \frac{1}{d}\sum_{i=1}^d (y_{n,i} - \hat{y}_{n,i})^2
%     \)
%     for all token positions. During this process, we only train the feature map weights, \textit{i.e.,} freezing all original LLM softmax weights.

%     % With MLP-based feature maps $\phi_\text{mlp} : \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$, for each head we train query and key-specific MLPs
%     % \begin{equation}
%     %     \phi_\text{mlp\_q}(\bm{q}) := f(\bm{q}\tilde{\bm{W}}_q + \tilde{\bm{b}}_q),
%     %     \;\;\;
%     %     \phi_\text{mlp\_k}(\bm{k}) := f(\bm{k}\tilde{\bm{W}}_k + \tilde{\bm{b}}_k)
%     % \end{equation}
%     % % \textit{i.e.,} $\phi_\text{mlp}(\bm{q}) := f(\bm{q}\tilde{\bm{W}} + \tilde{\bm{b}})$,
%     % where $\tilde{\bm{W}} \in \mathbb{R}^{d \times d'}$ and $\tilde{\bm{b}} \in \mathbb{R}^{d'}$ are MLP weights and biases, and $f(x)$ is any element-wise ``activation'' used in prior linear attentions ($\text{ReLU}(x)$ for T2R~\citep{kasai-etal-2021-finetuning}, $[\text{softmax}(x) \oplus \text{softmax}(-x)]$ for Hedgehog~\citep{zhang2024the}).

%     \textbf{Multiple heads and layers}. For an entire LLM with multiple heads and layers, we simply use unique MLPs for each head and layer, and train in a layer-wise fashion. We freeze all original LLM layers (attentions, MLPs, norms), save the attention-layer-wise inputs and outputs after running a forward pass with the original LLM, and train linear attention MLPs with these layer-wise inputs and outputs in each layer as above.
%     %
%     This remains parameter and computation-efficient. Parameter-wise, for Llama 3 8B or Mistral 7B, $d' = 64$, we have 
%     % $32 \times 32 \times 2 \times (128 \times 64) \approx 16.8$M trainable parameters (0.2$\%$ of the original LLM size).
%     32 layers $\times$ 32 heads $\times$ 2 feature maps $\times$ $(128 \times 64)$ $\approx$ 16.8M trainable parameters (0.2$\%$ of the original LLM size).
%     %
%     Computation-wise, similar to multi-head attention, we process the head-specific computations in parallel. We also jointly train all MLPs in a single end-to-end loop. To prevent errors in earlier layers from impacting attention transfer in later layers, we ``teacher-force'' and use the ground-truth softmax attention outputs $\bm{y}^{(m)}$ for layer $m$ to compute inputs $\bm{x}^{(m+1)}$ for the next layer. We include code for all our implementation in Appendix~\ref{}.

%    %  For multiple heads and multiple layers, we train separate query and key feature maps for each head and layer. 
    
%    %  we treat this strictly as a feature map learning problem. Given original softmax attention queries, keys, and values 
    
%    %  linear attention feature maps $\phi : \mathbb{R}^{d} \mapsto \mathbb{R}^{d'}$ where $d$ is the head dimen
    
%    %  linear attention. 
%    %  Considering a single attention head first, we freeze the 
    
%    %  For each softmax attention layer, we copy the query, key, value, and output projections to a linear attention layer with MLP-based feature maps. We then freeze the projection weights, and only train the feature map weights such that the resulting linear attention outputs $\hat{\bm{y}}$ match the original softmax attention outputs $\bm{y}$ via an MSE loss. We found separate query and key feature maps produced better quality linearizations. This remains efficient; with separate weights for each feature map, head, and layer, we still only train $\approx$ 0.2$\%$ of a 7B LLM's parameters.
    
%    %  \textbf{Positional encoding details}. As Llama and Mistral apply rotary embeddings after the query and key projections but before the exponential, \textit{i.e.,} 
%    %  % \(
%    %  % \bm{q}_i^\top \bm{k}_j = ( \bm{x}_i\bm{W}_q \bm{R}^d_\Theta)^\top (\bm{x}_j\bm{W}_k \bm{R}^d_\Theta)
%    %  % \)
%    %  % where $\bm{R}^d_\Theta$ represents the rotary position matrix~\citep{su2024roformer},
%    %  \(
%    %  \bm{q}_i^\top \bm{k}_j = \text{RoPE}( \bm{x}_i\bm{W}_q)^\top \text{RoPE}(\bm{x}_j\bm{W}_k)
%    %  \)
%    %  % where $\bm{R}^d_\Theta$ represents the rotary position matrix
%    %  \citep{su2024roformer},
%    %  unlike SUPRA we preserve the kernel function connection and apply the feature maps \emph{after} the rotary embeddings. 
%    %  % $a_{i, j} = \frac{\exp(\text{RoPE}(\bm{q}_i)^\top \text{RoPE}(\bm{k}_j) / \sqrt{d})}{\sum_{j=1}^n \exp(\text{RoPE}(\bm{q}_i)^\top \text{RoPE}(\bm{k}_j) / \sqrt{d})}$
%    %  For a single attention, we thus first compute MLP-based linear attention queries and keys:
%    %  \begin{equation}
%    %      \phi_q(\bm{q}_i) = f\big(\text{RoPE}(\bm{x}_i \bm{W}_q)\bm{W}_{(\phi^q)} + \bm{b}_{(\phi^q)}\big)
%    %      \;\;\text{and}\;\;
%    %      \phi_k(\bm{k}_j) = f\big(\text{RoPE}(\bm{x}_j \bm{W}_k)\bm{W}_{(\phi ^k)} + \bm{b}_{(\phi^k)}\big)
%    %  \end{equation}
%    %  where $f(x)$ is any element-wise ``activation'' used in prior linear attentions, (\textit{e.g.,} $\text{ReLU}(x)$ for T2R~\citep{kasai-etal-2021-finetuning}, $[\text{softmax}(x) \oplus \text{softmax}(-x)]$ for Hedgehog~\citep{zhang2024the}).
%    % We train the MLPs jointly to minimize an MSE loss:
%    %  \begin{equation}
%    %      \phi_q^*, \phi_k^* = \underset{\phi_q, \phi_k}{\argmin}\;\Big(\; \frac{1}{n}\sum_{i=1}^n (\bm{y}_i - \hat{\bm{y}_i})^2\; \Big)
%    %  \label{eq:lolcats_mse_loss}
%    %  \end{equation}
%    %  following Eq.~\ref{eq:causal_attention} and Eq.~\ref{eq:linear_attention} to compute softmax attention outputs $\bm{y}_i$ and linear attention outputs $\hat{\bm{y}_i}$. We jointly train all layers in a single end-to-end training loop, implemented in Appendix~\ref{}.
%    %  % optimize
%    %  % \begin{equation}
%    %  %     \underset{\bm{W}_q, \bm{W}_k}{\argmin}\;\; \frac{1}{n}\sum_{i=1}^n (\bm{y}_i - \hat{\bm{y}_i})^2
%    %  % \end{equation}
%    %  % \begin{equation}
%    %  %     % \hat{\bm{y}}_i = \frac{\text{softmax}(\text{RoPE}(\bm{q})\bm{W}_q)^\top \text{softmax}(\text{RoPE}(\bm{k})\bm{W}_k)}{}
%    %  %      \hat{\bm{y}}_i = \frac{\phi_q\big(\text{RoPE}(\bm{q}_i)\big)^\top \phi_k\big(\text{RoPE}(\bm{k}_j)\big)}{\sum_{j=1}^i \phi_q\big(\text{RoPE}(\bm{q}_i)\big)^\top \phi_k\big(\text{RoPE}(\bm{k}_j)\big) }
%    %  % \end{equation}
%    %  % such that the linear layers only need $\ldots$ This amounts to training $\approx$ 0.2$\%$ of a 7B LLM's parameters.
    
%     \item \textbf{Low-rank linearization:} We then swap the attentions, before simply replacing the full-parameter training of prior work with low-rank adaptation (LoRA)~\citep{hu2021lora}.
%     Here, we again focus training on the swapped attention layers, and only update the query, key, value, and output projections. However, rather than use full-rank updates $\bm{W}' \leftarrow \bm{W} + \Delta \bm{W}$, LoRA decomposes $\Delta \bm{W}$
%     into the product of two low-rank matrices $\bm{B}\bm{A}$, where $\bm{B} \in \mathbb{R}^{d \times r}$, $\bm{A} \in \mathbb{R}^{r \times d}$. For parameter-efficient training, we aim to pick small $r \ll d$ that still enables sufficient updates for adjusting to the swapped attentions.
%     %
%     Through experiments, we found $r = 8$ (versus $d = 128$ for Llama and Mistral LLMs) sufficient, enabling much more accessible linearizing by only updating $<$0.09\% of original LLM parameter counts.
    
%     % This freezes all layers except for each linear attention's query, key, value and output projections. To train these layers, instead of a full-parameter update 
%     % % \emph{e.g,} $\bm{W}_q' \leftarrow \bm{W}_q + \Delta \bm{W}_q$, we decompose $\Delta \bm{W}_q$
%     % $\bm{W}' \leftarrow \bm{W} + \Delta \bm{W}$, we decompose $\Delta \bm{W}$
%     % into the product of two low-rank matrices $\bm{B}\bm{A}$, where $\bm{B} \in \mathbb{R}^{d \times r}$, $\bm{A} \in \mathbb{R}^{r \times d}$. With $r \ll d$ (we use 8 versus 128 for Llama-3 and Mistral 7B), LoRA makes linearizing LLMs much more accessible (only updating $<$0.09\% of original LLM parameters).
% \end{enumerate}

% As an initial test, we compare the validation split perplexity of low-rank linearized Llama 3 8B and Mistral 7B with and without attention transfer. We compare across both T2R and Hedgehog feature maps, and linearize with the Alpaca dataset~\citep{alpaca}. For fair comparison, we equalize training budgets: 2 epochs for attention transfer and 2 epochs for post-swapped LLM training, or 4 epochs for only post-swapped training.

% Even when accounting for attention training time, linearizing with attention transfer consistently achieves lower perplexity faster. 
% % In Section~\ref{}, we find this corresponds to higher quality with magnitudes less training tokens versus prior linearizing methods.
% % in our empirical analysis below (Section~\ref{}). 
% We further study why this might be possible in Appendix~\ref{}.
% % leave further study of why this is possible to future work. However, 
% One hypothesis is that via only low-rank updates on the attention layers, we (1) preserve the pretrained ``knowledge and concepts'' in parameter-heavy layers such as the MLPs, and (2) focus the purpose of training on the linearizing data for recovering the sequence-mixing patterns of the original attentions. As a result, we can recover generalized LLM capabilities with limited samples.
% % reduce overfitting to linearizing data, avoid needing to ``reteach'' concepts into 
% % and allow for generalized LLM capability recovery with fewer samples. 
% % avoid deleterious changes to parameter-heavy pretrained layers such as the MLPs. This may help retain ``pretrained knowledge'' in para, reducing overfitting to the linearizing data and allowing for LLM recovery with less samples. 
% We find 
% % leave further empirical analysis of this idea to Appendix~\ref{}, but find 
% evidence of this in our main results (\textit{e.g.,} recovering zero-shot LM Eval and 5-shot MMLU quality despite training on 50K Alpaca instruction-following samples).



%
% We compare the validation split perplexity of low-rank linearized Llama 3 8B and Mistral 7B with and without attention transfer, across T2R and Hedgehog feature maps, with the Alpaca dataset~\citep{alpaca}. For fair comparison, we use the same training budget for both settings: 2 epochs for attention transfer and 2 epochs for post-swapped LLM training, or 4 epochs for only post-swapped LLM training. 

% Even when accounting for attention training time, linearizing with attention transfer consistently achieves lower perplexity faster (Figure~\ref{}, Table~\ref{}). In Section~\ref{}, we find this corresponds to higher quality with magnitudes less training tokens versus prior linearizing methods.

% \subsubsection{Improving Linearized Quality with Expanded Subquadratic Attentions}

% While long context quality still depends on the subquadratic analog, this simple switch makes linearizing longer context models more feasible.
% In our analysis below, we find while the Hedgehog loss limits linearizing to shorter contexts due to memory bottlenecks, it also struggles to extrapolate to longer contexts. This can result in significantly worse LLM quality and attention-matching fidelity, \eg{} for Llama 3 8B's native 8192 context length.
% %
% In contrast, \name{} can directly linearize over this longer context, maintaining language modeling quality and still recovering softmax attention weights, despite only training to match on outputs.



% in our main results, we validate each of the contributions above with 

% the less restrictive MSE loss. 




% SCRATCH
% \paragraph{} doing post-swapping training over two epochs over the Alpaca training set~\citep{alpaca} (about 20M token updates).

% Later, we show how this compares to 

% where $f(\bm{x})$ is a generalized function applied after the MLP ($\text{ReLU}(\bm{x})$ in the case of T2R, and $\exp(\bm{x}) \oplus \exp(-\bm{x})$ in the case of Hedgehog)

% Furthermore, to recover quality, we aim to avoid updating pretrained layers like the MLPs.


% To keep attention transfer efficient, we copy all query, key, value, and output projection weights, and only train the linear attention feature maps. We found that we could remove the bias term without loss in quality. Unlike SUPRA, we apply the feature maps \textit{after} the rotary embeddings, such that the normalized $\phi$ only have to learn to approximate the $\text{softmax}$ function.

% For some learnable feature map $\phi(\bm{x}) = \text{activation}(\text{RoPE}(\bm{x})\bm{W})$

% As a plus, we find this approach to be ``linear attention agnostic''. 



% To do so, our key idea is that if we could replace an LLM's softmax attentions with nearly-matching linear attentions, then we would only require a minimal amount of subsequent model parameter updating---if any at all---to adjust and recover original LLM quality. 

% We thus reduce LLM linearization into a two-step procedure, where we first aim to learn softmax-approximating  


% To make linearizing more accessible, we wish 


% As a first step, to improve linearizing training efficiency we simply swap the full-parameter training in existing approaches with low-rank adaptation (LoRA)~\citep{hu2021lora}. 
% %
% While doing so while all prior approaches call for full model training may seem like wishful thinking, we hypothesize that if we could replace an LLM's softmax attentions with nearly-matching linear attentions, then we would only require a minimal amount of model parameter updating---if any at all---to adjust and recover original LLM quality.

% Assuming we \emph{can} obtain these softmax-approximating linear attentions (\textit{e.g.,} via Hedgehog distillation), after attention swapping we first 
% % For every attention layer, we replace the Eq.~\ref{eq:causal_attention} computation with Eq.~\ref{eq:linear_attention}. For post-swap training, we 
% freeze all layers except for the attention query, key, value, and output projections. To then train these layers with LoRA, instead of a full-parameter update, \emph{e.g,} $\bm{W}_q' \leftarrow \bm{W}_q + \Delta \bm{W}_q$, we decompose $\Delta \bm{W}_q$ into the product of two low-rank matrices $\bm{B}\bm{A}$, where $\bm{B} \in \mathbb{R}^{d \times r}$, $\bm{A} \in \mathbb{R}^{r \times d}$. With $r \ll d$ (we use 8 versus 128 for Llama-3 and Mistral 7B), LoRA makes linearizing LLMs much more accessible (only updating $<$0.09\% of original LLM parameters).

% \subsubsection{Enabling Low-Rank Linearization with Attention Transfer}
% \label{sec:method_attention_transfer}
% To combine training efficiency with modeling quality, we subsequently train th


% First trains attention analogs. For different analogs, we found it was sufficient to copy and freeze the attention query, key, value, and output projections, while only training the weights and. 

% Unlocks state-of-the-art linearizing. Verify that much more efficient than prior approaches. Also enables more 


% actually make low-rank linearizing work, 


% While prior works show that we can linearize Transformers by simply swapping attention layers before fully finetuning the model on some downstream task, we make linearizing with LoRA sufficient by first explicitly training the attention analogs to approximate their softmax counterparts. We study if the training setup in \citet{zhang2024the} suffices for learning feature maps $\phi$ that can approximate LLM softmax attentions. 



% Start with attention transfer,

% Then improve tne quality

% Finally improve the linearizing effiiency. 






==> sections/tables/main_results_ablation.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}


\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{0.9\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}lccccc@{}}
\toprule
Feature Map                & \begin{tabular}[c]{@{}c@{}}LM Eval \\ Metric\end{tabular} & \begin{tabular}[c]{@{}c@{}}Swap \&\\ Finetune\end{tabular} & \begin{tabular}[c]{@{}c@{}}+Attention \\ Transfer\end{tabular} & \cellcolor[HTML]{ECF4FF}\begin{tabular}[c]{@{}c@{}}+Sliding Window,\\ +Attention Transfer \end{tabular} & \begin{tabular}[c]{@{}c@{}}+ Sliding Window, \\ No Attention Transfer\end{tabular} \\ \midrule
                           & Avg. Zero-Shot    & 44.20                                                      & 55.32                                                          & \cellcolor[HTML]{ECF4FF}\textbf{70.60}                                                      & {\ul 68.78}                                                                       \\
\multirow{-2}{*}{Hedgehog} & MMLU (5-shot)  & 23.80                                                      & 23.80                                                          & \cellcolor[HTML]{ECF4FF}\textbf{52.50}                                                      & 45.80                                                                             \\ \midrule
                           & Avg. Zero-Shot    & 38.84                                                      & {\ul 54.83}                                                    & \textbf{68.28}                                                                              & 39.52                                                                             \\
\multirow{-2}{*}{T2R}      & MMLU (5-shot)   & 23.20                                                      & 23.10                                                          & \textbf{40.70}                                                                              & 23.80                                                                             \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{\name{} component ablations}, linearizing Llama 3 8B over 1024-token sequences. Default configuration highlighted. Across Hedgehog and T2R feature maps, \name{}' attention transfer and sliding window increasingly improve linearized LLM quality on average LM Eval (Avg.) and 5-shot MMLU scores.
}
\label{table:main_results_ablations}
% \vspace{-0.5cm}
\end{table}

==> sections/tables/main_results_ablation_local.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}


\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{0.9\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}lccccc@{}}
\toprule
Feature Map                & \begin{tabular}[c]{@{}c@{}}LM Eval \\ Metric\end{tabular} & \begin{tabular}[c]{@{}c@{}}Swap \&\\ Finetune\end{tabular} & \begin{tabular}[c]{@{}c@{}}+Attention \\ Transfer\end{tabular} & \cellcolor[HTML]{ECF4FF}\begin{tabular}[c]{@{}c@{}}+Sliding Window,\\ +Attention Transfer \end{tabular} & \begin{tabular}[c]{@{}c@{}}+ Sliding Window, \\ No Attention Transfer\end{tabular} \\ \midrule
                           & Avg. Zero-Shot    & 44.20                                                      & 55.32                                                          & \cellcolor[HTML]{ECF4FF}\textbf{70.60}                                                      & {\ul 68.78}                                                                       \\
\multirow{-2}{*}{Hedgehog}  & MMLU (5-shot)  & 23.80                                                      & 23.80                                                          & \cellcolor[HTML]{ECF4FF}\textbf{52.50}                                                      & 45.80                                                                             \\ \midrule
                           & Avg. Zero-Shot    & 38.84                                                      & {\ul 54.83}                                                    & \textbf{68.28}                                                                              & 39.52                                                                             \\
\multirow{-2}{*}{T2R}      & MMLU (5-shot)   & 23.20                                                      & 23.10                                                          & \textbf{40.70}                                                                              & 23.80                                                                             \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{\name{} component ablations}, linearizing Llama 3 8B over 1024-token sequences. Default configuration highlighted. Across feature maps, \name{}' attention transfer and sliding window increasingly improve linearized LLM quality.
}
\label{table:main_results_ablations}
% \vspace{-0.5cm}
\end{table}

==> sections/tables/main_results_v2.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}


\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{1\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}l|c|cccccc|cc@{}}
\toprule
\multicolumn{1}{c|}{Model}                       & \begin{tabular}[c]{@{}c@{}}Training\\ Tokens (B)\end{tabular} & PiQA                                         & ARC-e                                        & \begin{tabular}[c]{@{}c@{}}ARC-c\\ (norm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HellaSwag\\ (norm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Wino-\\ grande\end{tabular} & \begin{tabular}[c]{@{}c@{}}MMLU \\ (5-shot)\end{tabular} & Avg.                                 & \begin{tabular}[c]{@{}c@{}}Avg. \\ (no MMLU)\end{tabular} \\ \midrule 

\rowcolor[HTML]{EFEFEF} 
\textbf{Transformer}                             & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
Gemma 7B                                         & 6000                                                          & 81.9                                         & 81.1                                         & 53.2                                                   & 80.7                                                       & 73.7                                                   & 62.9                                                     & 72.3                                         & 74.1                                                     \\
Mistral 7B                                       & 8000\footnote{As reported in \citet{mercat2024linearizing}}                                                         & \textbf{82.1}                                & 80.9                                         & \textbf{53.8}                                          & \textbf{81.0}                                              & 74.0                                                   & 62.4                                                     & 72.4                                         & 74.4                                                     \\
Llama 3 8B                                       & 15000                                                         & 79.9                                         & 80.1                                         & 53.3                                                   & 79.1                                                       & 73.1                                                   & \textbf{66.6}                                                     & 72.0                                         & 73.1                                                     \\

\rowcolor[HTML]{EFEFEF}
\textbf{Subquadratic}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
Mamba 7B                                         & 1200                                                          & 81.0                                         & 77.5                                         & 46.7                                                   & 77.9                                                       & 71.8                                                   & 33.3                                                     & 64.7                                         & 71.0                                                     \\
RWKV-6 World v2.1 7B                             & 1420                                                          & 78.7                                         & 76.8                                         & 46.3                                                   & 75.1                                                       & 70.0                                                   & -                                                        & 69.4                                         & 69.4                                                     \\
TransNormerLLM 7B                                & 1400                                                          & 80.1                                         & 75.4                                         & 44.4                                                   & 75.2                                                       & 66.1                                                   & 43.1                                                     & 64.1                                         & 68.2                                                     \\
Hawk 7B                                          & 300                                                           & 80.0                                         & 74.4                                         & 45.9                                                   & 77.6                                                       & 69.9                                                   & 35.0                                                     & 63.8                                         & 69.6                                                     \\
Griffin 7B                                       & 300                                                           & 81.0                                         & 75.4                                         & 47.9                                                   & 78.6                                                       & 72.6                                                   & 39.3                                                     & 65.8                                         & 71.1                                                     \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Hybrid}                                  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
StripedHyena-Nous-7B                             & -                                                             & 78.8                                         & 77.2                                         & 40.0                                                   & 76.4                                                       & 66.4                                                   & 26.0                                                     & 60.8                                         & 67.8                                                     \\
Zamba 7B                                         & 1000                                                          & 81.4                                         & 74.5                                         & 46.6                                                   & 80.2                                                       & \textbf{76.4}                                          & 57.7                                                     & 69.5                                         & 71.8                                                     \\
\rowcolor[HTML]{EFEFEF} 
\textbf{Linearized}                              & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
Mistral 7B SUPRA                                 & 20                                                            & 80.1                                         & 74.6                                         & 42.3                                                   & 74.8                                                       & 67.4                                                   & 28.0                                                     & 61.2                                         & 67.8                                                     \\
Mistral 7B SUPRA                                 & 100                                                           & 80.4                                         & 75.9                                         & 45.8                                                   & 77.1                                                       & 70.3                                                   & 34.2                                                     & 64.0                                         & 69.9                                                     \\
Mistral 7B Hedgehog                              & \textbf{0.04}                                                 & 79.3                                         & 76.4                                         & 45.1                                                   & 73.1                                                       & 57.5                                                   & 28.2                                                     & 59.9                                         & 66.3                                                     \\
\rowcolor[HTML]{96FFFB} 
Mistral 7B LoLCATs (Ours)                        & \textbf{0.04}                                                 & 81.1                                         & 81.1                                         & 52.9                                                   & 80.5                                                       & 73.2                                                   & 52.2                                                     & 70.2                                         & 73.8                                                     \\
Llama 3 8B Hedgehog                              & \textbf{0.04}                                                 & 77.4                                         & 71.1                                         & 40.6                                                   & 50.7                                                       & 54.3                                                   & 24.2                                                     & 53.1                                         & 58.8                                                     \\
\rowcolor[HTML]{96FFFB} 
Llama 3 8B LoLCATs (Ours)  & \textbf{0.04}                                                 & 80.6                                         & \textbf{81.8}                                & 53.5                                                   & 79.1                                                       & 73.4                                                   & 49.1                                                     & 69.6                                         & 73.7                                          
                          \\ \bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{LM Evaluation Harness Results}. Among popular 7B+ LLMs, \name{}-linearized Mistral 7B and Llama 3 8B achieve competitive LM Eval quality to Transformers and consistently outperforming prior pretrained subquadratic Transformer alternatives by 0.1 to 9.4 points (Avg.), while only training 0.2\% of the model parameters on 0.013\% to 0.003\% of past subquadratic LLM pretraining token counts, a 7,500 to 35,500$\times$ improvement in tokens-to-model efficiency. Compared to past linearizing methods, this improves model quality by 6.2 points, with only 0.04\% of their training tokens (a 2,500$\times$ token-efficiency improvement).
}
\label{table:main_results}
% \vspace{-0.5cm}
\end{table}

==> sections/tables/scaled_results.tex <==
\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{1\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}l|c|cccccc|cc@{}}
\toprule
\multicolumn{1}{c|}{Model}                       & \begin{tabular}[c]{@{}c@{}}Training\\ Tokens (B)\end{tabular} & PiQA                                         & ARC-e                                        & \begin{tabular}[c]{@{}c@{}}ARC-c\\ (norm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HellaSwag\\ (norm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Wino-\\ grande\end{tabular} & \begin{tabular}[c]{@{}c@{}}MMLU \\ (5-shot)\end{tabular} & Avg.                                 & \begin{tabular}[c]{@{}c@{}}Avg. \\ (no MMLU)\end{tabular} \\ \midrule 

\rowcolor[HTML]{EFEFEF} 
\textbf{Transformer}                             & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
Llama 70B   &  &  &   &   &  &  &  &   &  \\
\rowcolor[HTML]{EFEFEF}
\textbf{Subquadratic}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
NA           & - & - &  - &  - & - & - & - &  - & - \\                 
\rowcolor[HTML]{EFEFEF} 
\textbf{Hybrid}                                  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
NA & - & - &  - &  - & - & - & - &  - & - \\ 
\rowcolor[HTML]{EFEFEF} 
\textbf{Linearized}                              & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
\rowcolor[HTML]{96FFFB} 
Llama 3 70B LoLCATs (Ours)  & \textbf{0.04}   &  &  &   &   &  &  &  &  \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{LM Evaluation Harness Results}. 
\name{}-linearized Llama 3.1 70B is the first pure subquadratic model above 10Bn parameters. Our model achieves X quality, while only training X\% of the model parameters on X\% of pretraining token counts. 
% Among popular 7B+ LLMs, \name{}-linearized Mistral 7B and Llama 3 8B achieve competitive LM Eval quality to Transformers and consistently outperforming prior pretrained subquadratic Transformer alternatives by 0.1 to 9.4 points (Avg.), while only training 0.2\% of the model parameters on 0.013\% to 0.003\% of past subquadratic LLM pretraining token counts, a 7,500 to 35,500$\times$ improvement in tokens-to-model efficiency. Compared to past linearizing methods, this improves model quality by 6.2 points, with only 0.04\% of their training tokens (a 2,500$\times$ token-efficiency improvement).
}
\label{table:70b_results}
% \vspace{-0.5cm}
\end{table}


\begin{table}[t]
% \vspace{-0.25cm}
\begin{center}
\resizebox{1\linewidth}{!}{
% \addtolength{\tabcolsep}{-0.4em}
\begin{tabular}{@{}l|c|cccccc|cc@{}}
\toprule
\multicolumn{1}{c|}{Model}                       & \begin{tabular}[c]{@{}c@{}}Training\\ Tokens (B)\end{tabular} & PiQA                                         & ARC-e                                        & \begin{tabular}[c]{@{}c@{}}ARC-c\\ (norm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}HellaSwag\\ (norm)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Wino-\\ grande\end{tabular} & \begin{tabular}[c]{@{}c@{}}MMLU \\ (5-shot)\end{tabular} & Avg.                                 & \begin{tabular}[c]{@{}c@{}}Avg. \\ (no MMLU)\end{tabular} \\ \midrule 

\rowcolor[HTML]{EFEFEF} 
\textbf{Transformer}                             & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
Llama 3.1 405B   &  &  &   &   &  &  &  &   &  \\
\rowcolor[HTML]{EFEFEF}
\textbf{Subquadratic}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
NA           & - & - &  - &  - & - & - & - &  - & - \\                 
\rowcolor[HTML]{EFEFEF} 
\textbf{Hybrid}                                  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
Jamba 1.5 Large & - & - &  - &  - & - & - & - &  - & - \\ 
\rowcolor[HTML]{EFEFEF} 
\textbf{Linearized}                              & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}                 & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}               & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}           & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}}            & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}}             \\
\rowcolor[HTML]{96FFFB} 
Llama 3.1 405B LoLCATs (Ours)  & \textbf{0.04}   &  &  &   &   &  &  &  &  \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{\textbf{LM Evaluation Harness Results}. 
\name{}-linearized Llama 3.1 405B is the first pure subquadratic model above 100Bn parameters and the largest amongst all categories of non-Transformer models. Our model achieves X quality, while only training X\% of the model parameters on X\% of pretraining token counts. 
% Among popular 7B+ LLMs, \name{}-linearized Mistral 7B and Llama 3 8B achieve competitive LM Eval quality to Transformers and consistently outperforming prior pretrained subquadratic Transformer alternatives by 0.1 to 9.4 points (Avg.), while only training 0.2\% of the model parameters on 0.013\% to 0.003\% of past subquadratic LLM pretraining token counts, a 7,500 to 35,500$\times$ improvement in tokens-to-model efficiency. Compared to past linearizing methods, this improves model quality by 6.2 points, with only 0.04\% of their training tokens (a 2,500$\times$ token-efficiency improvement).
}
\label{table:405b_results}
% \vspace{-0.5cm}
\end{table}
